Two lectures on the enumeration of curves by means of floor diagrams

We discuss, following Mikhalkin, Brugall\'e, and many others, the counting of curves on toric surfaces with prescribed genus, Newton polygon, and intersection pattern with the toric boundary divisor, both at assigned and unassigned points. The first lecture is dedicated to the proof of a correspondence theorem (for plane curves) with the counting of floor diagrams, using a degeneration of the projective plane to a chain of rational ruled surfaces. This is due to Brugall\'e and does not involve any tropical geometry. The second lecture explores the relations with tropical geometry, and contains an introduction to toric varieties and tropical geometry. We discuss the correspondence theorem of Mikhalkin, and show how the corresponding tropical enumerative problem can be formulated in terms of the combinatorial problem of counting floor diagrams. We give many examples throughout, inspired by the study of the enumerative geometry of $K3$ surfaces, by degeneration to unions of rational surfaces with dual complex a tiling of the $\mathbf{S}^2$ sphere.

==> diag-degen.tex <==
\chaptitle{Enumeration of curves by floor diagrams,
  via degenerations of the projective plane}
\chapauthor{Thomas Dedieu}

\startchap
\label{07.th-diag-degen}

\setdefaultenum{(i)}{}{}{}
\setdefaultitem{---}{}{}{}

%\newcounter{memoire}
% already defined

% needs counter memoire
% \newenvironment{subnum-par}
% {\setcounter{memoire}{\value{paragraph}+1}
% \setcounter{paragraph}{0}
% \renewcommand{\theparagraph}
% {(\arabic{section}.\arabic{memoire}.\alph{paragraph})}
% }
% {\setcounter{paragraph}{\value{memoire}}}

% needs counter memoire
\newenvironment{subnum-fig}
{\setcounter{memoire}{\value{figure}+1}
\setcounter{figure}{0}
\renewcommand{\thefigure}
{\arabic{memoire}\alph{figure}}
}
{\setcounter{figure}{\value{memoire}}}

\providecommand{\cP}{\mathcal{P}}
\newcommand{\CM}{C \kern -.1em M}

\newcommand{\bigdlbrack}{\big[ \kern -.7ex \big[}
\newcommand{\bigdrbrack}{\big] \kern -.7ex \big]}

\newcommand{\NN}{\underline{\N}}
\newcommand{\Nseq}{\underline{\N}}

%\newcommand{\Card}{\operatorname{Card}}

\newcommand{\irr}{\mathrm{irr}}
\newcommand{\con}{\mathrm{con}}

% macros diagrammes
\newcommand{\diag}{\mathcal{D}}
\newcommand{\orient}{\mathsf{D}}
\newcommand{\vt}{\operatorname{Vert}}
\newcommand{\edg}{\operatorname{Edges}}

%\maketitle


\startcontents[diag-degen]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[diag-degen]{}{1}[2]{}


\bigskip
The goal of this text is to present a combinatorial translation of the
same enumerative problem considered in \cite{04.concettina}, namely
that of counting plane curves of given degree and genus, with a
prescribed intersection pattern with a fixed line, both at assigned
and unassigned point, and passing through the appropriate number of
fixed general points in the plane.
The result is the
Correspondence Theorem \ref{t:corresp}, which says that it is
equivalent to count curves as above, and to count certain
combinatorial gadgets called marked floor diagrams.
Although, as is well-known, being a problem combinatorial doesn't make
it easy, it is possible to teach a computer to count floor
diagrams, whereas teaching it to directly solve the initial
algebro-geometric problem is arguably hopeless.

The Correspondence Theorem has first been obtained by Brugallé and
Mikhalkin \cite{BM}, using tropical geometry.
Here we present a proof which is purely algebro-geometric,
due to Brugallé, see \cite{erwan}.
This proof is by degeneration of the projective plane.
The idea in Brugallé and Mikhalkin's first proof,
see \cite{11.th-toric-trop},
was to strech the
general base points of the enumerative problem along a preferred
direction in the plane;
in Brugallé's proof presented here, this idea takes the following
form.
Let $r$ be the number of fixed general points in the enumerative
problem. One lets the plane degenerate to a chain of $r$ rational
ruled surfaces $\F_1$, in such a way that the fixed points of the
problem end up one
on each of the surfaces of the chain.
This has the effect that the curves one has to count in the limit in
order to solve the enumerative problem are so to speak maximally
degenerate, in the sense that all their irreducible components are
rational curves, which are moreover either sections or fibres of
rational normal scrolls. One is thus left with objects from which all
irrationality has vanished, so that it is possible to encode them in
combinatorial terms.

The recursive formula obtained by Caporaso and Harris
about the same enumerative problem, presented in the previous
lecture \cite{04.concettina}, may be interpreted in terms of a
degeneration of the projective plane to a transverse union of two
rational surfaces, see \cite{08.th-exem}.
The base cases of this recursion are the enumerative problems for
degree one plane curves, \ie lines.
In Brugallé's proof, one somehow lets all the degenerations
corresponding to the various iterations of the Caporaso--Harris'
recursive procedure, all the way to the base cases,
happen at once.

In order to directly follow Brugallé's proof, it is necessary to
consider spaces of maps instead of the genuine Severi varieties,
which parametrize curves embedded in surfaces.
Indeed, multiple curves (or rather non-birational maps) inevitably
show up.
It follows that the results on degenerations of nodal curves along
degenerations of surfaces usually considered in this volume,
see \cite{01.ciro} say, are not directly applicable. Following
Brugallé, we use instead Jun Li's theory of relative stable maps
\cite{junli-stable, junli-degen}.
This theory will regrettably not be presented in this volume,
and here I shall directly state its output
without trying to give any explanation.
Based on my personal experience, I believe that they should
nevertheless look reasonable enough to anyone familiar with the
results presented in due form in this volume.
Finally, note that it should be possible
(albeit certainly less convenient)
to recast this proof using the theory expound in 
\cite{01.ciro}; indications to that effect are given in
Section \ref{S:ourway-07}.

In Section \ref{S:statements-07} we define floor diagrams and their
markings, and state the Correspondence Theorem.
In Section \ref{S:modspace} we introduce the moduli spaces of maps
that are needed for the proof of the Correspondence Theorem.
Section \ref{S:degen} is the heart of the text, it contains the
description of the degeneration
(see Proposition \ref{pr:erwan})
that will finally give the proof of the Correspondence Theorem
in Section \ref{S:combin}, when we interpret it in combinatorial
terms.
Lastly, Section \ref{S:ourway-07} is devoted to the interpretation of the
considerations in this text in terms of the theory expound in
\cite{01.ciro}. 


% \paragraph*{Thanks}
\medskip \noindent \textbf{Thanks.}
Many thanks to Erwan Brugallé for explaining all this to me and for
answering unflustered my endless questions.
Thanks also for your observations on this text.
I know the secret meaning of the ``French adage'' you quote
in \cite{erwan}.


\paragraph{Notation}
\label{p:genl-notation}
We use freely the notation introduced in
\cite[\ttref{not:Nseq}]{03.th-acz}.
In particular, $\Nseq$ denotes the set of sequences $\alpha =
[\alpha_i]_{i\geq 1}$ of non-negative integers with 
finitely many $\alpha_i$ non-zero, and for all $\alpha \in \Nseq$,
$|\alpha| = \sum_{i\geq 1} \alpha_i$ and
$I\alpha = \sum_{i \geq 1} i\alpha_i$.

For any two integers $a \leq b$, we let
$\intint a b = [a,b] \cap \Z$.

In regard to the projective plane $\P^2$, we let $H$ denote the line
class.
In regard to the Hirzebruch ruled surface $\F_1$
(equivalently, $\P^2$ blown-up at one point),
we let $E$ be the class of the $(-1)$-curve,
$F$ be the class of the fibers of the ruling $\F_1 \to \P^1$,
and $H=E+F$.


\section{Definitions and statement of the result}
\label{S:statements-07}

\subsection{Floor diagrams of plane curves relative to a line}
\label{s:diags}

In this section we define the floor diagrams corresponding to plane
algebraic curves relative to a line.
They are a particular instance of the floor diagrams considered in
\cite{11.th-toric-trop}, and they are the only floor diagrams that
will be considered in this text. Thus we simply call them floor
diagrams, with no additional epithet.

\paragraph{A special class of weighted oriented graphs}
\label{p:graphs}
We shall consider connected, acyclic, oriented graphs $\diag$, with
finitely many vertices and edges.
We denote by $\vt (\diag)$ and $\edg (\diag)$ the
sets of vertices and edges of $\diag$, respectively (or simply $\vt$
and $\edg$ if no confusion is likely).
We see $\edg$ as a subset of
$\vt \times \vt$,
with the first (resp.\ second) factor corresponding to the origin
(resp.\ target) of an edge.
We let $\diag_{\rm top}$ be the topological incarnation of $\diag$ as a
$1$-dimensional CW-complex.

We let
the \emph{vertices at  infinity} of $\diag$ be
those $1$-valent vertices of $\diag$
for which the  unique adjacent edge is outgoing.
The other vertices of $\diag$ will be called \emph{floors}
(this name will be explained in \cite{11.th-toric-trop}).
We denote by
$\vt ^{-\infty}$ and $\vt^{\rm fin}$
the sets of vertices at infinity and floors, respectively.
By definition, there cannot be any
edge joining two vertices at infinity.
Thus, there is a partition
$\edg = \edg^{\infty} \coprod \edg^{\rm fin}$,
where $\edg^{\infty}$ is the set of edges originating from a
vertex at infinity, and
$\edg^{\rm fin}$ is the set of those edges joining two floors.
The former edges are called \emph{infinite},
and the latter \emph{finite}.
% In the terminology of Definition \tmpref{d:floors-n-elevators}, one calls
% the edges of $\diag$ (either finite or infinite)
% \emph{elevators}.


We will in addition assume that our graphs are weighted, which means
that they come equipped with a
function $w: \edg \to \N^*$, which we call
\emph{weight function}
One then defines the
\emph{divergence} $\div (v)$ of a vertex $v$ (either at infinity or a
floor) as
\begin{equation*}
\textstyle
\div (v) = \sum _{(s,v) \in \edg} w(s,v) - \sum _{(v,t) \in \edg} w(v,t)
\end{equation*}
(``sum of weights of incoming edges minus sum of weights of outgoing
edges'').


\par We adopt the following graphical convention: floors will be
represented by ellipses, and vertices at infinity will not be
represented; 
edges will be represented by vertical line segments, oriented from the
bottom to the top.
The weight of an edge is indicated
only if it is greater than $1$, as a circled integer.

\begin{definition}[floor diagram]
Let $d,g$ be nonnegative integers.
A (plane) floor diagram of degree $d$ and
genus $g$ is a connected, acyclic,
weighted oriented graph of the class described in
\ref{p:graphs}, such that the following conditions hold:
\begin{mycpctenum}[(i)]
\item the first Betti number $b_1(\diag _{\rm top})$ equals $g$;
\item every floor has divergence $1$;
\item $\sum _{e \in \edg^\infty} w(e) = -d$.
\end{mycpctenum}
\end{definition}

\begin{example}
All possible floor diagrams of degree $3$ and genus
$1$ are pictured in Figure \ref{fig:d3g1}
below.
When computing the genus, \ie  $b_1(\diag _{\rm top})$,
one should keep in mind that ellipses represent floors, which are
vertices, hence the real ellipse does not contribute to
$b_1$.\footnote
{To make this a rational choice (pun intended),
  think of the ellipses as rational
curves (after all ellipses are conics!), hence as having genus $0$.}
In the three diagrams below, the only cycle contributing to $b_1$ is
that formed by the two lower floors and the two edges between them
(it consists of two edges joining the two same vertices).
\begin{figbox}
\includegraphics{d3g1-300.eps}
\hspace{10mm}
\includegraphics{d3g1-110.eps}
\hspace{10mm}
\includegraphics{d3g1-001.eps}
\captionof{figure}{Floor diagrams of degree $3$ and genus
  $1$}
\label{fig:d3g1}
\end{figbox}
\end{example}

\paragraph{}
We let $\orient$ be the abstract set $\vt ^{\rm fin} \coprod
\edg$, whose elements are all floors and edges.
Since $\diag$ is acylic, the set $\orient$ inherits a partial
ordering from the orientation.

\medskip\noindent
Before we state the next definition, it is worth noting the following
relations. 

\begin{lemma}
Let $\diag$ be a floor diagram of degree $d$ and genus $g$. The two
following equalities hold:
\begin{mycpctenum}[(i)]
\item \label{card-d} $\Card (\vt^{\rm fin}) = d$;
\item \label{card-dim} $\Card (\orient) = 2d+g-1 + \Card (\vt^{-\infty})$.
\end{mycpctenum}
\end{lemma}

\begin{proof}
One has
\begin{align*}
\textstyle
0 = \sum _{v\in \vt} \div (v)
&= \textstyle
 \sum _{v\in \vt ^{\rm fin}} \div (v) + \sum _{v\in \vt^{-\infty}}
\div (v) \\
&= \Card (\vt^{\rm fin})-d,
\end{align*}
which proves \eqref{card-d}.
The Euler characteristic of $\diag _{\rm top}$ is
\begin{equation*}
1-g = \Card (\vt) - \Card (\edg),
\end{equation*}
so
\begin{align*}
\Card (\orient) &= \Card (\vt^{\rm fin}) + \bigl(g-1+ \Card (\vt)\bigr) \\
&= 2\Card (\vt^{\rm fin}) + g -1 + \Card (\vt^{-\infty}),
\end{align*}
which together with \eqref{card-d} proves \eqref{card-dim}.
\end{proof}


\begin{definition}[marking]
Let $\diag$ be a floor diagram of degree $d$ and genus $g$,
and $\alpha, \beta \in \NN ^2$, such that $I\alpha + I\beta = d$.
A \emph{marking of type $(\alpha,\beta)$} of $\diag$ is
a strictly increasing function
\begin{equation*}
  m : \bigl\{ -|\alpha|+1, \ldots, 1, \ldots, 2d+g-1+|\beta|
  \bigr\}
\to \orient
\end{equation*}
such that:
\begin{mycpctenum}[(i)]
\item $\forall k \in \N^*$, 
$\forall i \in \bigdlbrack -|\alpha|+(\sum _{j\leq k-1} \alpha_j) +1,\,
-|\alpha|+\sum _{j\leq k} \alpha_j \bigdrbrack$,
$m(i) \in \edg ^\infty$ and $w(m(i))=k$;
\item $\forall k \in \N^*$, there are exactly $\beta _k$ infinite
  edges of weight $k$ in
$m \bigl( \bigdlbrack 1, 
2d+g-1+|\beta| \bigdrbrack \bigr)$.
\end{mycpctenum}
\end{definition}
% The condition that $m$ be injective and increasing means that for all
% $a,b \in \orient$, $a>b \implies m(a) > m(b)$.

\bigskip
A floor diagram $\diag$ enhanced with a marking $m$ of type
$(\alpha,\beta)$ is called a
\emph{marked floor diagram} $(\diag,m)$ of type $(\alpha,\beta)$.

Two marked floor diagrams of the same type are \emph{equivalent}
if there exists an isomorphism of oriented graphs
$\phi: \diag  \cong \diag'$ such that
$w=w'\circ \phi$
and $m= \phi \circ m'$.

Markings will be indicated on graphic representations by plain
numbers. Beware not to confuse them with weights, which are circled
integers. 

\begin{examples}
\label{ex:cubics-diag}
Up to equivalence, there is a unique marked floor diagram of degree $3$,
genus $1$, and type $(0,3)$.

\smallskip
\subparagraph{Marked floor diagrams of degree $3$ and genus
$0$ of type  $(0,3)$}
\label{p:d3g0-plain}
Below I give all possibilities for such diagrams.
For the leftmost diagram there is a
unique marking (up to equivalence). For the next one, there are $5$:
the label $i$ may be chosen arbitrarily in $\intint 1 5$, and this
choice determines uniquely the four labels not indicated on the picture.
For the rightmost diagram, there are $3$: the index $i$ may
be chosen arbitrarily in $\intint 6 8$, and then the two remaining
labels are uniquely determined.
% \footnote
% {For the rightmost diagram, the marking breaks
% the symmetry in that it is no longer possible to exchange the two
% upper ellipses; graphically it is best to put the two upper ellipses
% on two different levels, so as to respect the order of their
% respective markings.}
\begin{figbox}
\includegraphics[scale=1.3]{d3g0-3a.eps}
\hspace{10mm}
\includegraphics[scale=1.3]{d3g0-3b.eps}
\hspace{10mm}
\includegraphics[scale=1.3]{d3g0-3c.eps}
\captionof{figure}{Marked floor diagrams of degree $3$ and genus
  $0$ of type  $(0,3)$.}
\label{fig:d3g0-plain}
\end{figbox}


\smallskip
\subparagraph{Marked floor diagrams of degree $3$ and genus
$0$ of type  $(0,[1,1])$}
\label{p:d3g0-0+11}
All possible marked diagrams of this type are displayed below.
The leftmost diagram has two possible markings, determined by the
choice of $i \in \intint 1 2$.
The central diagram has four possible markings, determined by the
choice of $i \in \intint 1 4$.
The rightmost diagram has six possible markings, determined first by the
choice of $i \in \intint 1 2$, which fixes $i'$, and then by the
choice of $j \in \intint 5 7$ which fixes the rest.
\begin{figbox}
\includegraphics[scale=1.3]{d3g0-11a.eps}
\hspace{10mm}
\includegraphics[scale=1.3]{d3g0-11b.eps}
\hspace{10mm}
\includegraphics[scale=1.3]{d3g0-11c.eps}
\captionof{figure}{Marked floor diagrams of degree $3$ and genus
$0$ of type  $(0,[1,1])$.}
\end{figbox}


\smallskip
\subparagraph{Marked floor diagrams of degree $3$ and genus
$0$ of type  $([0,1],1)$}
All possible marked diagrams of this type are displayed below.
It is instructive to make comparisons with the type $(0,[1,1])$
considered in the previous paragraph \ref{p:d3g0-0+11}.
The leftmost diagram has a unique possible marking.
The central diagram has three possible markings, determined by the
choice of $i \in \intint 1 3$.
The rightmost diagram has three possible markings, determined by the
choice of $j \in \intint 4 6$.
\begin{figbox}
\includegraphics[scale=1.3]{d3g0-01+1a.eps}
\hspace{10mm}
\includegraphics[scale=1.3]{d3g0-01+1b.eps}
\hspace{10mm}
\includegraphics[scale=1.3]{d3g0-01+1c.eps}
\captionof{figure}{Marked floor diagrams of degree $3$ and genus
$0$ of type  $([0,1],1)$.}
\end{figbox}
\end{examples}



\subsection{The enumerative problem}
\label{s:severi}
% Log-Severi varieties and their degrees

We shall now state precisely the enumerative problem we are interested
in. The definitions below are specializations of those given in
\cite{03.th-acz}.

Assume a line $\Lambda \subset \P^2$ is fixed.
Let $d>0$ and $g\geq 0$ be integers, and $\alpha, \beta \in \Nseq$,
such that $I\alpha+I\beta = d$.
Let $\Omega$ be a general set of $\alpha$ points on $\Lambda$.
We let $V^{d, {\rm irr}}_g(\alpha,\beta)(\Omega)$ be the
Zariski closure in the projective space $\vert \O _{\P^2} (d) \vert$
of the localy closed set $\mathring V ^{d,
{\rm irr}}_g(\alpha,\beta)(\Omega)$ parametrizing irreducible
curves $C \subset \P^2$ of degree $d$, genus $g$,
and having intersection pattern with $\Lambda$ prescribed by $\alpha,\beta$
and $\Omega$ as follows:
write $\Omega = \bigl( \{p _{i,j}\} _{1 \leq j \leq \alpha_i}
\bigr) _{i \geq 1}$, and let $\nu: \bar C \to C$ be the normalization
of $C$; we ask that there exist $\alpha$ points $q _{i,j} \in C$, $1 \leq j
\leq \alpha_i$, and $\beta$ points $r _{i,j} \in C$, $1 \leq j \leq
\beta_i$, such that
\begin{equation*}
\forall\, 1 \leq j \leq \alpha_i:
\quad 
\phi (q_{i,j}) = p_{i,j} 
\qquad \text{and} \qquad
\phi^* \Lambda = \sum _{1 \leq j \leq \alpha_i} i \, q_{i,j}
+ \sum _{1 \leq j \leq \beta_i} i\, r_{i,j}.
\end{equation*}
The variety $V^{d, {\rm irr}}_g(\alpha,\beta)(\Omega)$
has dimension $2d+g-1+|\beta|$.
We call it a
logarithmic Severi variety of irreducible\footnote
{in the definition given in \cite{03.th-acz}, the curve $C$ was not
  required to be irreducible; the superscript '$\irr$' indicates this
  additional requirement.}
plane curves, relative to
the line $\Lambda$.

We let $N^{d, {\rm irr}}_g(\alpha,\beta)$ be
the degree of $V^{d, {\rm irr}}_g(\alpha,\beta)(\Omega)$ as a
projective subvariety of $|\O_{\P^2}(d)|$; it is independent of the
choice of $\Lambda$ and $\Omega$.
This is the number of plane curves of degree $d$, genus $g$, and
having contact of the required type with $\Lambda$, that pass through
$2d+g-1+|\beta|$ general points on $\P^2$.


\subsection{The Correspondence Theorem}
\label{s:corresp}

The Correspondence Theorem \ref{t:corresp} 
is the central result of this text. It will be proved in
the subsequent sections.
It states that one can compute the numbers
$N^{d, {\rm irr}}_g(\alpha,\beta)$
by enumerating floor diagrams. To do so, one needs
to count the latter with the appropriate multiplicity.

\begin{definition}
\label{d:mult-floor}
Let $(\diag,m)$ be a marked floor diagram of type $(\alpha,\beta)$.
Its multiplicity is
\begin{equation*}
\mu^\C (\diag,m) = I^\beta \prod _{e \in \edg^{\rm fin}} w(e) ^2.
\end{equation*}
\end{definition}

\noindent
Thus, the multiplicity of a marked
floor diagram is the product of the multiplicities of its edges where: 
\begin{mycpctenum}[(a)]
\item
  a finite edge of weight $w$ has multiplicity $w^2$;
\item
  an infinite edge of weight $w$ corresponding to a mobile boundary
  condition\footnote
  {the term 'boundary' comes from the definition \ref{p:stable-maps},
  see Paragraph \ref{p:corresp_diag-curve}.}
  (\ie such that its label in the marking is positive)
  has multiplicity $w$;
\item
  an infinite edge of weight $w$ corresponding to a fixed boundary
  condition
  (\ie such that its label in the marking is non-positive)
  has multiplicity $1$.
\end{mycpctenum}

\medskip
One may simply write $\mu^\C (\diag)$ in place of $\mu^\C (\diag,m)$
since the multiplicity only depends on the type and not on the 
marking. We leave the original superscript '$\C$' as a reminder that
this is the correct multiplicity only in order to count \emph{complex}
plane curves.

\begin{theorem}[Brugallé--Mikhalkin \cite{BM}, see also \cite{arroyoetal}]
\label{t:corresp}
Let $d>0$ and $g\geq 0$ be integers, and $\alpha, \beta \in \Nseq$,
such that $I\alpha+I\beta = d$.
One has
\begin{equation*}
N^{d, {\irr}}_g (\alpha,\beta)
= \sum _{(\diag,m)}%\, \in\, \operatorname{MkDiag}^d_g (\alpha,
% \beta)}
\mu^\C (\diag,m),
\end{equation*}
where the sum on the right-hand-side is taken over all
equivalence classes of marked floor diagrams of degree $d$, genus $g$,
and type $(\alpha,\beta)$.
\end{theorem}

\begin{example}
Let us compute the numbers
$N^{3, {\irr}}_0 (\alpha,\beta)$ in the cases considered in
Example \ref{ex:cubics-diag}, by enumerating floor diagrams.

For $(\alpha, \beta) = (0,3)$, the diagram of the leftmost shape has
multiplicity $4$, and all the other have multiplicity $1$.
Thus
\[
  N^{3, {\irr}}_0 (0,3) = 1 \times 4 + 5 + 3 = 12
\]
(the first number of each summand indicates the number of possible
markings for a diagram of the given shape, and the second one
indicates the multiplicity; it is omitted if it is one).

For $(\alpha, \beta) = (0,[1,1])$, the diagrams of the leftmostshape have
multiplicity $8$, and all the other have multiplicity $2$.
Thus
\[
  N^{3, {\irr}}_0 (0,[1,1]) = 2 \times 8 + 4 \times 2 + 6 \times 2 = 36.
\]

For $(\alpha, \beta) = ([0,1],1)$, the diagram of the leftmost shape has
multiplicity $4$, and all the other have multiplicity $1$.
Thus
\[
  N^{3, {\irr}}_0 (0,[1,1]) = 1 \times 4 + 3 + 3 = 10.
\]

\end{example}


\section{Log-GW invariants of $\P^2$ and
  Hirzebruch surfaces}
\label{S:modspace}

Despite the definition of logarithmic Severi varieties having been
given in terms of embedded curves in Section~\ref{s:severi}, it will be
necessary in the context of these notes to consider their counterparts
as spaces of stable maps. Indeed we will need to consider stable maps
that are not birational.
Moreover, we will degenerate $\P^2$
to the unions of $\P^2$ and various copies of $\F_1$,
and therefore we need
to define these spaces not only for the projective plane.
The results stated in this section initially appeared in \cite{ch-07}
and \cite{vakil-07}.

\begin{definition}
Let $X$ be a smooth variety. A \emph{stable map} to $X$ is a map
$f:C \to X$ with source $C$ a nodal curve,
such that $C$ has only finitely many automorphisms commuting with
$f$.
\end{definition}

The finiteness of automorphisms condition boils down to the following
requirement: for all irreducible components $C_i$ of $C$ such that
$p_a(C_i) \leq 1$ and $C_i$ is contracted by $f$,
if $p_a(C_i)=0$ (resp.\ $p_a(C_i)=1$),
then $C_i$ has at least three (resp.\ one)
intersection points with the other components of $C$.


\paragraph{Stable maps relative to a curve}
\label{p:stable-maps}
Let $S$ be a smooth projective surface, and $R \subset S$ be a fixed
smooth curve (not necessarily connected).
The curve $R$ is often called the \emph{boundary} of the pair $(S,R)$.
Let $g \in \Z _{\geq 0}$, $\xi \in \NS (S)$,
and $\alpha,\beta \in \Nseq$,
such that
$I\alpha + I\beta = \xi \cdot R$.
Let $n \in \N$.
Let
$\Omega = \bigl( \{p _{i,j}\} _{1 \leq j \leq \alpha_i}
\bigr) _{i \geq 1}$
be a set of $\alpha$ general points on $R$.
We define $M_g^{\xi, \con} (\alpha,\beta)(\Omega)$
as the moduli space
%set of isomorphism classes
of stable maps
$f: C \to S$ such that:
\begin{compactenum}
\item $C$ is a connected projective curve of arithmetic genus $g$;
\item $f_* [C] = \xi \in \H^2(S,\Z)$;
\item $f(C)$ and $R$ have no irreducible component in common;
\item there exist $\alpha$ points $q _{i,j} \in C$, $1 \leq j
\leq \alpha_i$, and $\beta$ points $r _{i,j} \in C$, $1 \leq j \leq
\beta_i$, such that
\begin{equation*}
f (q_{i,j}) = p_{i,j} 
\quad \forall\, 1 \leq j \leq \alpha_i,
\qquad \text{and} \qquad
f^* R = \sum _{1 \leq j \leq \alpha_i} i \, q_{i,j}
+ \sum _{1 \leq j \leq \beta_i} i\, r_{i,j}.
\end{equation*}
\setcounter{memoire}{\value{enumi}}
\end{compactenum}
If $x=\{x_1,\ldots,x_n\}$ is a set of $n$ general points on $S$, we
define 
$M_g^{\xi, \con} (\alpha,\beta)(\Omega,x)$
as the moduli subspace of $M_g^{\xi, \con} (\alpha,\beta)(\Omega)$
determined by the further requirement:
\begin{compactenum}
\setcounter{enumi}{\value{memoire}}
\item
\label{c:thru-x}
$f(C) \supset x$ as sets.
\end{compactenum}
Similarly, for all components $M$ of
$M_g^{\xi, \con} (\alpha,\beta)(\Omega)$,
$M(x)$ is the subspace of $M$ determined by condition
\eqref{c:thru-x} above.


The superscript '$\con$' stands for 'connected'; note that $C$ is
required to be connected but may be reducible.
We do not require that $f$ be birational.
% The above definition parallels the one given
% in \cite{03.th-acz}, but there are minor differences between the two.

An isomorphism between two stable maps $f_1:C_1 \to X$ and
$f_2:C_2 \to X$ is an isomorphism $\phi: C_1 \to C_2$ such that
$f_1 = f_2 \circ \phi$.
The existence of moduli spaces of stable maps is a highly non-trivial
result. We refer to \cite{stephane} for an exposition in the case of
plain stable maps; the result for relative stable maps
(\ie stable maps with additional features as in \ref{p:stable-maps})
is due to Jun Li, see \cite{junli-stable,junli-notes}.




\paragraph{}
\label{p:notations-P2-F1}
We shall consider instances of the space
$M_g^{\xi, \irr} (\alpha,\beta)(\Omega)$
in the two following situations.
\subparagraph{}\label{sp:mapsP^2}\smallskip
$S=\P^2$,
$\xi = dH$ with for some integer $d>0$,
and $R=\Lambda$ a line; we may then write 
$M^{d,\con}_g (\alpha, \beta)(\Omega)$ or even
$M^{d,\con}_g (\alpha, \beta)$ in place of 
$M_g^{\xi, \con} (\alpha,\beta)(\Omega)$. 
\subparagraph{} \label{sp:mapsF_1}\smallskip
$S = \F_1$,
$\xi = \lambda H + kF$ for some nonnegative integers
$\lambda, k$, and $R = \Lambda _{E} \sqcup \Lambda _{H}$, the
disjoint union of two curves $\Lambda _{E} \in |E|$ and $\Lambda _{H}
\in |H|$
(recall Notation \ref{p:genl-notation}).
In this case it is better to impose directly contact
conditions with $R$
that are decomposed in two disjoint set of contact conditions 
$(\alpha_E,\beta_E,\Omega_E)$ and $(\alpha_H,\beta_H,\Omega_H)$ with
$\Lambda_E$ and $\Lambda_H$ respectively.
One thus obtains a set
$M^{\xi,\con}_g (\alpha_E, \alpha_H, \beta_E, \beta_H)(\Omega_E, 
\Omega_H)$ of (isomorphism classes of) stable maps;
we may abuse the notation of \ref{p:stable-maps} and
still denote this space by $M_g^{\xi, \con}
(\alpha,\beta)(\Omega)$, with $\alpha = (\alpha_E,\alpha_H)$,
$I\alpha = I\alpha_E+I\alpha_H$ and $|\alpha| =
|\alpha_E|+|\alpha_H|$, 
and similarly for $\beta = (\beta_E,\beta_H)$.
One has
\[
I\alpha_E+I\beta_E = \xi \cdot E = k,
\qquad
I\alpha_H+I\beta_H = \xi \cdot H = \lambda +k,
\]
and $-(K_S+R)=2F$.


\bigskip
We shall be interested only in those irreducible components $M$ of
$M_g^{\xi, \con} (\alpha,\beta)(\Omega)$ that are
\emph{enumeratively relevant},
\ie such that for a set $x$ of $n=\dim(M)$ general points on $S$, the
subspace $M(x)$ of those stable maps in $M$ whose image contains $x$
is not empty.
The other irreducible components of $M$ are said to be
\emph{enumeratively irrelevant};
their enumerative contribution is zero, and therefore they will
always be ignored.
Note that if the general member of $M$ is birational onto its image,
then $M$ is enumeratively relevant.

% do not contribue to the
% Gromov--Witten invariant corresponding to the space 
% $M_g^{\xi, \con} (\alpha,\beta)(\Omega)$,
% and therefore will always be discarded.


%\begin{subnum-par}
\begin{theorem}\label{t:acz}
Assume we are either in situation \ref{sp:mapsP^2} above,
or in situation \ref{sp:mapsF_1} and $\lambda >0$.
% or $k \leq 1$.
Let $M$ be an irreducible component of
$M_g^{\xi, \con} (\alpha,\beta)(\Omega)$.
The family of those curves in $S$ that are the image of a stable map
in $M$ has dimension at most
\[
  -(K_S+R) \cdot \xi +g-1 +|\beta|
  =
  \begin{cases}
    2d+g-1+|\beta|
    & \text{in situation \ref{sp:mapsP^2}}
    \\
    2\lambda + g-1+|\beta_E|+|\beta_H|    
    & \text{in situation \ref{sp:mapsF_1}}.
  \end{cases}
\]
The component $M$ is enumeratively relevant if and only if equality
holds, 
and in this case its general member $[ f:C \to S ]$
enjoys the following properties:
\begin{compactenum}
\item \label{it:smooth} the curve $C$ is smooth (hence irreducible);
\item \label{it:imm} $f$ is an immersion, birational onto its image;
\item \label{it:sm-inter} $f(C)$ intersects $R$ at smooth
points;
\item \label{it:avoids} for all finite subset $y \subset S$, if $f$ is
  general with 
  respect to $y$, then $f(C)$ does not intersect $y$.
\end{compactenum}
\end{theorem}


In situation \ref{sp:mapsP^2}, the statement on the dimension and 
birationality follow from
\cite[Prop.~\ttref{pr:charact}]{03.th-acz},
% NB
% the ref is to a label inside chapter 3-thomas.
and the rest from \cite[Thm.~\ttref{T}]{03.th-acz}.
In situation \ref{sp:mapsF_1} the proof is similar; the first part is
proven in 
\cite[Prop.~3.4]{vakil-07}, and the rest again follows from
\cite[Thm.~\ttref{T}]{03.th-acz}.




\paragraph{}
\label{t:acz'}
In the cases not covered by \ref{t:acz}, \ie in situation
\ref{sp:mapsF_1} when $\xi = kF$ ($k>0$),
let $M$ be an irreducible component of
$M_g^{kF, \con} (\alpha,\beta)(\Omega)$.
The family of those curves in $\F_1$ that are the image of a stable
map in $M$ has dimension $0$ or $1$, always less or equal than
\[
  -(K_S+R) \cdot \xi +g-1 +|\beta|
  = g-1+|\beta_E|+|\beta_H|,
\]
and $M$ is enumeratively relevant if and only if equality
holds.
The space $M_g^{kF, \con} (\alpha,\beta)(\Omega)$
has an enumeratively relevant irreducible component if and only if
$g=0$, and either
\[
  \alpha_E=\beta_H = [0,\ldots,0,1]
  \quad \text{and}
  \quad
  \beta_E =\alpha_H = 0
  \quad  \text{or viceversa},
\]
or
\[
  \beta_E=\beta_H = [0,\ldots,0,1]
  \quad \text{and}
  \quad
  \alpha_E =\alpha_H = 0.
\]
In those cases there is
a unique  enumeratively relevant component,
which parametrizes degree $k$ maps from $\P^1$ to a fibre $F$ of $\F_1$,
with total ramification over the two points $F \cap \Lambda_E$ and
$F \cap \Lambda_H$.

\par This is a consequence of the basic observation that a connected
member of the linear system $|kF|$ necessarily consists of one single
fibre $F$ with multiplicity $k$, hence is uniquely determined by its
passing through one single point $x_1 \in \F_1$.
% Thus an enumeratively relevant component of
% $M_g^{kF, \con} (\alpha,\beta)(\Omega)$ must have dimension at
% most $1$, which implies that $g=0$.
When $g>0$, irreducible components of
$M_g^{kF, \con} (\alpha,\beta)(\Omega)$ even have dimension strictly
larger than the expected $g-1+|\beta|$, which itself is already strictly
larger than the dimension of the corresponding families of curves in
$\F_1$. 

Note that condition \eqref{it:avoids} of Thm.~\ref{t:acz}
holds for an enumeratively relevant component of
$M_0^{kF, \con} (0,\beta)(\Omega)$.


% So if there exists
% $(f: C \to \F_1) \in M_g^{kF, \con} (\alpha,\beta)(\Omega,x)$,
% then
% \[\left\{\begin{aligned}
% &r = g -1 + |\beta_E| + |\beta_H| \leq 1 \\
% &|\alpha_E|, |\alpha_H|, |\beta_E|, |\beta_H| \leq 1 \\
% &|\alpha_E| + |\alpha_H| \leq 1.
% \end{aligned}\right.\]
% This implies that either $\alpha_E = \alpha_H = 0$, and then $r=g+1$
% hence $g=0$ and $r=1$, 
% or $|\alpha_E| + |\alpha_H| =1$, and then $|\beta_E| + |\beta_H| =1$,
% $g=0$, and $r=0$; the claim follows.

%\end{subnum-par}

\paragraph{Log-GW invariants}
In favourable circumstances
(see, \eg \cite[Subsec.~2.3]{vakil-07}),
and in particular in the situations we are concerned with in this text,
one may define the
\emph{logarithmic Gromov--Witten invariant} (log-GW invariant for
short)
of the pair $(S,R)$ in genus $g$ and class $\xi$, with boundary conditions
$(\alpha,\beta)$ as the length, for a general choice of a set $\Omega$
of $\alpha$ points on $R$ and of a set $x$ of
\[
  n= -(K_S+R) \cdot \xi +g-1 +|\beta|
\]
points on $S$, of the $0$-dimensional space
$M_g^{\xi, \con} (\alpha,\beta)(\Omega,x)$.
The moduli space $M_g^{\xi, \con} (\alpha,\beta)(\Omega)$ is
endowed with the structure of a stack, and each point
$[f:C \to S] \in 
M_g^{\xi, \con} (\alpha,\beta)(\Omega,x)$
should be counted with the multiplicity
\begin{equation*}
\mu(f,x) = \frac 1 {\Card\, (\Aut f)}
\prod _{1 \leq i \leq r} \Card f^{-1} (x_i).
\end{equation*}

\paragraph{}
\label{p:GWplane}
In situations \ref{sp:mapsP^2} and \ref{sp:mapsF_1}, it follows from
\ref{t:acz} and \ref{t:acz'} that the space
$M_g^{\xi, \con} (\alpha,\beta)(\Omega,x)$ is finite,
and only those enumeratively relevant components of
$M_g^{\xi, \con} (\alpha,\beta)(\Omega)$
contribute to the corresponding log-GW invariant.
It holds also true that
the cardinality of $M_g^{\xi, \con}
(\alpha,\beta)(\Omega,x)$ is independent of the choice of $\Omega$ and
$x$ (as long as they are general).
Moreover,
conditions \eqref{it:imm} and \eqref{it:sm-inter} in \ref{t:acz}
together imply that $\mu(f,x)=1$ for all
$[f:C \to S] \in 
M_g^{\xi, \con} (\alpha,\beta)(\Omega,x)$.
Correspondingly, in situation
\ref{sp:mapsP^2} say, there is a $1:1$ correspondence between
$M_g^{\xi, \con} (\alpha,\beta)(\Omega,x)$ and 
$V^{d, \irr}_g(\alpha,\beta)(\Omega)
\cap \bigcap _{1 \leq i \leq r} \orth {x_i}$, where $\orth {x_i}$ denotes the
hyperplane of $|\O_{\P^2}(d)|$ consisting of those divisors that
contain $x_i$, so that
\begin{equation*}
\sum _{f \in M_g^{\xi, \con} (\alpha,\beta)(\Omega,x)} \mu(f,x)
= N^{d,\irr}_g (\alpha,\beta).
\end{equation*}
A similar result holds in situation \ref{sp:mapsF_1} with $\lambda>0$,
see \cite{vakil-07}.


\paragraph{Enumeratively relevant components of dimension at most $1$}
\label{p:atmost1}
It will be useful in the proof of Proposition \ref{pr:erwan} to have
a list of the enumeratively relevant components of dimension at most
$1$ of $M_g^{\xi, \con} (\alpha,\beta)(\Omega)$ in situation
\ref{sp:mapsF_1}, \ie
for the ruled surface $\F_1$.
For such a component, we 
must have $\lambda \leq 1$. If $\lambda=0$, we are in the situation of
\ref{t:acz'}: enumerative relevance imposes $g=0$, and all
enumeratively relevant components have dimension at most $1$.
The corresponding log-GW invariants are computed in \ref{p:mult:kF}
below.
If $\lambda=1$, we must have $g=0$ and $\beta=0$.
Then the space $M_0^{H+kF,\irr}(\alpha,0)(\Omega)$ is isomorphic to the
sublinear system of $|H+kF|$ defined by the contact conditions imposed
at $\Omega$: indeed the arithmetic genus of
$H+kF$ is $0$, and the contact conditions at fixed points are linear.
Therefore for a general point $x \in \F_1$,
$M_0^{H+kF,\irr}(\alpha,0)(\Omega,x)$ has exactly one member, which
has multiplicity $1$.

Note moreover that in situation \ref{sp:mapsP^2},
\ie for the projective plane,
there is no enumeratively relevant components of
of dimension $0$ of $M_g^{\xi, \con} (\alpha,\beta)(\Omega)$,
as follows from similar considerations.


\paragraph{Multiplicity for multiple fibres}
\label{p:mult:kF}
Now let us compute the log-GW invariants in the cases considered in
\ref{t:acz'} above,
\ie we consider the spaces $M_0^{kF,\irr}(\alpha,\beta)$ for the pair
$(\F_1,\Lambda_E+\Lambda_H)$, and either
(a) $\alpha_E=\beta_H = [0,\ldots,0,1]$ and $\beta_E=\alpha_H=0$ (or
viceversa),
or (b) $\beta_E=\beta_H = [0,\ldots,0,1]$ and $\alpha_E=\alpha_H=0$.

In case (a) $\Omega$ consists of one point, and
$M_0^{kF,\irr}(\alpha,\beta)(\Omega)$ has a unique enumeratively
meaningful component, of dimension $0$,
and in case (b) $\Omega$ is empty, the unique enumeratively
meaningful component of
$M_0^{kF,\irr}(\alpha,\beta)$ has dimension $1$, hence one should
impose the passing through $1$ point $x$.
In either case there is a unique stable map to consider,
\ie $M_0^{kF,\irr}(\alpha,\beta)(\Omega)$ in case (a) and
$M_0^{kF,\irr}(\alpha,\beta)(x)$ in case (b) are supported on exactly
one point,
and this map is a degree $k$ cover of the form 
$z \in \P^1 \mapsto z^k \in \P^1$ where the target $\P^1$ identifies
with the relevant fibre of $\F_1$, and $f(0)$ and $f(\infty)$ are on
$\Lambda_E$ and $\Lambda_H$ respectively.
The automorphism group of this map is thus
isomorphic to $\Z / k\Z$.

On the other hand, there is no point $x$ in case (a), and the unique
point $x$ in case (b) has $k$ different points in its preimage by $f$.
Therefore the log-GW invariants are $\frac 1 k$ in case (a), and $1$
in case (b).



\section{Degeneration of $\P^2$ to a chain of ruled 
surfaces of maximal length}
\label{S:degen}


This section contains the heart of Brugallé's proof of the
Correspondence Theorem. We introduce the necessary degeneration of the
projective plane, and provide (in Proposition \ref{pr:erwan})
the description of the limit enumerative problem that will be encoded
in terms of floor diagrams in the next section.


\paragraph{Degeneration of the plane}
\label{p:degenP^2}
We shall construct a sequence $\pi_r : \cP_r \to \D$,
indexed by $r \in \N$, %$Z _{\geq 0}$,
of degenerations over the unit disk $\D$ 
of the projective plane together with a distinguished line,
with central fibre $\pi_r ^{-1} (0)$ a reduced chain of rational
surfaces 
\[
S_{r+1} \cup S_r \cup \cdots \cup S_1 \cup S_0
\]
with $S_{r+1} = \P^2$ and $S_i = \F_1$ for
$0 \leq i \leq r$:
for all $i=1,\ldots, r$, the surface 
$S_i$ intersects only $S_{i+1}$ and $S_{i-1}$, along
two smooth rational curves, respectively,
while $S_{r+1}$ intersects only $S_r$ and $S_0$ intersects only $S_1$,
along one smooth rational curve.
We set $\Lambda_{i} = S_i \cap S_{i-1}$ for all $i=1,\ldots,r+1$, and
require that it is
linearly equivalent to $H$ on $S_{i}$ and to $E$ on $S_{i-1}$.
%in the notation of \ref{p:notations-P2-F1}.
We require moreover that the limit as $t\in \D^*$ tends to $0$ of the
distinguished lines in the planes $\pi_r ^{-1} (t)$,
which we will denote by $R(t)$,
be a smooth rational curve
$\Lambda_0$ in $S_0$, linearly equivalent to $H$.

\begin{figbox}
\includegraphics[height=3.5cm]{degen-07.eps}
\captionof{figure}{The degeneration $\pi_r : \cP_r \to \D$,
  together with limit base points and tangency points along the
  boundary}
\label{fig:degen}
\end{figbox}

\par The construction is by induction on $r \geq 0$. To construct
$\cP_0$, consider the trivial family $\P^2 \times \D$ together with a
trivial family of lines $\Lambda \times \D$, and let 
$\epsilon_0 : \cP_0 \to \P^2 \times \D$ be the blow-up of $\Lambda
\times \{0\}$, the distinguished line in the central fibre, and let 
$\pi_0 := \pr_2 \circ \epsilon_0$; 
then $S_1 \cong \P^2$ is the proper transform of the initial central
plane $\P^2 \times \{0\}$,
$S_0 \cong \F_1$ is the exceptional divisor of $\epsilon_0$, and 
$\Lambda_0$ is the intersection with $S_0$ of the proper transform of
the initial family of lines $\Lambda \times \D$.
\par The inductive construction is pretty much identical. Assuming
$\pi_r: \cP_r \to \D$ is constructed, let $\epsilon_{r+1}: \cP_{r+1}
\to \cP_r$ be the blow-up of $\Lambda_0 \subset \cP_r$, and $\pi_{r+1}
:= \pi_r \circ \epsilon_{r+1}$. In $\cP_{r+1}$ the surface $S_0$ is
the exceptional divisor of $\epsilon_{r+1}$, and the curve $\Lambda_0$
is the central fibre of the proper transform of the family of lines in
$\cP_r$ (or equivalently of the proper transform by $\epsilon_0 \circ
\cdots \epsilon_{r+1}$ of the initial family of lines $\Lambda \times
\D$).
For $i=1,\ldots,r+2$, the surface $S_i$ in $\cP_{r+1}$ is the proper
transform of $S_{i-1}$ in $\cP_r$.


\paragraph{Degenerations of stable maps}
\label{p:degen-maps}
We now fix $d,g \in \Z _{\geq 0}$ and $\alpha,\beta \in \NN$ such that
$I\alpha + I\beta=d$, and a set $\Omega$ of $\alpha$ points on
$\Lambda$. We want to look at degenerations of the space
$M^{d,{\rm irr}}_g (\alpha, \beta)(\Omega,x)$
for the pair $(\P^2,\Lambda)$
as the projective plane degenerates as
in \ref{p:degenP^2} above,
for some specific degeneration of a set $x$ of $r=2d+g-1+|\beta|$
points, as follows.

We consider a set
$x=\{x_1,\ldots,x_r\}$ of sections of $\pi_r: \cP_r \to \D$ such that
for all $t\in \D^*$, the set $x(t)$ consists of $r$ general points in
the plane $\pi_r^{-1}(t)$,
and for $t=0$, $x(0)=\{x_1(0),\ldots,x_r(0)\}$
with $x_i(0)$ a general point of $S_i \subset
\pi_r^{-1}(0)$ for all $i \in \dlbrack 1, r \drbrack$.
We choose in addition a set $\Omega$ of $\alpha$ sections of
$\pi_r: \cP_r \to \D$,
such that for all $t\in \D$, $\Omega(t)$ is a set of $\alpha$ general
points on the line $R(t)$.

The points $x_1(0),\ldots,x_r(0)$ are indicated on
Figure~\ref{fig:degen}
(where they are simply indicated as $x_1,\ldots,x_r$ to lighten the
picture), as well as the points of $\Omega(0)$, indicated on the
picture as $\omega_{1,1}, \ldots, \omega_{1,\alpha_1}, \ldots,
\omega_{n,1}, \ldots, \omega_{n, \alpha_n}$.
Note that $S_{r+1}$, the proper transform of the central fibre of
$\P^2 \times \D$, does not support anything,
$S_i$ supports the base point $x_i(0)$ for all $i=1,\ldots,r$,
and $S_0$
supports all the fixed contact points on the boundary $\Lambda_0$.

\par We then let $M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$ be the limit
as $t \in \D^*$ tends to $0$ of the moduli spaces of stable maps
$M_g ^{d,\irr}(\alpha,\beta) (\Omega(t),x(t))$ for the pairs
$(\pi_r^{-1}(t), R(t))$.
It is a moduli space of stable maps
$f:C \to \pi_r^{-1}(0)$
satisfying the following conditions:
\begin{compactenum}
\item $C$ is a connected nodal curve of arithmetic genus $g$;
\item $f(C) \supset x(0)$;
\item $f(C)$ does not contain $\Lambda_0$, and there 
  exist $\alpha$ points $q _{i,j} \in C$,
  and $\beta$ points $r _{i,j} \in C$
  such that
\begin{equation*}
\bigl \{ \phi (q_{i,j}) \bigr\} = \Omega(0)
\qquad \text{and} \qquad
\phi^* \Lambda_0 = \sum _{1 \leq j \leq \alpha_i} i \, q_{i,j}
+ \sum _{1 \leq j \leq \beta_i} i\, r_{i,j};
\end{equation*}
\item\label{cond:match}
 if $p \in f^{-1}(S_{i+1} \cap S_i)$ does not lie on a component
  of $C$ which is entirely mapped to $S_{i+1} \cap S_i$, then it is a
  node of $C$, the intersection of two components $C'$ and $C''$
  mapped to $S_{i+1}$ and $S_i$ respectively, and appears with the
  same multiplicity $\mu_p$ in $(f|_{C'})^* \Lambda_{i+1}$ and
$(f|_{C''})^* \Lambda_{i+1}$.
\end{compactenum}
That such a limit of moduli spaces of stable maps indeed exists is a
highly non-trivial fact which is due to Jun Li,
see \cite{junli-degen,junli-notes}.


\bigskip
The following result is the core of the proof by
degeneration of the Correspondence Theorem \ref{t:corresp}.
\begin{proposition}[Brugallé]
\label{pr:erwan}
The moduli space
% space of those curves in $\pi_r^{-1}(0)$ that are the image of a
% stable map in
$M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$ (defined in
\ref{p:degen-maps} above) is finite, and depends on $(\Omega,x)$ only
by way of 
$(\Omega(0),x(0))$.
\par Let $\bigl[ f:C \to \pi_r^{-1}(0)\bigr] \in
M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$.
% and assume it is
% enumeratively relevant (see below).
Then all the irreducible components $C_1,\ldots,C_n$ of $C$ are smooth
rational curves,
none of them is entirely mapped to one of the curves $\Lambda_i$,
$0 \leq i \leq r +1$, and the following conditions hold after suitable
relabelling: 
\begin{compactenum}
\item\label{pr:erwan:floors}
 $C_1,\ldots,C_d$ are pairwise disjoint smooth rational curves,
and there exist
$1 \leq a_1 < \cdots < a_d \leq r$ such that for each $i \in \dlbrack
1, d \drbrack$ the curve $f(C_i)$ is a member of the linear system 
$|H+k_iF|$ on $S_{a_i}$ (for some nonnegative integer $k_i$) and passes
through the point $x_{a_i}(0) \in S_{a_i}$;
\item\label{pr:erwan:elev}
the remaining curves form $r-d$ pairwise disjoint 
chains of smooth rational curves
\[\bar C_j = C_{d+\ell_1+\cdots+\ell_{j-1} +1} \cup \cdots 
\cup C_{d+\ell_1+\cdots+\ell_{j-1} +\ell_j}\]
(\ie for all $1 \leq s<s' \leq \ell_j$, $C_{d+\ell_1+\cdots+\ell_{j-1}
  +s}$
and $C_{d+\ell_1+\cdots+\ell_{j-1} +s'}$ intersect if and only if
$s'=s+1$, and in that case transversally in exactly one point,
and $\bar C_j \cap \bar C_{j'}$ is empty if $j\neq j'$);
 there are integers $b_1,\ldots,b_{r-d} \in \dlbrack 0, r \drbrack$
and $\mu_1,\ldots,\mu_{r-d} \geq 1$ such that the divisor
$f_*( C_{d+\ell_1+\cdots+\ell_{j-1} +s})$, $1 \leq j \leq r-d$ and $1
\leq s \leq \ell_j$, belongs to the linear system
$|\mu_j F|$ on the ruled surface $S _{b_j +s-1}$;
for all $j=1,\ldots,r-d$, the chain $\bar C_j$
intersects exactly $1$ or $2$ curves among $C_1,\ldots,C_d$,
necessarily at points mapped to
$\Lambda_{r} \cup \cdots \cup \Lambda_1$ by $f$, and
$f(\bar C_j)$ passes through exactly one of the points in
$(\Omega(0),x(0))$.
\end{compactenum}
\end{proposition}

% \bigskip
% In the above statement,
% $\bigl[ f:C \to \pi_r^{-1}(0)\bigr] \in
% M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$ is
% \emph{enumeratively relevant} if
% the subspace of $M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$ of those
% stable maps $\bigl[ f':C' \to \pi_r^{-1}(0)\bigr]$ such that
% $f_*C = f'_* C'$ as cycles in $\pi_r^{-1}(0)$ has dimension $0$ at $[f]$.


\begin{example}
Depicted in Fig.~\ref{example1a} is an example of a source curve $C$
of a member $\bigl[ f:C \to \pi_7^{-1}(0) \bigr]$ of
$M^{3,\lim}_0 (0, [1,1])$,
together with its image by $f$ in Fig.~\ref{example1b}.
The circled numbers on Fig.~\ref{example1b} indicate that the
restrictions of $f$ to $C_4,C_5,C_6$ have degree $2$; the restrictions
to all other irreducible components of $C$ are birational.

The picture on $S_3$ means that 
$f(C_1)$ is the only curve in $S_3$: it is irreducible,
linearly equivalent to $H+2F$.%
\footnote
{the picture is slightly incorrect, as $f(C_1)$ should be unisecant to
all fibres of the ruling of $S_3$; we will only be able to fix this
when we use tropical representations of curves,
see \cite[Section \tref{S:trop-design}]{11.th-toric-trop}.
There is the same issue with the two curves linearly equivalent to $H$
on $S_6$ and $S_7$, respectively.}
On the other hand, there are two irreducible components of $f(C)$ in
$S_6$, linearly equivalent to $H$ and $F$, respectively.
Note that $f$ normalizes the one node indicated by a
square dot on $S_6$.
% Fig.~\ref{example1b}.

To help the reader get their way around, I indicated on
Fig.~\ref{example1a} one point in the pre-image of each element of
$x(0)$; there is only one point in $f^{-1}(x_i(0))$ if $i\neq
1$, but there are two points in $f^{-1}(x_1(0))$, both in $C_5$.
In this example one has
\begin{align*}
(a_1,a_2,a_3)& =(3,6,7)
& \bar C_1 &= C_4 \cup C_5 \cup C_6
& \bar C_3 &= C_{10} \cup C_{11} \\
(b_1,b_2,b_3,b_4) &= (0,0,4,4),
& \bar C_2 &= C_7 \cup C_8 \cup C_9
& \bar C_4 &= C_{12} \cup C_{13} \cup C_{14}.
\end{align*}

\begin{subnum-fig}
\begin{figbox}
% \textwidth = 415pt = 14,59cm
\includegraphics[height=3cm]{example1a.eps}
\captionof{figure}{Source curve of a member of
$M^{3,{\rm irr}}_0 (0, [1,1])(x(0))$}
\label{example1a}
\end{figbox}

\begin{figbox}
\includegraphics[height=3.5cm]{example1b.eps}
\captionof{figure}{Image in $\pi_7^{-1}(0)$}
\label{example1b}

\end{figbox}
\end{subnum-fig}
\end{example}

% The rest of this Section is devoted to the proof of
% Proposition~\ref{pr:erwan}.
\paragraph{Proof of Proposition~\ref{pr:erwan}}
Let $\bigl[ f:C \to \pi_r^{-1}(0)\bigr] \in
M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$.
The fact that no component of $C$ is entirely mapped to one of the
curves $\Lambda_i$ follows from
\cite[Example 11.4 and Lemma 14.6]{ionel-parker},
and we will take it for granted.
The other assertions essentially follow from a series of dimension
counts, which are now going to expound.

Let $C_1,\ldots,C_n$ be the irreducible components of $C$.
For all $j=1,\ldots,n$, we let
$f_j: C_j \to S_{s(j)}$ be the restriction of $f$ to $C_j$,
$g_j$ the arithmetic genus of $C_j$,
$\xi_j$ the linear equivalence class of $f_*(C_j)$ on
the surface $S_{s(j)}$
(note that a priori $\xi_j$ may vanish, in case $C_j$ is contracted),
$\zeta_j \in \{0,1\}$ the number of points in $x(0)$
contained in
$f_j(C_j)$,
and $\beta_j^E,\beta_j^H \in \NN$ the types of contact of $f_j(C_j)$
with $\Lambda_{s(j)+1}$ and $\Lambda_{s(j)}$ respectively, pretending
that all contacts are at unassigned points. Thus
\[
  \bigl[ f_j \bigr] \in
  M _{g_j} ^{\xi_j, \irr} (0,0,\beta_j^E,\beta_j^H)
\]
as a moduli space of stable maps to $S_{s(j)}$
with boundary $R=\Lambda_{s(j)} \coprod \Lambda_{s(j)+1}$,
where the set $\Omega$
is empty, and where we choose to forget the datum of the possible
point of $x(0)$ contained in $f(C_j)$.
(This all comes with a harmless abuse of notation in case $s(j)=r+1$;
in fact we shall see that this case never occurs).

Then we consider $M_j \subset M _{g_j} ^{\xi_j, \irr}
(0,0,\beta_j^E,\beta_j^H)$ the smallest irreducible subvariety in
which $[f_j]$ 
moves as we let $x$ vary, maintaining the requirements of
\ref{p:degen-maps}.
We let $\CM_j$ be the corresponding family of curves in $S_{s(j)}$.
By generality of the point $x_{s(j)}(0)$ in  $S_{s(j)}$,
we must have $\dim(\CM_j) \geq \zeta_j$; let
$\epsilon_j = \dim(\CM_j) - \zeta_j$.
By Theorem~\ref{t:acz} and Paragraph \ref{t:acz'} we also have:
\begin{equation}
\label{eq:5.1.1}
\zeta_j
\leq
\dim(\CM_j)=\zeta_j + \epsilon_j
\leq
2F\cdot \xi_j +g_j -1 + |\beta_j^E| + |\beta_j^F|.
\end{equation}

On the other hand, the various $f(C_j)$'s are subject to matching
conditions at the boundary of the various $S_{s(j)}$,
in order for condition \eqref{cond:match} of
\ref{p:degen-maps} to hold.
(A priori there may be other matching conditions if the $C_j$'s
intersect at points mapped off $\Lambda_{r+1}\cup \cdots \cup
\Lambda_1$ by $f$,
but we don't need to consider them for the moment; we shall see that
in fact this does not happen).
These matching conditions are in the number of
\[
  a= \Card \bigl( f^{-1}(\Lambda_{r+1}\cup \cdots \cup \Lambda_1 )
  \bigr),
\]
and they are independent by Theorem~\ref{t:acz}, \ref{t:acz'},
and \cite{03.th-acz}: consider some curve $f(C_{j_0})$, and assume all
the other components $f(C_j)$ are fixed; then the matching conditions
imposed to $f(C_{j_0})$ amount to turn some of the contact conditions
$\beta_j^E,\beta_j^H$ at unassigned points to contact conditions at
assigned points,
and it follows from \cite[\ttref{P0}]{03.th-acz} that each assigned
contact point makes the dimension drop by $1$.
Note that the assigned contact points may not be in general position;
fortunately this does not cause any trouble, as we have observed in
\cite{03.th-acz}.

Lastly, the assigned contact points $\Omega(0)$ on $\Lambda_0$
impose $|\alpha|$ further conditions, independent from all the rest
for the same reasons as before.
Therefore, if we let $\CM$ be
the smallest irreducible variety in which $f(C)$ moves as we let $x$
vary, then $\CM$ has codimension at least $a+|\alpha|$ in
$\prod_j \CM_j$.

In the upshot, we must have:
\begin{equation}
\label{eq:5.1.2}
 \tsum_j \dim (CM_j)
\geq
\bigl( \tsum_j \zeta_j \bigr) + a + |\alpha|
= r+a+|\alpha|.
\end{equation}
On the other hand, summing the inequalities \eqref{eq:5.1.1} for all
$j=1,\ldots,n$, we get 
{\addtolength{\multlinegap}{1cm}
\begin{multline}
\label{eq:5.1.3}
  \sum_j \dim (\CM_j) \leq 
  \sum_j \Bigl(
  2F\cdot \xi_j +g_j -1 + |\beta_j^E| + |\beta_j^F|
  \Bigr)
  \\
  \stackrel{\star}=
  2d+g-1+|\beta|+|\alpha|+a-a'
  =r+|\alpha|+a-a',
\end{multline}
}%
where $a'$ is the number of intersection points of the $C_j$'s mapped off
$\Lambda_{r+1}\cup \cdots \cup \Lambda_1$ by $f$;
equality $(\star)$ is given by the three relations of
Lemma \ref{l:relazioni} below.
Comparing with \eqref{eq:5.1.2}, we get that
\[
  a'=0
  \quad \text{and}
  \quad
  \tsum_j \dim (\CM_j) = r+|\alpha|+a,
\]
which in particular implies that the family of curves corresponding to 
$M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$
is finite and depends only on
$(\Omega(0),x(0))$.

The inequalities \eqref{eq:5.1.2} and \eqref{eq:5.1.3} also imply that
for all $j=1,\ldots,n$ one has
\begin{equation}
\label{eq:5.1.4}
  \dim(\CM_j) = \zeta_j+\epsilon_j
  = 2F\cdot \xi_j +g_j -1 + |\beta_j^E| + |\beta_j^F|,
\end{equation}
and moreover 
$  \tsum_j \epsilon_j = |\alpha|+a$.
By Theorem \ref{t:acz} and \ref{t:acz'}, Equation \eqref{eq:5.1.4}
implies that each $M_j$ is an enumeratively relevant irreducible
component of
$M _{g_j} ^{\xi_j, \irr} (0,0,\beta_j^E,\beta_j^H)$.
In particular, the finiteness of the family of curves
in $\bigcup_j S_j$ corresponding to 
$M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$ implies the finiteness
of $M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$ itself.

These finiteness results imply that for all $j$, if we fix the
intersection points of $f(C_j)$ with $\Lambda_{s(j)+1}$ and
$\Lambda_{s(j)}$ (again with a slight abuse of notation if
$s(j)=r+1$), then $[f_j]$ moves in dimension at most $\zeta_j$.
By \ref{p:atmost1}, this implies that for all $j$ one has $g_j=0$,
$s(j)<r+1$, and
\[
  \xi_j =
  \begin{cases}
    k_jF & \text{if}\ \zeta_j=0 \\
    k_jF \ \text{or}\ H+k_jF & \text{if}\ \zeta_j=1.
  \end{cases}
\]
% $\xi_j=k_jF$ if $\zeta_j=0$, or
% $\xi_j$ equals either $k_jF$ or $H+k_jF$ if $\zeta_j=1$.
By relation \eqref{rel:degree} below,
there are exactly $d$ indices $j$ such that $\xi_j$ is of the form
$H+k_jF$ and, relabelling if necessary, we will assume that they are
$j=1,\ldots,d$.
Then, the indices $s(1),\ldots,s(d)$ are pairwise distinct and in the
interval 
$\dlbrack 1, r \drbrack$, because there is only one point of $x(0)$ on
each of $S_1,\ldots,S_r$.

Condition \eqref{cond:match} of \ref{p:degen-maps} imposes that the
curves $C_{d+1},\ldots,C_n$ (\ie those $C_j$ such that $\xi_j=k_j F$)
organize in chains of fibres of
the same multiplicity as stated in Proposition \ref{pr:erwan}.
The vanishing of
$a'$ imposes that each chain meets exactly one or two among
$C_1,\ldots,C_d$, at points mapped to $\Lambda_{r+1}\cup \cdots \cup
\Lambda_1$. The finiteness results above imply that each chain must
pass through exactly one point of $(\Omega(0),x(0))$.

It remains to show that two curves among $C_1,\ldots,C_d$ cannot
intersect each other. Assume by contradiction that $f(C_1)\subset
S_1$, $f(C_2) \subset S_2$, and $C_1$ and $C_2$ intersect at a point
mapped to $y\in S_1\cap S_2 = \Lambda_2$. Then we would find a
$1$-dimensional family of stable maps in $M^{d,\lim}_g (\alpha,
\beta)(\Omega,x)$ by letting $y$ move along $\Lambda_2$, a
contradiction.
This ends the proof of Proposition \ref{pr:erwan}.
\qed


\begin{lemma}
\label{l:relazioni}
In the above notation, we have the following relations:
\begin{gather}
\label{rel:bndary}
  \tsum _j \bigl(
  |\beta_j^E| + |\beta_j^H|
  \bigr) = 2a + |\alpha| + |\beta|;
  \\
\label{rel:pa}
  g = \bigl( \tsum_j g_j \bigr) +1-n+a+a'.
  \\
\label{rel:degree}
  \tsum _j (\xi_j\cdot F)_{S_{s(j)}} = d;
\end{gather}
\end{lemma}

% \begin{lemma}
% \subparagraph{}
% $  \sum _j \bigl(
%   |\beta_j^E| + |\beta_j^F|
%   \bigr) = 2a + |\alpha| + |\beta|;$
% \subparagraph{}
% $  \sum _j (\xi_j\cdot F)_{S_{s(j)}} = d;$
% \subparagraph{}
% $  g = \bigl( \tsum_j g_j \bigr) +1-n+a$.
% \end{lemma}

\begin{proof}
The points corresponding to those $\beta_j^E$ such that $0\leq s(j)
\leq r$, and equally those corresponding to those $\beta_j^H$ such
that $1 \leq s(j) \leq r+1$,
are exactly the points in the singular locus of
$\pi_r ^{-1}(0)$ at which the matching conditions referred to in the
proof of Proposition \ref{pr:erwan} above happen, which are in the
number $a$. Each such point is counted twice, once in some number
$\beta_{s(j)}^E$, and once in the corresponding number
$\beta_{s(j)+1}^H$.
On the other hand, those $\beta_j^H$ such that $s(j)=0$ sum up as the
number of points in $\Omega(0)$, which is $|\alpha| + |\beta|$.
This proves \eqref{rel:bndary}.

Relation \eqref{rel:pa} is the expression of the arithmetic genus of
the nodal curve $C$, which has $n$ irreducible components
$C_1\ldots,C_n$ of respective genera $g_1,\ldots,g_n$, and
$a+a'$ nodes, where $a'$ is the number of intersection points among
the $C_j$'s that are mapped off
$\Lambda_{r+1}\cup \cdots \cup \Lambda_1$ by $f$.

Relation \eqref{rel:degree} comes with an abuse of notation, namely
that for those $j$ such that $s(j)=r+1$, $F$ should be replaced by $H$.
Then the curve class on the limit surface $\pi_r ^{-1}(0)$ consisting
of the class $F$ on all $S_i$, $i=0,\ldots,r+1$
(which thus has to be taken as $F$ on all $S_i$, $i=0,\ldots,r$, and
$H$ on $S_{r+1}$), is a limit of the class $H$ on the projective planes
$\pi_r ^{-1}(t)$ as $t \in \D^*$ tends to $0\in \D$.
Relation \eqref{rel:degree} is then a consequence of the fact that
$\bigl[ f:C \to \pi_r^{-1}(0)\bigr] \in
M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$ is a limit of stable maps
realizing the curve class $dH$ on
the projective planes $\pi_r ^{-1}(t)$, $t \in \D^*$.
See also \ref{p:twists} for another point of view on this argument.
\end{proof}


\bigskip
Proposition \ref{pr:erwan} has the following corollary, which we will
translate in Section \ref{S:combin} below as saying that the number of
plane curves $N_g ^{d,\irr}(\alpha, \beta)$ may be computed by
enumerating floor diagrams.

\begin{corollary}
\label{cor:junli}
In the notation of \ref{p:degenP^2} to  \ref{pr:erwan},
one has
\begin{equation*}
  N_g ^{d,\irr}(\alpha, \beta) =
  \sum _
  { [ f:C \to \pi_r^{-1}(0) ] \in
    M^{d,\lim}_g (\alpha, \beta)(\Omega,x)}
  \mu(f)
\end{equation*}
where $\mu(f)$ is defined as
\begin{equation*}
  \mu(f) =
  \raisebox{-.2em}{$\biggl($}
  \prod _{p \in f^{-1} (\Lambda_{r+1}\cup \cdots \cup \Lambda_1)} \mu_p
  \raisebox{-.2em}{$\biggr)$}
  \raisebox{-.2em}{$\biggl($}
  \prod _{p \in x(0)} \Card f^{-1}(p)
  \raisebox{-.2em}{$\biggr)$}
  \raisebox{-.2em}{$\biggl($}
  \prod _{1 \leq j \leq n} \Card(\Aut( \restr f {C_j}))
  \raisebox{-.2em}{$\biggr)$}
  ^{-1}
\end{equation*}
(recall in particular the definition of $\mu_p$ in Condition
\eqref{cond:match} of \ref{p:degen-maps}).
\end{corollary}


\begin{proof}
By Proposition \ref{pr:erwan} and Jun Li's Formula,
see \cite{junli-degen,junli-notes}, for all $t\in \D^*$, one has
\begin{equation*}
\sum _{f \in M_g^{\xi, {\irr}} (\alpha,\beta)(\Omega(t),x(t))} \mu(f,x(t))
= \sum _
  { [ f:C \to \pi_r^{-1}(0) ] \in
    M^{d,\lim}_g (\alpha, \beta)(\Omega,x)}
  \mu(f).
%= N^{d,{\rm irr}}_g (\alpha,\beta).
\end{equation*}
The result follows, since the left-hand-side of the equation above
equals $N^{d,{\rm irr}}_g (\alpha,\beta)$,
as we have seen in \ref{p:GWplane}.
\end{proof}


\paragraph{}
\label{p:mult-junli}
It will be useful to have a ready-to-use expression for the
multiplicity $\mu(f)$ of a stable map
$[f] \in M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$ as in Proposition
\ref{pr:erwan}.
Only the chains of multiple fibers $\bar C_1,\ldots, \bar C_{r-d}$ may
contribute non-trivially to the multiplicity $\mu(f)$,
and their respective contributions may be computed in a similar way as
in \ref{p:mult:kF}.

Let $\bar C_j$
be such a chain, with multiplicity $\mu_j$ and length $\ell _j$ (the
number of its irreducible components).
% , and $\zeta_j$ the number of
% points from $x(0)$ through which $f(\bar C_j)$ passes (this is $0$ or
% $1$).
There are the following three cases:
\begin{mycpctenum}[(a)]
\item\label{case:finite}
no irreducible components of $\bar C_j$ is mapped to $S_0$: then
$f(\bar C_j)$ passes through exactly one point $p$ of $x(0)$,
for which $f^{-1}(p)$ has cardinality $\mu_j$,
there are $\ell_j+1$ points $p \in f^{-1} (\Lambda_{r+1}\cup \cdots
\cup \Lambda_1)$ lying on $\bar C_j$, all with multiplicity $\mu_p =
\mu_j$, and 
for each irreducible component of $\bar C_j$, there is an automorphism
group of cardinality $\mu_j$. Thus the contribution of the chain $\bar
C_j$ to the multiplicity $\mu(f)$ is
\[
  \mu_j ^{\ell_j +1} \cdot
  \mu_j \cdot
  \mu_j^{-\ell_j}
  = \mu_j ^2;
\]
\item\label{case:infbeta}
  there is an irreducible components of $\bar C_j$ mapped to
  $S_0$, and
  $f(\bar C_j)$ passes through exactly one point $p$ of $x(0)$
  and no point of $\Omega(0)$:
  then there are only $\ell_j$ points $p \in f^{-1} (\Lambda_{r+1}\cup \cdots
\cup \Lambda_1)$ lying on $\bar C_j$, but otherwise the situation is
the same as in case \eqref{case:finite}.
The contribution of the chain $\bar
C_j$ to the multiplicity $\mu(f)$ is thus
\[
  \mu_j ^{\ell_j} \cdot
  \mu_j \cdot
  \mu_j^{-\ell_j}
  = \mu_j;
\]
\item there is an irreducible components of $\bar C_j$ mapped to
  $S_0$, and
  $f(\bar C_j)$ passes through exactly one point $p$ of $\Omega(0)$
  and no point of $x(0)$:
  then there are $\ell_j$ points $p \in f^{-1} (\Lambda_{r+1}\cup \cdots
\cup \Lambda_1)$ lying on $\bar C_j$ as in case \eqref{case:infbeta},
but
now there is no point $p \in x(0)$ contributing to the multiplicity.
The contribution of the chain $\bar
C_j$ to the multiplicity $\mu(f)$ is thus
\[
  \mu_j ^{\ell_j} \cdot
  1 \cdot
  \mu_j^{-\ell_j}
  = 1.
\]
\end{mycpctenum}



\section{Combinatorial translation}
\label{S:combin}

We are now ready to give the proof of \cite{erwan} of the
Correspondence Theorem \ref{t:corresp}.
In fact, most of the work has already been done in
Section~\ref{S:degen}, and it only remains to interpret Proposition
\ref{pr:erwan} and Corollary \ref{cor:junli} in terms of floor
diagrams. 


\paragraph{Proof of the Correspondence Theorem \ref{t:corresp}}
\label{p:corresp_diag-curve}
We associate each stable map
$[ f:C \to \pi_r^{-1}(0)] \in M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$
as in Proposition \ref{pr:erwan} with a marked floor diagram of genus
$g$, degree $d$, and type $(\alpha, \beta)$ as follows.

We first identify the vertices. To each irreducible component $C_i$ of
$C$ such that $f_* C_i = H+kF$ on some $S_{s(i)}$ we associate a
floor, and to each point in $f(C) \cap \Lambda_0$ we associate a vertex at
infinity. We provide the vertices with an ordering, which in turn will
determine the orientation of the edges: each vertex $v$
corresponds to an object lying on a unique ruled surface
$S_{s(v)}$, and for all vertices $v$ and $v'$, we declare that $v$
precedes $v'$ if $s(v) \leq
s(v')$.

Now let us define the edges: they are in bijective correspondence with the
chains $\bar C_j$ described in \eqref{pr:erwan:elev} of Proposition
\ref{pr:erwan}, and the weight of the edge corresponding to $\bar C_j$
is the positive integer $\mu_j$.
The edge corresponding to $\bar C_j$ is adjacent to
the floor corresponding to $C_i$ (resp.\ the vertex at infinity
corresponding to $p\in \Lambda_0$) if $\bar C_j$ and $C_i$ intersect
at a point (resp.\ if $f(\bar C_j)$ passes through $p$).

It follows from Proposition \ref{pr:erwan} that the object constructed
so far is a floor diagram $\diag$ of genus $g$ and degree $d$,
and the corresponding set
$\orient =\vt ^{\rm fin} \coprod \edg$ is in bijection with
$\Omega(0) \coprod x(0)$. The set $x(0)$ naturally comes with a
bijection with $\intint 1 r$ (remember that each $x_i(0)$ lies on the
surface $S_i$). By appropriately labelling the points in $\Omega(0)$
with indices in $\intint {-|\alpha|+1} 0$, we obtain a marking of
$\diag$ of type $(\alpha,\beta)$. There are several possible ways of
labelling the points in $\Omega(0)$, but they are equivalent up to
automorphisms of the marked floor diagram.

Conversely, from any marked floor diagram of type $(\alpha,\beta)$ one
can construct a stable map as in Proposition \ref{pr:erwan}, and this
is a point in
$[ f:C \to \pi_r^{-1}(0)] \in M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$.
It only remains to observe that the multiplicity of the map
$[ f:C \to \pi_r^{-1}(0)] \in M^{d,\lim}_g (\alpha, \beta)(\Omega,x)$
in the formula of Corollary \ref{cor:junli} equals that of the
corresponding floor diagram, which follows from \ref{p:mult-junli}
and Definition \ref{d:mult-floor}.
\endproof


\begin{example}
I shall now illustrate the correspondence
of \ref{p:corresp_diag-curve}
between floor diagrams and limit curves on various examples
pertaining to plane cubic curves. I will only consider curves with
trivial boundary conditions, \ie $(\alpha,\beta)=(0,3)$, so
nothing relevant happens on $S_0$ (and on $S_{r+1}$ either, as
always),
and thus I
will only represent the $S_i$'s for $i=1,\ldots,r$.

Under each ruled surface $S_i$, I have indicated the total curve class
supported on this component, \ie the sum of the $\xi_j=f_*C_j$ for all
$j$ such that $C_j$ is mapped to $S_i$. The limit base points
$x_1(0),\ldots,x_r(0)$ on $S_1,\ldots,S_r$ respectively are indicated
by black disks.

Note that (obviously, I hope) to obtain a proper graphic
correspondence between our representations of floor diagrams and limit
curves, the diagrams should be rotated by $+ \frac \pi 2$.

\smallskip
\subparagraph{Limit of a smooth cubic}
Below is displayed the limit curve of a smooth cubic, corresponding to
the unique possible marked floor diagram of degree $3$ and genus $1$
(and type $(0,3)$).
The two curves in $S_7$ and $S_4$ are irreducible. Later on
(in Lecture \cite{11.th-toric-trop}) we will have a
better way of representing these curves, coming from tropical geometry.

\begin{figbox}
\includegraphics[align=c,scale=1.3]{d3g1-marquee.eps}
\hspace{8mm}
\includegraphics[align=c,height=30mm]{cubique-lisse.eps}
\captionof{figure}{Limit of a smooth cubic}
\end{figbox}


\smallskip
\subparagraph{Various limits of rational cubics}
\label{ex:rat-cubics}
Below I display limit curves corresponding to the various diagrams of
degree $3$ and genus $0$ (and type $(0,3)$),
see  Example \ref{p:d3g0-plain}. For the diagram shape at the center
of Figure~\ref{fig:d3g0-plain}, I consider two different markings
(Figures \ref{fig:d3g0-bi} and \ref{fig:d3g0-bii} below), so
that one can better see what is encoded in the marking.

On Figure~\ref{fig:d3g0-a}, the two curves in $S_6$ and $S_4$ are
irreducible, and tangent to $S_6\cap S_5$ and $S_5 \cap S_4$
respectively; the curve on $S_5$ is a fibre with multiplicity $2$.
\begin{figbox}
\includegraphics[align=c,scale=1.3]{d3g0-3a.eps}
\hspace{8mm}
\includegraphics[align=c,height=30mm]{cubique-a.eps}
\captionof{figure}{Limit of rational cubics (a)}
\label{fig:d3g0-a}
\end{figbox}

On Figure~\ref{fig:d3g0-bi}, the curve in $S_6$ is irreducible, and
that in $S_4$ has two components of classes $H+F$ and $F$ respectively,
which intersect at one point represented by a full black square. On
Figure~\ref{fig:d3g0-bii} the situation is similar.
\begin{figbox}
\includegraphics[align=c,scale=1.3]{d3g0-3bi.eps}
\hspace{8mm}
\includegraphics[align=c,height=30mm]{cubique-bi.eps}
\captionof{figure}{Limit of rational cubics (b)}
\label{fig:d3g0-bi}
\end{figbox}

\begin{figbox}
\includegraphics[align=c,scale=1.3]{d3g0-3bii.eps}
\hspace{8mm}
\includegraphics[align=c,height=30mm]{cubique-bii.eps}
\captionof{figure}{Limit of rational cubics (b')}
\label{fig:d3g0-bii}
\end{figbox}

On Figure~\ref{fig:d3g0-c}, the curve in $S_4$ is irreducible, and
that in $S_7$ has two components of classes $H$ and $F$ respectively,
which intersect at one point represented by a black square.

\begin{figbox}
\includegraphics[align=c,scale=1.3]{d3g0-3ci.eps}
\hspace{8mm}
\includegraphics[align=c,height=30mm]{cubique-ci.eps}
\captionof{figure}{Limit of rational cubics (c)}
\label{fig:d3g0-c}
\end{figbox}

I have tried to maintain the black dots representing the points of
$x(0)$ in the series of Figures \ref{fig:d3g0-a}--\ref{fig:d3g0-c} at
a fixed position. I have only cheated a little bit on
Figure \ref{fig:d3g0-c}, on which I have moved the base point on
$S_7$, for otherwise the picture was outrageously unclear.
\end{example}


\section{Projective geometric interpretation}
\label{S:ourway-07}

In this section, I propose a formulation of the degenerations of stable
maps considered in this lecture in terms of degenerations of nodal
curves,
in the framework of the theory expound
in \cite{01.ciro}.
%  as exposed in Lecture \tmpref{ciro}.
% {\blue Verify with terminology introduced by Ciro.}


\paragraph{Twists}
\label{p:twists}
Let us consider the degeneration
$\pi_r: \cP_r \to \D$ of the projective plane introduced in
\ref{p:degenP^2}. It comes with a map
$\bar \epsilon_r: \cP_r \to \cP := \P^2 \times \D$ which is the
composition of blow-ups
$\bar \epsilon_r = \epsilon_r \, \cdots \, \epsilon_0$.
Consider the line bundle
\begin{equation*}
  \L_{r,d} = \bar \epsilon_r^* \, \pr_1^* \bigl( \O_{\P^2}(d) \bigr);
\end{equation*}
it restricts to $\O_{\P^2}(d)$ on the fibres $\pi_r^{-1}(t)$, $t\in
\D^*$, and thus its restriction to the central fibre $\pi_r^{-1}(0)$
defines a possible linear system for the linear system of plane degree
$d$ curves to degenerate to within the degeneration $\pi_r: \cP_r \to \D$.
In this paragraph I will describe the various \emph{twists}
$\L_{r,d}(-W)$ that have the same property: the requirements are that
$W$ is an effective divisor of $\cP_r$ supported on the central fibre,
such that the restriction $\restr {\L_{r,d}(-W)} {\pi_r^{-1}(0)}$
defines a linear system on the central fibre that has the same
dimension as 
$|\O_{\P^2}(d)|$.

It is elementary to prove that these twists all have the form
\begin{equation*}
  \L_{r,d}\bigl( -\tsum _{i=0} ^r m_i \bar S_i \bigr),
\end{equation*}
where $\bar S_i = \sum _{i' \leq i} S_{i'}$, and the $m_i$'s are
non-negative integers subject to the inequalities
\begin{equation*}
  d \geq m_r \geq \cdots \geq m_0.
\end{equation*}
As a sideremark, note that this gives an alternative way of proving
the relation \eqref{rel:degree}.
Since $\L_{r,d}$ restricts to $dH$ on $S_{r+1}$ and to $dF$ on the
other $S_i$'s, the line bundle
$\L_{r,d}\bigl( -\tsum _{i=0} ^r m_i \bar S_i \bigr)$
restricts to the following linear equivalence classes on the various
irreducible components of the central fibre of $\pi_r$:
\begin{compactitem}
\item on $S_{r+1}$: $(d-m_r)H$;
\item on $S_{i}$, $0<i\leq r$: $dF+m_iE-m_{i-1}H=(m_i-m_{i-1})H+(d-m_i)F$;
\item on $S_0$: $dF+m_0 =m_0H+(d-m_0)F$.
\end{compactitem}

Now, the choice of the limiting positions of the base points that has
been made in \ref{p:degen-maps},
\ie the choice that $x_i(0)$ lies on $S_i$ for all $i=1,\ldots,r$,
implies that the twists that are relevant for the enumeration of limit
curves are subject to the further restrictions:
\begin{equation*}
  m_r=d;
  \quad
  m_0=0;
  \quad
  m_i-m_{i-1} \leq 1
  \quad \text{for all } i=r,\ldots,1.
\end{equation*}
This corresponds to the fact that the classes $\xi_j$, in the notation
of Proposition \ref{pr:erwan}, are necessarily of the form
$H+k_jF$ or $k_jF$.

\medskip
\subparagraph{Example}
The twist giving the limiting linear system in which the curve
represented on Figure~\ref{example1b} lives is the following:
\[
  \L_{7,3}\bigl(
  -3\bar S_7
  -2\bar S_6
  -\bar S_5
  -\bar S_4
  -\bar S_5
  \bigr).
\]


\paragraph{Projective models of the degeneration}
I now describe the projective model of the degeneration
$\pi_r: \cP_r \to \D$ given by a twist which is relevant for the
enumeration of limit curves with the limit base points as in
\ref{p:degen-maps}.

By what we have seen above, such a twist
gives the classes
$H,H+F,\ldots,H+(d-1)F$ respectively on the ruled surfaces
$S_{r_0},S_{r_1},\ldots,S_{r_{d-1}}$,
with $r =r_0 > r_1 > \cdots > r_{d-1}$, and multiples of the class $F$
on the other ruled surfaces
(specifically, it gives the class $kF$ on the surfaces $S_i$ for
$r_{k-1} > i > r_k$, for all $k=1,\ldots,d$, setting $r_{-1}=r+2$ and
$r_d=-1$ for convenience, and with the abuse of considering $S_{r+1}$
as a ruled surface).

It follows that the restriction of such a twist to the central fibre
maps $S_{r_0},S_{r_1},\ldots,S_{r_{d-1}}$ to rational normal scrolls
of types
$\Sigma(0,1),\Sigma(1,2),\ldots,\Sigma(d-1,d)$ respectively,
and contracts all the other irreducible components to rational normal
curves
(with the notation that a rational normal scroll of type
$\Sigma(k_1,k_2)$ is 
built on two rational normal curves of degrees $k_1$ and $k_2$
which span two supplementary linear spaces). Two
successive scrolls $\Sigma(k,k+1)$ and $\Sigma(k+1,k+2)$ in the
previous list are glued along the rational normal degree $k+1$ curves
$\Lambda_{r_k}$ and $\Lambda_{r_{k+1}-1}$.

The upshot is that the restriction to the fibres of $\pi_r: \cP_r \to
\D$ of the twist of $\L_{r,d}$ under consideration gives a
degeneration of the $d$-th Veronese image of $\P^2$ to a chain of
rational normal scrolls. Correspondingly, we see limits of plane
degree $d$ curves as hyperplane sections of this chain of rational
normal scrolls.

As a sanity check, let us verify that the degrees and embedding
dimension of such a projective model are correct.
The total degree is
\begin{equation*}
  \sum _{k=0} ^{d-1} \deg \bigl( \Sigma(k,k+1) \bigr)
  = \sum _{k=0} ^{d-1} (2k+1)
  = d^2,
\end{equation*}
and the dimension of the projective linear space spanned by our chain
of scrolls is
\begin{equation*}
  \sum _{k=0} ^{d-1} h^0(\O_{\P^1}(k+1))
  = \sum _{k=0} ^{d-1} (k+2)
  = 2d + \sum _{k=1} ^{d-1} k
  = \sum _{k=1} ^{d+1} k-1,
\end{equation*}
which indeed coincide respectively to the degree and embedding
dimension of $d$-th Veronese image of $\P^2$.

We will be able to give a nice graphic representation of this
degeneration of the 
$d$-th Veronese to a chain of rational normal scrolls when we know
some toric and tropical geometry, see
\cite[\tref{p:trop-erwan}]{11.th-toric-trop}. 


\paragraph{Limits of nodes}
\label{p:lim-nodes}
It is a central theme of this set of notes
(in particular, see \cite[\ttref{s:Severi-1}]{01.ciro})
that the limit of a node
may be of the two following types.
\begin{inparaenum}[(a)]

\item It may be a node on one of the irreducible components of the
degeneration.
In our situation the irreducible components of the central fibre are
rational normal scrolls, so the only way a hyperplane section has a
node is that it splits off a fibre.

This is indeed what we have observed in the previous examples. See in
particular \ref{ex:rat-cubics}: nodes as above are indicated by a
black square. There is such a node on Figures \ref{fig:d3g0-bi},
\ref{fig:d3g0-bii}, and \ref{fig:d3g0-c}.

\item It may be a tacnode along the transverse intersection curve of
two irreducible components of the central fibre
(or, more generally, $\mu-1$ nodes may degenerate together to a
$\mu$-tacnode).
In our situation in this lecture, this phenomenon occurs when two
curves of respective classes $H+kF$ and $H+(k+1)F$ are linked by a
chain of fibres of multiplicity $\mu$.

This happens for instance on Figure~\ref{fig:d3g0-a}. In the
projective model given by the appropriate twist for the curve
displayed on Figure~\ref{fig:d3g0-a}, $S_5$ is contracted to a conic,
and the two scrolls images of $S_6$ and $S_4$ intersect along this
conic; the two curves on $S_6$ and $S_4$ are then cut out by a
hyperplane which is tangent to this conic.
Thus, there is an ordinary tacnode, and one can find
the correct multiplicity $4$ for this limit curve as follows.

A multiplicity $\mu$ chain of fibres
(of type \eqref{case:finite} in the notation of \ref{p:mult-junli},
say) 
contributes enumeratively with multiplicity $\mu^2$, whereas a
$\mu$-tacnode 
contributes with multiplicity $\mu$ in the count of $(\mu-1)$-nodal
curves.
The principle to obtain the multiplicity $\mu^2$ in the tacnodal
context is the following: the points at which one can have a
$\mu$-tacnode should be searched within a $g^{\mu-1}_\mu$ on a
smooth rational curve, and there are $\mu$ divisors of the form
$\mu.p$ in such a linear series (for instance, this may be seen by
applying the de Jonquières formula, see
\cite[Section \ttref{s:deJonqu}]{13.th-classic}).
Then, each of those $\mu$ possibilities counts with
multiplicity $\mu$, thus giving the total contribution $\mu^2$ in the
end, as required. 
\end{inparaenum}

It is nevertheless not obvious how to understand in full generality
the limits of the nodes along the degeneration considered in the
present lecture
in terms of the theory
presented in \cite{01.ciro}.
For instance, one ought to deal with situations as
in Figure~\ref{fig:pb-tac} below, where the multiple chain of
fibres is not entirely contracted in the appropriate projective
model.
The curve on Figure~\ref{fig:pb-tac} is a limit of rational
plane quartics, hence carries the limits of three nodes. One node is
amounted for by the tacnode, and the two others by the intersection
point of the double fibre with the curve of class $H$ on $S_7$.
In order to understand this situation within the theory of
\cite{01.ciro}, it is necessary to consider an alternative model
of the degeneration, in such a way that one gets rid of the multiple
curves. 

\begin{figbox}\noindent
\null\hfill
\includegraphics[align=c,scale=1.3]{pb-tac-diag.eps}
\hspace{8mm}
\includegraphics[align=c,height=30mm]{pb-tac-curve.eps}
\hfill\null
\captionof{figure}{Limit of a rational plane quartic with multiple fibres
  (detail)}
\label{fig:pb-tac}
\end{figbox}


% may be written in the following form:
% \begin{equation*}
%   \L_{r,d}\bigl(
%   -d\bar S_r
%   -(d-1)\sum_{i=0}^{k_2} \bar S_{r-1-i}
%   -\cdots
%   \bigr)
% \end{equation*}




\begin{references}

\begin{thebibliography}[Chapters in this Volume\footnote
  {see \url{https://www.math.univ-toulouse.fr/~tdedieu/\#enumTV}}]{III}

\bibitem[I]{01.ciro}
C.~Ciliberto and Th.~Dedieu,
\emph{Limits of nodal curves: generalities and examples}.

\bibitem[III]{03.th-acz}
Th.~Dedieu,
\emph{Geometry of logarithmic Severi varieties at a general point}.

\bibitem[VI]{04.concettina}
Th.~Dedieu and C.~Galati,
\emph{Degenerations and deformations of generalized Severi varieties}.

\bibitem[VII]{08.th-exem}
Th.~Dedieu,
\emph{The Caporaso--Harris recursion within a degeneration of the
  plane}.

\bibitem[X]{11.th-toric-trop}
Th.~Dedieu,
\emph{Enumeration of curves in toric surfaces, tropical geometry, and
floor diagrams}.

\bibitem[XII]{13.th-classic}
Th.~Dedieu,
\emph{Some classical formul{\ae} for curves and surfaces}.

\end{thebibliography}

\begin{thebibliography}[External References]{9}

\bibitem{arroyoetal}
A.~Arroyo, E.~Brugall\'{e} {\normalfont \smfandname} L.~L\'{o}pez~de Medrano,
  \emph{Recursive formulas for {W}elschinger invariants of the projective
  plane}, Int. Math. Res. Not. IMRN (2011), no.~5, 1107--1134.

\bibitem{erwan}
  E.~Brugallé,
  \emph{Floor diagrams relative to a conic, and GW–W
    invariants of Del Pezzo surfaces},
  Adv.\ Math.\ \textbf{279} (2015), 438--500.

\bibitem{BM}
E.~Brugall\'{e} {\normalfont \smfandname} G.~Mikhalkin, \emph{Floor
  decompositions of tropical curves: the planar case}, in \emph{Proceedings of
  {G}\"{o}kova {G}eometry-{T}opology {C}onference 2008}, G\"{o}kova
  Geometry/Topology Conference (GGT), G\"{o}kova, 2009, 64--90.

\bibitem{ch-07}
L.~Caporaso {\normalfont \smfandname} J.~Harris, \emph{Counting plane curves of
  any genus}, Invent. Math. \textbf{131} (1998), no.~2, 345--392.

\bibitem{stephane}
  S.~Druel, 
  \emph{Courbes sur les variétés et leurs espaces de modules --
    Quelques applications},
  lecture notes available at
  \url{http://druel.perso.math.cnrs.fr/textes/ecole2010.pdf}.

\bibitem{ionel-parker}
E.-N. Ionel {\normalfont \smfandname} T.~H. Parker, \emph{The symplectic sum
  formula for {G}romov-{W}itten invariants}, Ann. of Math. (2) \textbf{159}
  (2004), no.~3, 935--1025.

\bibitem{junli-stable}
Jun Li, \emph{Stable morphisms to singular schemes and relative stable
  morphisms}, J. Differential Geom. \textbf{57} (2001), no.~3, 509--578.

\bibitem{junli-degen}
\bysame , \emph{A degeneration formula of {GW}-invariants}, J. Differential
  Geom. \textbf{60} (2002), no.~2, 199--293.

\bibitem{junli-notes}
\bysame , \emph{Lecture notes on relative {GW}-invariants}, in
  \emph{Intersection theory and moduli}, ICTP Lect. Notes, vol.~XIX, Abdus
  Salam Int. Cent. Theoret. Phys., Trieste, 2004, 41--96.

\bibitem{vakil-07}
R.~Vakil, \emph{Counting curves on rational surfaces}, Manuscripta Math.
  \textbf{102} (2000), no.~1, 53--84.

\end{thebibliography}

% \bibliographystyle{mysmf-alpha}
% \bibliography{etages}

\end{references}

\stopcontents[diag-degen]






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End: 
 	


==> toric-trop.tex <==
\chaptitle{Enumeration of curves in toric surfaces, tropical geometry,
  and floor diagrams}
\chapauthor{Thomas Dedieu}

\startchap
\label{11.th-toric-trop}

% WARNING
% redefinition of \:
\def\:{\!:\!}

\newcommand{\Nseq}{\underline{\N}}

\newcommand{\ux}{\underline{x}}

\newcommand{\cE}{\mathcal{E}}

\newcommand{\stp}{\mathsf{p}}
\newcommand{\sL}{\mathsf{L}}

\newcommand{\sd}{\mathsf{d}}

\newcommand{\lz}{\ell_\Z}
\newcommand{\Az}{\mathscr{A}_\Z}
\newcommand{\Ar}{\mathscr{A}}
\newcommand{\amoeba}{am{\oe}ba}
\newcommand{\amoebae}{am{\oe}b{\ae}}
\newcommand{\Val}{\mathrm{Val}}

\newcommand{\Tz}{\mathrm{Tz}}

%\newcommand{\Kappa}{\mathrm{K}}
\newcommand{\antiK}{\reflectbox{$\mathrm{K}$}}
\newcommand{\antiKscr}{\reflectbox{\scriptsize $\mathrm{K}$}}

\newcommand{\diag}{\mathcal{D}}
\newcommand{\orient}{\mathsf{D}}
\newcommand{\vt}{\operatorname{Vert}}
\newcommand{\edg}{\operatorname{Edges}}

\newcommand{\trop}{{\text{trop}}}
\newcommand{\alg}{\mathrm{alg}}
\renewcommand{\top}{\mathrm{top}}

% needs counter memoire
\newenvironment{subnum-fig}
{\setcounter{memoire}{\value{figure}+1}
\setcounter{figure}{0}
\renewcommand{\thefigure}
{\arabic{memoire}\alph{figure}}
}
{\setcounter{figure}{\value{memoire}}}


\startcontents[toric-trop]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[toric-trop]{}{1}[2]{}


\bigskip

The theme of this text is an enumerative problem for curves on toric
surfaces, analogous to the one studied in previous chapters for the
projective plane, and its interplay with related enumerative problems
in different contexts.  Specifically, we will discuss an equivalent
enumerative problem in the framework of tropical geometry, as well as
its translation, under favourable technical circumstances, into a
purely combinatorial enumerative problem involving ad hoc objects
called floor diagrams.
The text also includes an introduction to both toric varieties and
tropical geometry, intended for readers with absolutely no prior
knowledge of these topics (\eg the author himself).

Toric surfaces are compact surfaces containing a torus $(\C^*)^2$, the
complement of which is an anticanonical divisor made of a cycle of
rational curves.
The enumerative problem we are interested in consists in counting
curves of given genus $g$ and Newton polygon $\Delta$, with prescribed
contact pattern with the anticanonical cycle, both at assigned and
unassigned points, and passing through the appropriate number of
general base points; the shape of the polygon $\Delta$ determines which
toric surface the curves live in, while the lengths of its sides
determine their linear equivalence class.
Problems of this kind naturally arise when one studies an enumerative
problem by degeneration as discussed in \cite{01.ciro}, much in the
same way that logarithmic Severi varieties of the pair
$(\P^2, \text{line})$ show up when one studies plain Severi varieties
of the projective plane, as explained in \cite{04.concettina}.

Plane tropical\footnote
{The term `tropical' is empty from mathematical intuition: it refers
  to Imre Simon who resided in Brazil,
see \cite[p.~283]{mikhalkin-faces}.}
curves are piecewise linear objects in the real plane
$\R^2$ (equipped with the integral structure determined by $\Z^2$),
which appear as a sort of projected shadows of algebraic
curves in $(\C^*)^2$, following seminal ideas of Kapranov
\cite{kapranov-etal}
and others. Of course much information is lost in the
projection, but it is quite miraculous how good tropical curves are at
representing algebraic curves.
In particular, it has been shown by Mikhalkin, following a suggestion
by Kontsevich (see \cite{kontsevich-soibelman}),
that the aforementioned enumerative problem for curves in toric
surfaces is equivalent to its tropical shadow.

An advantage of tropical curves over algebraic curves is that they are
much more hands-on: it is possible to play around with them using a
ruler and a sheet of gridded paper without losing any piece of
information. The tropical enumerative problem is therefore more
tractable than the original toric problem, and in principle it can be
solved with elementary considerations only: we shall see several
instances of this in the text.
Yet, of course, when the size of the problem gets too large, it is
no longer possible to solve it with bare hands.

It has been realized by Brugallé and Mikhalkin that
stretching the base points of the tropical enumerative problem
along a chosen direction in $\R^2$ helps structuring its solution.
In particular, under mildly favourable technical conditions, if the base
points are far enough one from another along this direction, then
for all the tropical curves one wants to count, the base points are
distributed one by one on certain ``components'';
these ``components'' are of two types, floors
and elevators, and their incidence relations may be neatly encoded in
a combinatorial device called a floor diagram.
Then, the tropical enumerative problem translates into a problem of
enumeration of floor diagrams enhanced with a marking,
the latter encoding
the distribution of the base points on the various components.
The tropical enumerative problem may also be solved using the so-called
lattice path algorithm, which had been given by Mikhalkin already in
\cite{mikhalkin-JAMS},
but we will not discuss it here.

To conclude this introduction, let me mention some aspects and
developments that will not be discussed any further in the text.
Quite remarkably,
tropical geometry and floor diagrams also allow the study of
enumerative problems in real algebraic geometry.
In particular they have permitted the computation of Welschinger
invariants, which count real rational curves with a sign depending on
the real nature of their singularities
(see the nice survey \cite{BIMS}).
It has to be noted that
the correspondence between (algebraic) curves and floor diagrams
counting can be established without resorting to tropical geometry, by
degeneration, as has been discovered by Brugallé \cite{erwan-11}
(this is explained in \cite{07.th-diag-degen}).
On the other hand, tropical geometry gives a framework in which it is
possible to define new enumerative invariants.
For instance, one can define tropical Welschinger invariants in
positive genus, whereas it is proven that the corresponding real
algebraic enumerative problem is not invariant under the choice of the
general base points.
One can also count plane tropical curves with multiplicities that are
rational fractions in the (quantum) indeterminate $q$, which leads to
the so-called Block--Göttsche invariants; the latter are polynomials
in $q$ interpolating between Welschinger (given by $q=-1$) and
Gromov--Witten (given by $q=1$) invariants; the
enumerative interpretation of their coefficients is still unclear.
About these new invariants, see \cite{BIMS} and the references
therein.

The formulation as an enumerative problem about floor diagrams has
enabled Fomin and Mikhalkin \cite{fomin-mikhalkin} to prove various
nice results about complex algebraic plane curves. In particular, they
have obtained a proof of the Di Francesco--Itzykson conjecture, to the
effect that for all $\delta \geq 0$, there exists a degree $2\delta$
polynomial $P_\delta \in \Q[d]$ such that for all large enough $d$,
$P_\delta(d)$ is the number of degree $d$ plane curves with $\delta$
nodes passing through the appropriate number of general base points.
This is a particular case of the Göttsche conjecture, and
it is related to the results discussed in
\cite{14.th-vainsencher} and \cite{12.fra-goettsche}.

Floor diagrams have been used by Brugallé and Mikhalkin
\cite{BM-higherdim} to give an equivalent formulation of the
problem of enumerating rational curves in a complex projective space
of arbitrary dimension.
Also, adapted versions of floor diagrams have been applied to the
study of Gromov--Witten invariants with (stationary) descendant
insertions of Hirzebruch surfaces, see
\cite{block-gathmann-markwig} and \cite{cavalieri-etal}
(the descendant insertions mean that we are imposing more elaborate
conditions than the passing through base points in order to arrive at
a finite number of curves).

\medskip
For this presentation I have drawn from various sources, to which I
owe a great intellectual debt.
The general presentation of tropical geometry follows rather closely a 
mini course given by Ilia Itenberg,
{\emph{Géométrie tropicale énumérative}, at the 2010 GAGC meeting at
  CIRM.}
The presentation of plane and abstract tropical curves, and of the
tropical enumerative problem, exists only thanks to personal lectures
offered by Erwan Brugallé to the author in Jussieu, 2016.
The presentation of floor diagrams and their enumeration follows
Brugallé and Mikhalkin's article \cite{BM-11}.
Finally, I wish to mention a wonderful talk by
Kontsevich \cite{Kontsevich}, which in principle was targeted for
master students, but contains illuminating insights on tropical
geometry and its interplay with algebraic geometry.

There are several texts written by experts of tropical geometry which
the reader can consult:
\cite{AMMonthly} is written for a broad audience of mathematicians,
and does not discuss enumerative geometry;
\cite{X-UPS} does discuss enumerative geometry, and targets an
audience of graduate students;
\cite{BIMS} and \cite{tropicalOW} are intended for geometers.
I also recommend the somehow historical \cite{viro}.

\medskip
The text starts by a quick introduction to toric surfaces
(in Section \ref{s:toric-surf}),
based on my personal down-to-earth understanding of it
(but supported by the reference \cite{CLS})
and guaranteed free of fans,
after what we state the
enumerative problem for curves on toric surfaces
(in Section \ref{s:enumpb}).
Section \ref{s:degenK3} gives several examples, showing how the toric
enumerative problem in question arises when one studies, say, the
enumerative geometry of $K3$ surfaces by degeneration to unions of
planes. 
Plane tropical curves are introduced in Section \ref{S:trop-curves}
in the way we need them in order to state
and study the relevant tropical enumerative problem.
Before that, I briefly explain in Section \ref{S:tor-to-trop} the ideas
that led to the definition of these objects.
Section \ref{s:legendre} is a parenthesis about the
Legendre--Fenchel transformation (often merely called Legendre
transformation), which is a useful tool in the study of corner loci
and tropical hypersurfaces. It is possible to skip Sections
\ref{S:tor-to-trop} and \ref{s:legendre}, as Section \ref{S:trop-curves}
should be self-contained, and sufficient to understand the remainder
of the text.
In Section \ref{S:trop-enumpb} we state the tropical enumerative
problem (using the definitions of Section \ref{S:trop-curves})
and explain the correspondence with the toric enumerative problem.
Finally, Section \ref{S:floors} is dedicated to the translation of the
tropical enumerative problem in terms of floor diagrams.
The last Section \ref{S:trop-design} is a sort of appendix, in which
we develop the idea that tropical curves are great
for the graphic representation of
algebraic curves; we will see in particular that the graphic
representation of the degeneration procedure of
\cite{07.th-diag-degen} (which is an alternative path to floor
diagrams) makes for striking revelations.



\paragraph*{Thanks}
I am grateful to Thomas Blomme and Ilia Itenberg for their comments on
a preliminary version of this text, and to Erwan Brugallé for his
essential help in the conception of this text.




\paragraph{General notation}
\label{p:notation}
% \phantomsection
% \addcontentsline{toc}{subsection}{General notation}
We use the notation of
\cite[\ttref{not:Nseq}]{03.th-acz}
and \cite[\ttref{not:CH-Nseq}]{04.concettina}.
In particular $\Nseq$ denotes the set of sequences $\alpha =
[\alpha_1,\alpha_2,\ldots]$ of non-negative integers with
only finitely many $\alpha_i$ non-zero,
and for all $\alpha \in \Nseq$, 
\begin{equation*}
  |\alpha| = \sum_i \,\alpha_i,
  \qquad
  I\alpha = \sum_i \,i\, \alpha_i,
  \Et
  I ^\alpha = \prod_i \,i^{\alpha _i}.
\end{equation*}

For any vector $u$ in the real plane $\R^2$, we denote
by $\orth u$
the vector obtained by rotating $u$ by $+\pi/2$.
A vector $u=(a,b) \in \Z^2$ is \emph{primitive} if $a$ and $b$ are
relatively prime.

On the projective plane $\P^2$, we let $H$ denote the line
class.
On Hirzebruch ruled surfaces $\F_e$, we let $E$ be the exceptional
section, $F$ the class of fibres of the ruling, and $H=E+eF$. 






\section{Toric projective surfaces}
\label{s:toric-surf}


\subsection{The prototypical examples}
\label{p:proto-toric}
Let $S$ be a surface equipped with a system of (pluri) homogeneous
coordinates, and fix a (multi) degree $d$.
The projectivization of the space
$V_d$ of all homogeneous polynomials of degree $d$ is a complete linear
system of curves on $S$. 
The notion of \emph{Newton polygon} enables one to define linear
subsystems of $\P V_d$ in a remarkably meaningful way, as follows.

Degree $d$ monomials form a basis of $V_d$, and may be represented as
lattice points $\stp_1,\ldots,\stp_{N_d}$ in some real affine space
(by \emph{lattice points}, or \emph{integral points}, we mean points
with integral coordinates).
Consider a convex polygon $\Delta$, the vertices of which belong to
$\{ \stp_1,\ldots,\stp_{N_d} \}$.
One lets $V_\Delta$ be the subspace of $V_d$ generated by those
monomials whose corresponding lattice point $\stp$ lies in
$\Delta$
(thus, we see $\Delta$ as a $2$-dimensional convex domain).
We will see that the subsystem $\P V_\Delta$ of $\P V_d$ may
alternatively be defined in a natural way by base
points, possibly infinitely near.
This is best understood by looking at a couple of examples.

\begin{example}[$\P^2$]
\label{ex:P2}
It comes with a system of homogeneous coordinates $(x\!:\!y\!:\!z)$.
Fix a degree $d \in \N$; to each monomial $x^ay^bz^c$ of degree $d$,
we associate the lattice point $(a,b) \in \R^2$ 
(of course this determines $c=d-a-b$). Degree $d$ monomials then
correspond bijectively to points with integral coordinates in the
triangle 
\[
T_d\overset{\text{def.}}=
\{ (a,b) \in \R^2: a,b \geq 0\ \text{and}\ a+b \leq d \}.
\]
We may for instance consider the two Newton polygons pictured
below. 
\begin{center}
(a)
\includegraphics[trim=-.5cm 1cm 0 0]{conics-1pt.eps}
\hspace{1cm}
(b)
\includegraphics[trim=-.5cm 1cm 0 0]{conics-2infpt.eps}\vspace*{1cm}
\end{center}

In case (a), the elements of $V_\Delta$ are the quadratic
polynomials of the form
\begin{equation*}
f_2(x,z) + y f_1(x,z),
\end{equation*}
with $f_2$ and $f_1$  homogeneous polynomials of degrees $2$ and
$1$, respectively. Thus, $\P V_\Delta$ is the linear system
of conics passing through the point $(0\!:\!1\!:\!0)$.

In case (b), $V_\Delta$ consists of the polynomials of the form
\begin{equation*}
f_2(x,z)  + \alpha  \cdot yz,
\end{equation*}
with $f_2$ a degree $2$ homogeneous polynomial, and $\alpha \in
\C$.
Thus, $\P V_\Delta$ is the linear system of conics
passing by the point $(0\:1\:0)$, and tangent to the line
$z=0$ there
(if you set $z=0$ in the above expression, only the $x^2$ term does not
vanish).
\end{example}

\begin{example}[$\P^1 \times \P^1$]
\label{ex:P1P1}
It comes with a system of bihomogeneous coordinates 
$((x_0:x_1),(y_0:y_1))$.
Fix a bidegree $d=(d_1,d_2) \in \N^2$; to each monomial 
$x_0 ^{a_0} x_1 ^{a_1} y_0 ^{b_0} y_1 ^{b_1}$ of bidegree $d$, we
associate the lattice point $(a_1,b_1) \in \R^2$. Bidegree $d$
monomials then correspond bijectively to points with integral
coordinates in the rectangle
\[
R_{d_1,d_2}\overset{\text{def.}}=
\{ (a,b) \in \R^2: a,b \geq 0,\ a\leq d_1,\ \text{and}\ b \leq d_2 \}.
\]
On the picture below, the polygon (a) (resp.\ (b)) corresponds to
the linear system of hyperplane sections (resp.\ of sections by
quadrics) of $\P^1 \times \P^1$ embedded as a smooth quadric surface
in $\P^3$.
\begin{center}
(a)
\includegraphics[trim=-.5cm .5cm 0 0]{quadric-hyp.eps}
\hspace{1cm}
(b)
\includegraphics[trim=-.5cm 1cm 0 0]{quadric-qu.eps}
\vspace*{1cm}
\end{center}

Observe that the polygon (a) may also be realized inside the triangle
$T_2$ of Example \ref{ex:P2}.
In this incarnation, it corresponds to the linear
system of plane conics with 
the two base points $(1\:0\:0)$ and $(0\:1\:0)$.
The map associated to this linear system is birational from $\P^2$ to
a smooth quadric surface. It follows that the two incarnations of the
polygon (a) give the same linear system of curves.
\end{example}


\subsection{The general construction}


\paragraph{}
\label{p:gnl-tor-cstr}
Let $\Delta \subset \R^2$ be a convex polygon with vertices at
integral points (this is called a \emph{lattice polygon}), and let
$\stp_i=(a_i,b_i)$, $i=1,\ldots, N_\Delta$, be the integral points of
$\R^2$ lying inside $\Delta$. 
We associate the following map to $\Delta$:
\begin{alignat*}{2}
\phi_\Delta:&\quad & (\C^*)^2 &\to \P^{N_\Delta -1} \\[-1.5mm]
&& (t_1,t_2) & \mapsto \bigl( t_1^{a_1}t_2^{b_1}: \ldots : 
t_1^{a_{N_\Delta}}t_2^{b_{N_\Delta}} \bigr).
\end{alignat*}
Then, we define $X_\Delta \subset \P^{N_\Delta -1}$
to be the Zariski closure in $\P^{N_\Delta -1}$ of the
image of $\phi_\Delta$; it is a projectively normal surface,
see \cite[Thm.~2.4.1, Def.~2.3.14, and Cor.~2.2.13]{CLS}.

Thus, the object associated to $\Delta$ is a normal
surface in a given projective embedding; equivalently, it is a
surface together with a linear system of Cartier divisors. 
It is possible to build a combinatorial object from $\Delta$ that
forgets about the embedding, which is called a \emph{fan};
it is usually the preferred object in toric geometry.
In this text however, our primary interest resides in linear
systems (hence in polytopes), and we shall not discuss fans.

Quite remarkably, the surface $X_\Delta$ thus constructed may always
be equipped with a system of homogeneous coordinates,
see \cite[Chapter 5]{CLS},
so that we can play the game of Section \ref{p:proto-toric} with it, and
associate the complete linear system $|\O_{X_\Delta}(1)|$ with a
polygon. The latter polygon is the very $\Delta$ we started with.

\begin{remark}
\label{rk:gnl-tor-cstr}
One may rephrase the above definition in the terms
of Section \ref{p:proto-toric}.
For instance, any $\Delta$ as above may be realized inside a
triangle $T_d$ as in \ref{ex:P2}, for sufficiently large $d$
(note that the definition of $\phi_\Delta$ is invariant
under translation of $\Delta$). Then, $\Delta$ determines a linear
system of degree $d$ plane curves of dimension $N_\Delta -1$, and
$\phi_\Delta$ equals the restriction to
\[
  (\C^*)^2 \simeq \bigl\{ (t_0\:t_1\:t_2):
  t_0t_1t_2\neq 0
  \bigr\}
  \,\subset\, \P^2
\]
of the rational
map $\P^2 \dashrightarrow \P^{N_\Delta -1}$ associated with this
linear system.

Similarly, $\Delta$ may always be realized inside a rectangle
$R_{d_1,d_2}$ as in \ref{ex:P1P1}, and $\phi_\Delta$ identified with
the restriction to 
\[
  (\C^*)^2 \simeq \bigl\{ (s_1\:t_1),(s_2\:t_2)):
  s_1t_1s_2t_2\neq 0
  \bigr\}
  \,\subset\, \P^1\times\P^1
\]
of the rational map $\P^1\times\P^1 \dashrightarrow \P^{N_\Delta -1}$
associated with the corresponding linear system.

We thus see that the construction in Section \ref{p:proto-toric} does not
depend on the choice of the surface $S$ at the beginning, but only on
the polygon $\Delta$.
\end{remark}


\paragraph{Equations}
One may compute the equations of $X_\Delta$ in $\P^{N_\Delta-1}$ by
elimination from a parametrization of the affine cone
$\widehat X_\Delta$ over $X_\Delta$.
To do so, beware that the map
\[
  \widehat \phi_\Delta:
  (t_1,t_2) \in (\C^*)^2
  \mapsto
  \bigl( t_1^{a_1}t_2^{b_1}: \ldots : 
  t_1^{a_{N_\Delta}}t_2^{b_{N_\Delta}} \bigr)
  \in (\C^*)^{N_\Delta}
\]
of course does not parametrize (an open subset of) the affine cone
$\widehat X_\Delta$.
To obtain such a parametrization, one may apply the trick described in
\cite[top of p.~58]{CLS}, and consider instead the map
\[
  (t_0,t_1,t_2) \in (\C^*)^3
  \mapsto
  \bigl( t_0t_1^{a_1}t_2^{b_1}: \ldots : 
  t_0t_1^{a_{N_\Delta}}t_2^{b_{N_\Delta}} \bigr)
  \in (\C^*)^{N_\Delta}.
\]
Then, the equations of $X_\Delta$ in $\P^{N_\Delta-1}$
may be obtained by eliminating $(t_0,t_1,t_2)$ from the ideal
\[
  \bigl( x_1-t_0t_1^{a_1}t_2^{b_1},\, \ldots,\,
  x_{N_\Delta}-t_0t_1^{a_{N_\Delta}}t_2^{b_{N_\Delta}} \bigr)
  \subset\, \C[t_0,t_1,t_2]\otimes \C[x_1,\ldots,x_{N_\Delta}].
\]

Alternatively, one may consider the map
\begin{equation}
\label{eq:param_P2}
  (t_0,t_1,t_2) \in (\C^*)^3
  \mapsto
  \bigl( t_0^{d-a_1-b_1}t_1^{a_1}t_2^{b_1}: \ldots : 
  t_0 ^{d-a_{N_\Delta}-b_{N_\Delta}}
  t_1^{a_{N_\Delta}}t_2^{b_{N_\Delta}} \bigr) 
  \in (\C^*)^{N_\Delta},
\end{equation}
corresponding to the extension of $\phi_\Delta$ to a rational map
$\P^2 \dashrightarrow \P^{N_\Delta -1}$ discussed in
Remark \ref{rk:gnl-tor-cstr}.
It does parametrize an open subset of the affine cone
$\widehat X_\Delta$ by \cite[Prop.~2.1.4]{CLS},
since the linear functional on monomials
$t_0^ct_1^at_2^b \mapsto a+b+c$ takes the value $d$ on all monomials
appearing in the map \eqref{eq:param_P2}.
Then, one may obtain the equations of $X_\Delta$ in $\P^{N_\Delta-1}$
by eliminating $(t_0,t_1,t_2)$ from the ideal
\[
  \bigl(
  x_1-t_0^{d-a_1-b_1}t_1^{a_1}t_2^{b_1},\, \ldots,\,
  x_{N_\Delta}-t_0 ^{d-a_{N_\Delta}-b_{N_\Delta}}
  t_1^{a_{N_\Delta}}t_2^{b_{N_\Delta}} \bigr) 
\]
as above.
  
Similarly, one may consider the map
\begin{equation}
  \label{eq:param_P1xP1}
  (s_1,s_2,t_1,t_2) \in (\C^*)^4
  \mapsto
  \bigl( s_1^{d_1-a_1}s_2^{d_2-b_1}t_1^{a_1}t_2^{b_1}: \ldots : 
  s_1^{d_1-a_{N_\Delta}}s_2^{d_2-b_{N_\Delta}}
  t_1^{a_{N_\Delta}}t_2^{b_{N_\Delta}} \bigr) 
  \in (\C^*)^{N_\Delta}
\end{equation}
corresponding to the extension of $\phi_\Delta$ to a rational map
$\P^1\times\P^1 \dashrightarrow \P^{N_\Delta -1}$ discussed in
Remark \ref{rk:gnl-tor-cstr},
which parametrizes an open subset of the affine cone
$\widehat X_\Delta$ by \cite[Prop.~2.1.4]{CLS},
since the two linear functionals
$s_1^{a'}s_2^{b'}t_1^at_2^b \mapsto a+a'$
and $s_1^{a'}s_2^{b'}t_1^at_2^b \mapsto b+b'$ take the values $d_1$
and $d_2$, respectively, on all monomials
appearing in the map \eqref{eq:param_P1xP1}.


\begin{example}
\label{sp:trapezium}
The trapezium 
\[
  \Tz^r_{a,b}
  = \bigl\{
  (x,y) \in \Z^2:
  0 \leq y \leq a
  \text{ and }
  0 \leq x \leq b +(r-y)a
  \bigr\}
\]
corresponds to the complete linear system
$|aH+bF|$ on the Hirzebruch surface $\F_r$, where $F$ is the class of
a fibre, and $H=E+rF$ with $E$ the class of the section with
self-intersection $-r$.
\begin{figure}[htbp]
\centering
\includegraphics{Tz.eps}
\caption{The trapezium $\Tz^2_{3,2}$:
  $|3H+2F|$ on $\F_2$}
\label{fig:tz}
\end{figure}
\end{example}



\subsection{Geometric properties and numerical invariants}
Consider a surface $X_\Delta$ constructed from a convex integral
polygon $\Delta \subset \R^2$ as in \ref{p:gnl-tor-cstr}.

\paragraph{Anticanonical cycle}
The complement $X_\Delta \setminus \phi_\Delta
((\C^*)^2)$ is a cycle of rational curves, and it is a Weil divisor
belonging to the anticanonical linear equivalence class
$-K_{X_\Delta}$, see
\cite[Theorem 8.2.3]{CLS}; we shall
call it the \emph{anticanonical cycle} of $X_\Delta$, and denote it by
$\antiK_\Delta$.
% \footnote
% {this is a capital 'kappa', standing for cycle. Hopefully no confusion
%   will occur between $\Kappa_\Delta$ and $-K_{X_\Delta}$.}
\par Being a cycle of rational curves means that $\antiK_\Delta$ is a
union of rational curves $C_1,\ldots,C_n$, where each $C_i$ intersects
$C_{i-1}$ and $C_{i+1}$ transversely\footnote
{two consecutive curves $C_i$ and $C_{i+1}$ of $\antiK_\Delta$
  certainly intersect transversely in $\P^{N_\Delta-1}$, because they
  span two linear subspaces $\P^{\ell_i}$ and $\P^{\ell_{i+1}}$ which
  intersect at one point only. However, the surface $X_\Delta$ may be
  singular at the point $C_i \cap C_{i+1}$, and the intersection
  number $C_i \cdot C_{i+1}$ differs from $1$ in general.}
at one point (with the convention
that $C_0=C_n$ and $C_{n+1}=C_1$) and no other curve.
\par The curves $C_1,\ldots,C_n$ correspond to the edges
$\Sigma_1,\ldots,\Sigma_n$ (labelled in a cyclic way)
of the polygon $\Delta$, and the intersection points
$C_i \cap C_{i+1}$ to its vertices.
In the projective embedding given by $\Delta$,
the curve $C_i$ is a rational normal curve
of degree $\lz(\Sigma_i)$,
which we define as the \emph{integral length} of the
segment $\Sigma_i$,
\ie the number of integral points lying on
$\Sigma_i$ minus one.

\paragraph{Degree and number of sections}
\label{p:deg-Delta}
We let $H_\Delta$ be the class $c_1(\O_{X_\Delta}(1))$, corresponding to the
embedding defined by $\Delta$. 
The dimension $h^0(\O_{X_\Delta}(1))$ is
the number $N_\Delta$ of integral points lying in $\Delta$ minus one.
One may think of $N_\Delta$ as an integral measure of the area of
$\Delta$, in analogy with the integral length $\lz$, but beware that
the integral area of $\Delta$ is usually defined as 
$2 \Ar (\Delta)$, in the notation introduced in \ref{sp:p_a} below.

\par The anticanonical degree of $H_\Delta$ is
\begin{equation*}
-K_{X_\Delta} \cdot H_\Delta = \antiK_\Delta \cdot H_\Delta
= {\textstyle \sum _{i=1}^n \lz(\Sigma_i)}
= \Card (\partial \Delta_\Z),
\end{equation*}
where $\partial \Delta_\Z$ stands for the set of integral points in
the boundary of $\Delta$,
see \cite[Proposition 10.5.6]{CLS}.

\paragraph{Arithmetic genus}
\label{sp:p_a}
The arithmetic genus of the divisors belonging to the linear system
$|\O_{X_\Delta}(1)|$ is
\begin{equation*}
p_a(\Delta)\overset{\text{def.}}= p_a (H_\Delta) = 
\Card (\mathring{\Delta} _\Z),
\end{equation*}
where $\mathring{\Delta} _\Z$ stands for the set of integral points in
the interior of $\Delta$,
see \cite[Proposition 10.5.8]{CLS}.

Equivalently, one has
\begin{equation*}
(H_\Delta)^2 = 2 \Ar (\Delta),
\end{equation*}
where $\Ar(\Delta)$ is the \emph{Euclidean area} of $\Delta$,
taking
the area of the quadrilateral defined by any lattice basis of
$\R^2$
as the unit,
\cite[Proposition 10.5.6]{CLS}.

With the two above identities, the adjunction formula
\[
  2p_a(H_\Delta)-2 =  (K_{X_\Delta}+H_\Delta)\cdot H_\Delta
\]
amounts to Pick's formula, see \cite[Example 9.4.4]{CLS}, which
expresses the area of a lattice polygon in terms of its lattice
points. 


\paragraph{Singularities}
\label{p:sings}
The surface $X_\Delta$ is smooth except (possibly) at the points
corresponding to the vertices of the anticanonical cycle
$\antiK_\Delta$, where it has cyclic quotient singularities,
the types of which are determined as follows
(see \cite[Section 10.1]{CLS}).

Consider a vertex $v$ of $\Delta$, and
let $u_v'$ and $u''_v$ be the two primitive integral vectors
giving the directions of the
two edges of $\Delta$ intersecting at $v$ and pointing away from $v$,
in such a way that the angle $(u'_v,u''_v)$ points inside $\Delta$.
Then the two vectors $\orth [u_v']$ and $-\orth [u_v'']$ are the normal
vectors of the two edges at $v$, pointing towards the interior of
$\Delta$
(see Figure~\ref{fig:sings-F2} for an example).
It is always possible to find an integral basis $(e_1,e_2)$ of $\Z^2$
such that the two vectors
$\orth [u_v']$ and $-\orth [u_v'']$
write
\[
  e_2
  \quad \text{and}
  \quad
  de_1-ke_2,
\]
where $d$ and $k$ are relatively prime integers such that
$d>0$ and $0\leq k <d$.
Then the singularity of the surface $X_\Delta$ at the point
corresponding to the vertex $v$ is of type $\frac 1 d (1,k)$,
\ie it is analytically locally isomorphic to the quotient of
$\C^2$ by the group of $d$-th roots of unity acting as
$\zeta.(x,y) = (\zeta x, \zeta^k y)$.

In particular,
the Euclidean area of the parallelogram defined by $u_v'$ and
$u''_v$, namely
\[
  \Ar \bigl(\vect {u_v', u''_v} \bigr)
  = \det(u_v',u_v'')
\]
computes the order $d$ of the cyclic group, the action of which
defines the singularity at the point of $X_\Delta$ corresponding to
$v$.
The surface is smooth at this point if $(u'_v,u''_v)$ forms a basis of
$\Z^2$, and it has an ordinary double point if
$\det(u_v',u_v'') = 2$.

\begin{figbox}
\includegraphics{sings-F2.eps}
\captionof{figure}{Determination of the types of singularities at the
  vertices: the triangle $\Tz^2_{3,0}$,
  $|3H|$ on $\F_2$}
\label{fig:sings-F2}
\end{figbox}


\begin{example}
Consider $v$ the lower-right corner of the
trapezium $\Tz^r_{a,b}$, see \ref{sp:trapezium} and
Figure~\ref{fig:sings-F2} above.
Then
$u_v'=(-r,1)$ and $u_v''=(-1,0)$,
hence
$\orth [u_v'] = (-1,-r)$ and $-\orth [u_v'']=(0,1)$,
and we find that the corresponding
point in the image of $\F_r$ by $|aH+bF|$ is a smooth point.

Consider on the other hand $v$ the upper vertex of the triangle
$\Tz^r_{a,0}$.
Then $u_v' =(0,-1)$ and $u_v''=(r,-1)$,
hence 
$\orth [u_v'] = (1,0)$ and $-\orth [u_v'']=(-1,-r)$.
We may take $e_1=(0,-1)$ and $e_2=(1,0)$, to the effect that
\[
  \orth [u_v'] = e_2
  \quad \text{and}
  \quad
  -\orth [u_v'']= r e_1 - e_2.
\]
Thus the singularity at the point corresponding to $v$ is of type
$\frac 1 r (1,1)$,
which analytically locally is the vertex of the
cone over a rational normal curve of degree $r$.
And indeed the image of $\F_r$ by $|aH|$ is a generalized cone over a
degree $r$ rational normal curve, and the point under consideration is
its vertex.
\end{example}



\section{The toric enumerative problem}
\label{S:toric}


\subsection{Toric Cayley--Bacharach}

The following may be considered as a toric Cayley--Bacharach property,
and needs to be taken in consideration in order to properly state the
toric enumerative problem.
Later on, we will also see a tropical incarnation of this phenomenon,
see Figure~\ref{fig:tropical-CB}
and Figure~\ref{fig:Wij:tropical-CB}.

\begin{lemma}
\label{l:torCB}
Let $Z$ be a subscheme of\/ $\antiK_\Delta$ cut out by a 
(properly intersecting) hyperplane in
$\P^{N_\Delta -1}$. It imposes only\/ $\deg Z -1$ independent conditions
to the linear system $|\O_{X_\Delta}(1)|$,
\ie the linear subsystem of divisors containing $Z$ has codimension
$\deg Z -1$ in $|\O_{X_\Delta}(1)|$.
\end{lemma}

This follows from a basic cohomological argument, valid regardless of
our toric setup, see also \cite[Example \ttref{ex:logK3i}]{03.th-acz}.
In the toric setup however, there is a nice elementary way of
understanding it.

% \begin{proof}
% This is a mere application of the Riemann--Roch formula.
% One has
% \begin{equation*}
% h^0(\O_{X_\Delta}(1))
% = \chi(H_\Delta) = 1 + \frac
% {(-K_{X_\Delta}+H_\Delta)\cdot H_\Delta} 2
% \end{equation*}
% and
% \begin{align*}
% h^0(\O_{X_\Delta}(1) \otimes \I_Z)
% = \chi (\O_{X_\Delta}(1) \otimes \I_Z) &= 1 + \frac
% {\bigl(-K_{X_\Delta}+(H_\Delta +K_{X_\Delta}) \bigr)
% \cdot (H_\Delta +K_{X_\Delta})} 2 \\
% &= 1 + \frac 
% {(K_{X_\Delta} +H_\Delta) \cdot H_\Delta} 2 \\
% &= h^0(H_\Delta) + K_{X_\Delta} \cdot H_\Delta
% =  h^0(H_\Delta) - \antiK_{\Delta} \cdot H_\Delta.
% \end{align*}
% \end{proof}

\begin{proof}%[Dull cohomological proof]
The lemma follows from the long exact sequence in cohomology
induced by the restriction exact sequence,
\[
  0 \to
  \O_{X_\Delta}(K_{X_\Delta}+H) \to
  \O_{X_\Delta}(H) \to
  \O_{\antiKscr_\Delta}(H)
  \to 0.
\]
Indeed, $h^1(O_{X_\Delta}(K_{X_\Delta}+H))=0$ by Kawamata-Viehweg
vanishing,
and $h^0(\O_{\antiKscr_\Delta}(H)) = \deg Z$ by Riemann--Roch, since
$p_a(\antiK_\Delta)=1$.
\end{proof}

% \begin{proof}[Nice elementary proof]
% \end{proof}

Let me now give an elementary argument showing
why $Z$ cannot impose independent conditions to hyperplane sections
of $X_\Delta$.
Let $C_1,\ldots,C_n$ be the smooth rational curves forming the cycle
$\antiK_\Delta$. We shall exhibit an explicit relation between
the roots of the polynomials $\restr P {C_1}, \ldots, \restr P {C_n}$, 
for all polynomials $P$ with Newton polygon $\Delta$,
which implies that if $P$ vanishes at all the points of $Z$ but one,
then it also vanishes at the last point.

Let $P$ be a polynomial with Newton polygon $\Delta$, and name its
coefficients regarding the monomials on the boundary of $\Delta$ as
indicated on the picture below.
\begin{center}
\includegraphics[scale=2]{toric-CB.eps}
\end{center}
\noindent
Thus, for all $i=1,\ldots,n$, we have
$\restr P {C_i}
= a_{i,0} + \cdots + a_{i,\ell_i} X^{\ell_i}$, hence the product of
the roots of $\restr P {C_i}$ equals
$(-1) ^{\ell_i} {a_{i,0}} / {a_{i,\ell_i}}$.
Therefore, the product of the roots of
$\restr P {C_1}, \ldots, \restr P {C_n}$ altogether equals
\[
  (-1) ^{\ell_1+\cdots+\ell_n}\,
  \frac {a_{1,0}} {a_{1,\ell_1}}\,
  \cdots\,
  \frac {a_{n,0}} {a_{n,\ell_n}}
  = (-1) ^{\ell_1+\cdots+\ell_n},
\]
which is the announced relation.



\subsection{The enumerative problem}
\label{s:enumpb}

\paragraph{}
\label{p:enumpb}
Let $\Delta \subset \R^2$ be a convex integral polygon as in
Section~\ref{s:toric-surf}. We call $\Sigma_1,\ldots,\Sigma_n$ its
edges, and correspondingly $C_1,\ldots,C_n$ the irreducible components
of the anticanonical cycle $\antiK_\Delta$. 
\par Let $g$ be an integer such that $0 \leq g \leq p_a(\Delta) =
\Card (\mathring{\Delta}_\Z)$,
and $\alpha=(\alpha_1,\ldots,\alpha_n),
\beta=(\beta_1,\ldots,\beta_n) \in \Nseq^n$.
We assume that for $s=1,\ldots,n$,
\begin{equation*}
I\alpha_s + I\beta_s=(C_s \cdot H_\Delta) = \lz (\Sigma_s),
\end{equation*}
and
\begin{equation*}
I\alpha \overset{\text{def.}}{=} \textstyle{\sum _{s=1}^n I\alpha_s} 
< (\antiK_\Delta \cdot H_\Delta) = \Card (\partial \Delta_\Z).
\end{equation*}
The problem is to find the number $N^\Delta_g (\alpha,\beta)$
 of genus $g$ curves in the linear
system $|H_\Delta|$ that 
(i) are the Zariski closure of a curve in 
$\phi_\Delta ((\C^*)^2) \cong (\C^*)^2 \subset X_\Delta$, 
(ii) verify the contact conditions with $\antiK_\Delta$ at assigned and
unassigned points fixed by $\alpha$ and $\beta$, respectively,
and (iii) pass through the appropriate number of fixed general points
in $X_\Delta$.
\par The precise setup is as follows.
We fix $\ux=\{x_1,\ldots,x_{g-1+|\beta|} \}$ a set of 
\begin{equation*}
g-1+|\beta| = \Card (\partial \Delta_\Z) +g-1-I\alpha-(I\beta-|\beta|)
\end{equation*}
general points in $X_\Delta$,
and $\Omega = (\{ p_{s,i,j} \} _{1\leq j \leq \alpha_{s,i}} )
_{1\leq s \leq n, 1 \leq i}$
a set of $\alpha$ general points on $\antiK_\Delta$,
\ie for $s=1,\ldots,n$, 
$\Omega_s = (\{ p_{s,i,j} \} _{1\leq j \leq \alpha_{s,i}} ) _{1 \leq i}$
is a set of $\alpha_s \in \Nseq$ general points on the
curve $C_s$.
We want the number of birational maps $\phi: C \to X_\Delta$, 
where $C$ is a
%\taf{irreducible?}
reduced, nodal curve of arithmetic genus $g$,
such that (i) $\phi(C)$ equals the Zariski closure of 
$\phi (C) \cap (X_\Delta \setminus \antiK_\Delta)$,
(ii) there exist $\alpha$ points $q _{s,i,j}$
%$1 \leq s \leq n$, $1 \leq j \leq \alpha_{s,i}$, 
and $\beta$ points $r _{s,i,j}$ on  $C$ such that
$\phi (q_{s,i,j}) = p_{s,i,j}$
and
\begin{equation*}
\phi^* \antiK_\Delta = 
\sum _{1 \leq s \leq n}
\sum _{1 \leq i}
\raisebox{-1mm}{$\biggl($}
\sum _{1 \leq j \leq \alpha_i} i \, q_{i,j}
+ \sum _{1 \leq j \leq \beta_i} i\, r_{i,j}
\raisebox{-1mm}{$\biggr)$},
\end{equation*}
and (iii) $\phi(C)$ contains all $g-1+|\beta|$ points of $\ux$.


\begin{remarks}
This is exactly the same problem that we considered in
\cite{03.th-acz} and subsequent chapters.
In particular,
\cite[Theorem \ttref{T}]{03.th-acz}
applies to our present situation.
\par The condition that $I\alpha < (\antiK_\Delta \cdot H_\Delta)$ is
necessary because of Lemma~\ref{l:torCB}: if we impose all contact
points with $\antiK_\Delta$ to be assigned at general points, then
there is no curve at all.
\par The condition (i) that the curves are the Zariski closures of
their intersections with $X_\Delta \setminus \antiK_\Delta$ really
means that we count curves that do not contain any irreducible
component of the anticanonical cycle.
\end{remarks}


\subsection{Examples from degenerations of $K3$ surfaces}
\label{s:degenK3}


An emblematic situation where enumerative problems of the kind described
in Section \ref{s:enumpb} occur is when one undertakes the enumeration
of curves on $K3$
surfaces by considering type III degenerations, \eg degenerations of
$K3$ surfaces to unions of planes $X_0 \subset \P^N$ realizing a
triangulation of the sphere $\SS^2$ (by this we mean that the dual
complex of $X_0$ is the dual complex of a triangulation of $\SS^2$).
Such a degeneration in general has various relevant birational models,
see \cite{01.ciro},
all isomorphic one with another outside the central fibre.
Typically, as we shall illustrate below,
the irreducible components of the central
fibres of these
alternative degenerations are toric surfaces, with the anticanonical
cycle cut out by the other components of the central fibre.
The examples in \ref{sp:3A2}, \ref{sp:W_ij} and \ref{sp:12pts} below
show up when one considers a degeneration of quartic hypersurfaces in
$\P^3$ to a \emph{tetrahedron}, \ie the union of four general planes
in $\P^3$
(equivalently, there exist homogeneous coordinates
$(x\!:\!y\!:\!z\!:\!w)$
in which it is defined by the equation
$xyzw=0$).
We refer to \cite{quartiche} for a detailed study,
and to \cite[Section \ttref{ssec:quartiche}]{01.ciro} for a brief
discussion. 
The last example in \ref{sp:E4} shows up when one considers a
degeneration of octic $K3$ surfaces in $\P^5$
(\ie smooth complete intersections of three quadrics)
to an \emph{octahedron}, \ie the union of eight $2$-planes
in $\P^5$, the dual complex of which is a plain, Platonic, cube in
$\R^3$
(equivalently, there exist homogeneous coordinates
$(x\!:\!y\!:\!z\!:\!w\!:\!u\!:\!v)$
in which it is defined by the equations
$xy=zw=uv=0$).



\paragraph{A cubic surface with an anticanonical triangle}
\label{sp:3A2}
The surface $X_\Delta \subset \P^3$ corresponding to the Newton
polygon $\Delta$ below
\begin{center}
\includegraphics[height=1.5cm, trim=0 -1mm 0 -1mm]{3A2-N.eps}
\end{center}
is the cubic hypersurface $xyz=w^3$
in homogeneous coordinates
$(x\!:\!y\!:\!z\!:\!w)$.
Its anticanonical cycle $\antiK _\Delta$ is the triangle $xyz=w=0$.
The three sides of this triangle are the only lines contained in
$X_\Delta$; the surface $X_\Delta$ has an $A_2$ double point at
each vertex of $\antiK_\Delta$, and is smooth elsewhere.

Let us verify the type of singularity at the vertex at the bottom,
following the rule of \ref{p:sings}. One has
$u_v'=(1,1)$ and $u_v''=(-1,2)$, hence
$\orth [u_v'] = (-1,1)$ and $-\orth [u_v'']=(2,1)$.
We may take
$e_1 = (0,1)$ and $e_2=(-1,1)$, to the effect that
\[
  \orth [u_v'] = e_2
  \quad \text{and}
  \quad
  -\orth [u_v'']= 3 e_1 - 2e_2.
\]
The singularity corresponding to this vertex is of type
$\frac 1 3 (1,2)$, \ie an $A_2$ double point.

\par The linear system of hyperplane sections $|\O_{X_\Delta}(1)|$ may
be realized, much in the same way as in 
Example~\ref{ex:P2}, (b), above,
as the linear system of plane cubics with six base points
in the configuration indicated on the picture below.
On the picture, 
two successive blow-ups of $\P^2$ at three
points are drawn, with exceptional divisors $E_x, E_y, E_z$ and $E'_x,
E'_y, E'_z$ respectively; base points are
represented by black dots when they are proper, and arrows when they
are infinitely near. 
\begin{center}
\includegraphics[height=2.5cm]{3A2-blup.eps}
\end{center}
The three sides of $\antiK_\Delta$ are
the three $(-1)$-curves: $C_1=E'_y$, $C_2=E'_z$, and
$C_3 = E'_x$.
The cubic $X_\Delta$ is the main character of
\cite[Section \ttref{ssec:bad}]{01.ciro}.

Alternatively, the surface $X_\Delta$ may be realized as a
cyclic triple cover of $\P^2$ branched over a general triangle.

\par It turns out that, when considered as limits of hyperplane
sections of neighbouring quartic $K3$ surfaces, 
sections of a tetrahedron $X_0 \subset \P^3$
by a hyperplane passing through one of its vertices $v$ are best
substituted by
hyperplane sections of
the quartic $X_\Delta \cup \Pi_v \subset \P^3$, where
$\Pi_v$ is the face of $X_0$ opposite to $v$, identified with the
plane spanned by $\antiK_\Delta$ in such a way that the triangle cut
out on $\Pi_v$ by the three other faces of $X_0$ agrees with
$\antiK_v$.
In order to see this, one has to realize
the cubic $X _\Delta$ as some exceptional divisor living over $v$
in an appropriate blow-up of the total space of the degeneration
to $X_0$.
We refer to \cite{01.ciro} for details.

\par Correspondingly, one wants to enumerate genus $0$ hyperplane
sections of $X_\Delta$ matching with the divisor cut out on the
triangle $\antiK_\Delta$ by a general line in the span $\vect
{\antiK_\Delta}$. 
Such a divisor is made of three points, 
one on each of the three sides of the
triangle, that together impose only two independent linear conditions
on $|\O_{X_\Delta}(1)|$, in line with Lemma~\ref{l:torCB}.

To reduce to the enumerative problem \ref{p:enumpb}, one may
impose the passing through a fixed point on only two sides of
$\antiK_\Delta$, and let the intersection point with the third side
move freely. For instance, one may set $\alpha=(1,1,0)$ and
$\beta=(0,0,1)$.
The upshot of Lemma~\ref{l:torCB} is that this third point, although
free to move, will turn out to remain fixed.
About this trick, see also \cite[Paragraph~\ttref{p:logK3}]{03.th-acz}.

\par One may see that $N^\Delta_0 (\alpha,\beta)=3$ with the
topological formula giving the number of singular members in a pencil
of curves,
see \cite[Section~\ttref{s:pencil}]{10.th-panoramico}, as follows.
The two fixed points on $\antiK _\Delta$ (or
three aligned fixed points) define a pencil in
$|\O_{X_\Delta}(1)|$; this is a pencil of plane cubics, hence it has twelve
singular members, counted with multiplicities. There is a special
member in this pencil that corresponds to $\antiK _\Delta$ itself,
incarnated as its pull-back to the minimal desingularization of $X
_\Delta$, namely the $9$-gon in the picture above; it counts with
multiplicity $9$ among the singular members of the pencil. It follows
that there are $12-9=3$ irreducible $1$-nodal curves in this pencil.
We will confirm this number by solving the tropical counterpart of this
enumerative problem in \ref{sp:3A2-trop}.

\paragraph{}
\label{sp:W_ij}
Consider the surface $X _\Delta$ corresponding to the Newton polygon
depicted below.
\begin{center}
\includegraphics[height=2cm]{Wij-N.eps}
\end{center}
Its anticanonical cycle $\antiK _\Delta$ consists of two conics
$C_1,C_3$ corresponding to the sides $\Sigma_1,\Sigma_3$, and two
lines $C_2,C_4$ corresponding to the sides $\Sigma_2,\Sigma_4$.

Along a degeneration of quartic $K3$ surfaces to a tetrahedron
$X_0 \subset \P^3$, 
the sections of $X_0$ by a hyperplane containing one of its edges $W$
are best substituted by 
the hyperplane sections of $X_\Delta$ passing by two base points on
$C_1$ and two base points on $C_3$,
in order to be understood as limits of hyperplane sections of the
$K3$ surfaces neighbouring $X_0$.
The four base points on $C_1$ and $C_3$
are determined by the neighbouring quartic $K3$ surfaces,
as in \cite[Examples \ttref{ex:pi3} and \ttref{ex:K3}]{01.ciro};
they impose four independent conditions to the linear system
corresponding to $\Delta$, and therefore determine a $3$-dimensional
linear subsystem of
$|\O _{X_\Delta} (1)|$.
The latter can be realized as the linear system of plane quartics
with base points as indicated on the picture below
(with the same graphic convention as in \ref{sp:3A2};
there are four simple and one double proper base points, and four
infinitely near base points, all simple).
\begin{center}
\includegraphics[height=2.5cm]{Wij-blup.eps}
\end{center}
The projection map $\phi:X_\Delta \to \P^3$ from the four base points
contracts the two conics
$C_1$ and $C_3$ to two triple points, and identifies the two lines $C_2$
and $C_4$; its image is a rational quartic surface 
$X_W \subset \P^3$, with a
double line (the image of both $C_2$ and $C_4$),
two triple points on the latter
(the images of $C_1$ and $C_3$, respectively), and
no further singularity.
The rational quartic surface $X_W \subset \P^3$ is one of the relevant
degenerations of $K3$ surfaces alternative to the tetrahedron $X_0$;
in this perspective,
the double line of $X_W$ is reminiscent of the edge of $X_0$ opposite
to $W$. 
\par
Correspondingly, one wants to enumerate genus $0$ hyperplane sections
of $\phi(X_\Delta) = X_W$
passing through a general point of the double line
$\phi(C_2) = \phi(C_4)$.
This amounts to adding two more base points on $C_2$ and $C_4$
having the same image by $\phi$.
Equivalently,
these two base points together with the four on $C_1$ and $C_3$ 
only impose five independent linear conditions to
$|\O_{X_\Delta}(1)|$,
again in line with Lemma~\ref{l:torCB}.
To set up our enumerative problem in the terms of \ref{p:enumpb},
we fix the intersection with $C_2$, and let that with $C_4$ move
freely; in other words, we set 
$\alpha=(2,1,2,0)$ and $\beta=(0,0,0,1)$.
\par
By carefully analysing the geometry, one finds with
the Plücker formulae that
$N^\Delta _1 (\alpha, \beta) = 10$
and $N^\Delta _0 (\alpha, \beta) = 16$,
see \cite[Section~5.5]{quartiche}.
We will come back to this with a tropical point of view in
Example~\ref{sp:tropWij}.
For related floor diagram considerations, see
Examples \ref{ex:h-tr}, \ref{ex:h-tr2}, \ref{ex:h-tr3},
and \ref{sp:tropWij0}.

\paragraph{}
\label{sp:12pts}
Consider the $4$-Veronese surface $X_\Delta = v_4(\P^2)
\subset \P^{14}$,
corresponding to the triangle $\Delta = T_4$ as in \ref{ex:P2}.
The anticanonical cycle $\antiK_\Delta$ is the image by $v_4$ of the
triangle $xyz=0$ in $\P^2$.

Along a degeneration of quartic $K3$ surfaces to a tetrahedron $X_0
\subset \P^3$, 
to the limits of hyperplane sections of the general surfaces
tending to sections of $X_0 \subset \P^3$ by one of its faces $F$,
there correspond hyperplane sections of
$X_\Delta$ passing through twelve base points on $\antiK_\Delta$.
These base points are determined by the neighbouring surfaces
as in \cite[Examples \ttref{ex:pi3} and \ttref{ex:K3}]{01.ciro},
and together form the
image by $v_4$ of the divisor cut out on the triangle $xyz=0$ in
$\P^2$ by a general quartic curve.
As in \cite[Example \ttref{ex:logK3i}]{03.th-acz},
they impose only eleven independent
linear conditions to $|\O_{X_\Delta}(1)|$.
The projection of
$X_\Delta \subset \P^{14}$ from these twelve points is a quartic
surface $X_F \subset \P^3$,
with a triple point as a result of the contraction of $\antiK_\Delta$.
It is one of the relevant degenerations of $K3$ surfaces alternative
to the tetrahedron $X_0$.

Correspondingly, one wants to enumerate hyperplane sections of this
quartic surface $X_F \subset \P^3$ of genera $2,1,0$, respectively,
and passing through $2,1,0$ general points of $X_F$, respectively.
Again, to set this up as in \ref{p:enumpb}, we impose the passing
through only eleven out of the twelve base points. 
For instance, we set $\alpha=(4,4,3)$ and $\beta=(0,0,1)$.
\par
By degeneration, one finds
\begin{equation*}
N^\Delta_2(\alpha,\beta)=21;\quad
N^\Delta_1(\alpha,\beta)=132;\quad
N^\Delta_0(\alpha,\beta)=304,
\end{equation*}
\cf \cite[Theorem~3]{quartiche}.
Mikhalkin (private communication) has been able to find these numbers
with floor diagrams, but we won't do it in these notes.

% Together with Brugallé, we generalize this
% computation in CHAPTER IN THIS VOLUME.
% {\color{blue}Well, no longer I'm affraid.}



\paragraph{}
\label{sp:E4}
Consider the surface $X_\Delta \subset \P^4$ corresponding to the
polygon $\Delta$ represented below.
\begin{center}
\includegraphics[height=1.4cm]{E4-N.eps}
\hspace{.8cm}
\raisebox{.5cm}{$=$} 
\hspace{.8cm}
\includegraphics[height=1cm]{E4-Nalt.eps}
\end{center}
It is the quartic surface $xy-t^2=zw-t^2=0$
in homogeneous coordinates
$(x\!:\!y\!:\!z\!:\!w\!:\!t)$.
It has four ordinary double points and no
further singularity. Its anticanonical cycle $\antiK _\Delta$ is a
quadrilateral made of four lines, the vertices of which coincide with the
ordinary double points of the surface.
\par The linear system $|\O_{X_\Delta}(1)|$ may be thought of either
as a linear system of plane cubics with five base points
---~as indicated by the picture on the left~---, or
as a
linear system of curves of bidegree $(2,2)$ on $\P^1 \times \P^1$ with
four base points ---~as indicated by the picture on the right.
Alternatively, $X_\Delta$ may be realized as the double cover of $\P^1
\times \P^1$ branched over an anticanonical quadrilateral.

The quartic surface $X_\Delta \subset \P^4$ and the complete linear
system of its hyperplane sections is the key to understand the limits,
in terms of the theory expound in \cite{01.ciro},
of hyperplane sections of smooth surfaces degenerating to sections of 
some surface $X_0$ by a hyperplane passing through a point $v$, such
that $X_0$ has four irreducible components through $v$, all
$2$-planes, and the face of the dual complex of $X_0$ corresponding to
$v$ is a quadrilateral,
\eg $v$ is a vertex of an octahedron $X_0 \subset \P^5$.
This is analogous to the cubic $X_\Delta \subset \P^3$
of \ref{sp:3A2}
corresponding to sections of $X_0$ by a hyperplane passing through a
triple point formed by three $2$-planes, see
\cite[Section \ttref{ssec:bad}]{01.ciro}.

In this context,
the enumerative problem one needs to consider is that of counting
the hyperplane sections of $X_\Delta$ of genus $0$ intersecting
$\antiK_\Delta$ along a prescribed member of $|\O_{\antiKscr_\Delta}(1)|$;
such a divisor consists of four coplanar points, one on each side of
$\antiK_\Delta$.
% (Actually, also the sections of genus $-1$ come into
% play, but we do not enter into this here).
Correspondingly, one sets (for example) $\alpha=(1,1,1,0)$ and
$\beta = (0,0,0,1)$. One finds 
$N^\Delta _0(\alpha, \beta) =4$ in the same way as in \ref{sp:3A2}.
We will compute this number from the tropical perspective in
\ref{sp:E4-trop0}, see also
\ref{sp:E4-trop},
and using floor diagrams in \ref{sp:E4-floor}.




\section{From the torus to the tropics}
\label{S:tor-to-trop}


In this section we present \amoebae{} and tropical hypersurfaces.
The \amoeba{} of a hypersurface in the torus $(\C^*)^n$
has first been considered by
Gelfand--Kapranov--Zelevinsky in \cite{gkz}.
Non-archimedean \amoebae{} have been introduced by Kapranov, who
showed that they coincide with tropical hypersurfaces.


\paragraph{Am{\oe}ba of a hypersurface in a torus}
Let $X$ be a hypersurface of the torus $(\C^*)^n$. The
\emph{am{\oe}ba} of $X$ is the image
% $\Log (X)$
of $X$ by the logarithmic moment map
\begin{alignat*}{2}
\Log: &\quad & (\C^*)^n & \to \R^n \\[-1mm]
&& (z_1,\ldots,z_n) & \mapsto \bigl(
\log |z_1|,\ldots, \log |z_n|
\bigr).
\end{alignat*}
Pictured below is the \amoeba{} of a line in $(\C^*)^2$. From this you
should guess whence the name '\amoeba' came from.
\begin{center}
\includegraphics{amoeba.eps}
\end{center}

\paragraph{Limits of \amoebae}
One of the ideas at the origin of tropical geometry is to consider
limits of \amoebae{}.
To this effect, consider a hypersurface $X \subset (\C(t)^*)^n$, which
may be seen as a rational family of hypersurfaces in $(\C^*)^n$.
The $\C(t)$-points of $X$ are $n$-tuples $z(t)$ of rational functions
$(z_1(t),\ldots,z_n(t))$. Renormalizing, it is possible to consider
the limit of $\Log (z(t))$ at $t=0$, namely
\begin{equation*}
\lim _{t \to 0}
\frac 1 {\log |t|} \bigl(
\log |z_1(t)|,\ldots, \log |z_n(t)|
\bigr)
= \bigl( v(z_1),\ldots, v(z_n) \bigr),
\end{equation*}
where $v$ is the $t$-adic valuation, \ie for $f(t) \in \C(t)$, $v(f(t))$ is the integer $a$
such that one may write
$f(t) = t^a (\alpha+ \sum_{n=1}^{+\infty} \alpha_n t^n)$ for some
$\alpha \neq 0$.

The field $\C(t)$ however is not algebraically closed, so in general
$X$ doesn't have enough $\C(t)$-points, and the previous
considerations don't give a fully satisfactory definition of the limit
at $t=0$. The straightforward workaround to this issue is to replace
$\C(t)$ by its algebraic closure; another nice possibility is to work
over the field of Puiseux series
---~the latter being the algebraic closure of the field of formal
Laurent series $\C((t))$. Recall that a Puiseux series of the
variable $t$ and with coefficients in $\C$ is a formal power series of
the form
\begin{equation*}
f(t) = \sum _{n=n_0} ^{+\infty} \alpha_n t^{n/N}
\end{equation*}
for some $n_0 \in \Z$ and $N \in \N^*$.

The idea of taking limits of \amoebae{} is one inspiration for the
definitions in the following paragraph.



\paragraph{Non-Archimedean am{\oe}bae}
Let $\K$ be a valuated, non-Archimedean, algebraically closed field.
Being non-Archimedean means that $\K$ has some infinitely large
elements, \ie elements that are larger than all integers: in the
context of series in $t$ observed at $t=0$, these are the series with
negative $t$-adic valuation.
\par Precisely, we say that $\K$ is \emph{valuated non-Archimedean} if
it comes with a function
% \begin{equation*}
$v: \K^* \to \R$,
% \end{equation*}
the \emph{valuation}, such that
\begin{equation*}
\forall f,g \in \K^* :\quad 
% \left\{
% \begin{aligned}
v(fg) = v(f) + v(g), \quad\text{and} \quad
v(f+g) \geq \min \{ v(f),v(g) \}
\ \text{(if $f+g\neq 0$)}.
% \end{aligned}
% \right.
\end{equation*}
This determines a \emph{non-Archimedean norm}
$|\cdot|$, by setting
\begin{equation*}
|f|=
\begin{cases}
e^{-v(f)} & \text{if $f \in \K^*$}\\
0 & \text{if $f=0$.}
\end{cases}
\end{equation*}

Now, let $X \subset (\K^*)^n$ be a hypersurface.
The (non-Archimedean) \emph{\amoeba} of $X$ is, by definition,
its image by the
valuative moment map
\begin{alignat*}{2}
\Val: &\quad & (\K^*)^n & \longrightarrow \R^n \\
&& (x_1,\ldots,x_n) & \longmapsto \bigl(
v(x_1),\ldots,v(x_n)
\bigr).
\end{alignat*}
Pictured below is the \amoeba{} of a line in $(\K^*)^2$.
One way to think about it is
as the limit of the \amoebae{} of a rational family of
lines in $(\R^*)^2$,
\ie the limit as $t$ goes to $0$ of the \amoebae{} of
a family of lines defined by an equation
$a(t)x+b(t)y+c(t)=0$, where $a,b,c$ are rational functions in the
parameter $t$.
\begin{center}
\includegraphics{amoeba-trop.eps}
\end{center}

\begin{theorem}
[Kapranov\footnotemark, see \cite{kapranov-etal}]
\label{T:kapranov}
\footnotetext{this theorem has apparently appeared in a preprint of
  Kparanov only, in 2000;
  this preprint is referenced
  in \cite{mikhalkin-faces}
  for instance.}
Let $\K$ be a valuated, non-Archimedean, algebraically closed field,
and assume its valuation $v: \K^* \to \R$ is surjective.
\par Consider a hypersurface $X \subset (\K^*)^n$ defined by a
polynomial
\begin{equation*}
P(x) = \sum _{I \in \Supp(P)} a_I x^I
\end{equation*}
(\/$\Supp(P)$ is the support of $P$, \ie the set of those multi-indices
$I$ such that that coefficient of $P$ in the monomial $x^I$ is
non-zero).
\par The \amoeba{} of $X$ 
is the corner locus of the piecewise linear function
\begin{equation*}
p \in \R^n \longmapsto 
\max _{I \in \Supp(P)} \{ I \cdot p - v(a_I) \}.
\end{equation*}
\end{theorem}

The corner locus of a piecewise linear function $f:\R^n \to \R$ is the set
of walls in $\R^n$ separating the chambers on which $f$ equals a
unique linear function. We will come back to this notion in the next
section.

The theorem also holds in case the valuation is not surjective,
provided one takes the closure of the {\amoeba}. This typically happens
when $\K$ is the field of Puiseux series.


\paragraph{The tropical semi-field}
\label{trop-semifd}
Still applying the idea of taking the limit at $t=0$, one defines a
structure of semi-field on $\R$ as the limit of the usual field
structure. 
\par We consider the family indexed by $t \in \R_+^*$ of bijective maps
\[
\frac \log {\log t}: \R_+^* \to \R,
\]
and use it to degenerate the field structure on $\R$: One defines the
two operation laws $\boxplus$ and $\boxdot$ as the limits of $+$ and
$\cdot$ respectively, \ie for all $x,y \in \R$
\begin{equation*}
\begin{aligned}
 & x \boxplus y \overset{\text{def.}}=  \lim _{t \to 0^+}
\frac 1 {\log t}
\log \bigl((\log t))e^x + (\log t) e^y
\bigr)
= \max \{x,y\} \\
\text{and} \quad &
x \boxdot y \overset{\text{def.}}= \lim _{t \to 0^+}
\frac 1 {\log t}
\log \bigl((\log t))e^x \cdot (\log t) e^y
\bigr)
= x+y.
\end{aligned}
\end{equation*}
We call $(\R,\boxplus,\boxdot)$ the \emph{tropical semi-field}, and
denote it by $\T$. A convenient notation for the operations
$\boxplus$ and $\boxdot$ is to surround algebraic expressions by
quotation marks to indicate that they are meant in the tropical
semi-field. Thus, $\text{``}x+y\text{''} = x \boxplus y$
and $\text{``}xy\text{''} = x \boxdot y$.


\paragraph{Tropical polynomials and hypersurfaces}
\label{p:trop-hypsce}
The definition of a {tropical polynomial} (function) is
pretty straightforward, 
one just replace the ordinary algebraic expression by its counterpart
in the tropical semifield.
Thus, a \emph{tropical polynomial} is a function $P:\T^n \to \T$ 
defined by an expression of the form
\begin{align*}
P(x_1,\ldots,x_n) &= 
\scalebox{1.4}{``}\,\sum_I a_I x^I
\,\scalebox{1.4}{''}
= \raisebox {-.5em} {$\underset I {\scalebox{2}{$\boxplus$}}$}
\, (a_I \boxdot x^{\boxdot I}) \\
& = \max_I \{ a_I + i_1 \cdot x_1 + \cdots i_n \cdot x_n \},
\end{align*}
where the sum is taken on a finite set of multi-indices.

It does not make much sense to consider the zero locus of a function
as above. Instead, a \emph{tropical hypersurface} in $\T^n$ is by
definition the corner locus of a tropical polynomial.

\bigskip
With these definitions, the content of 
Theorem~\ref{T:kapranov} is that 
{\amoebae} of hypersurfaces in $(\K^*)^n$ and tropical hypersurfaces
in $\T^n$ ($\R^n$, if one prefers) are the same objects.


\section[Parabolic polarity, b.k.a.\
Legendre--Fenchel duality]
{Parabolic polarity\footnotemark, b.k.a.\
  Legendre--Fenchel duality}
\label{s:legendre}
\footnotetext{about this name,
  imagined (but not used) by Fenchel,
  see \cite[p.~247]{hull}.}


This section is about what is often called Legendre transformation.
A nice reference is \cite[Part E]{hull}.
For the case of twice differentiable functions, a classical reference
is \cite[Section 14]{arnold}.

\begin{definition}
Let $f: \R^n \to \R$ be a function.  The \emph{Legendre--Fenchel
  transform} of $f$ is the function
\begin{equation*}
\begin{aligned}
\dual f: \quad \check \R^n & \to \R \\[-1.5mm]
p & \mapsto \sup _{x \in \R^n} \bigl\{ p\cdot x - f(x) \bigr\},
\end{aligned}
\end{equation*}
where $\check \R^n$ is the dual of\/ $\R^n$.
\end{definition}

\noindent
The definition is intended for all
functions defined on a subset $U$ of $\R^n$,
so in fact the supremum in the definition is to be taken on
all $x \in U$ only.

In fact we don't allow $\dual f$ to take the value $+\infty$,
and thus $\dual f$ is in general only defined on a subset of
$\check \R^n$.
To make sure that $\dual f$ is defined on a non-empty subset of
$\check \R^n$, one may assume that there exists an affine function $m$
such that $m \leq f$.
We make this assumption from now on and for the
rest of the section; it is true in particular if $f$ is convex.

The Legendre--Fenchel transform is always a closed convex function,
see \cite[Example B.2.1.3]{hull}.
The Legendre--Fenchel transformation is involutive on closed convex
functions. More precisely, for all functions $f$, the ``bi-conjugate''
$\dual [\dual f]$ is the closed convex hull of $f$,
see \cite[Theorem E.1.3.5]{hull}.
By definition, the closed convex hull of $f$ is obtained by
considering the epigraph $\mathrm{epi}(f)$
(\ie the part of $\R^n\times \R$ lying above the graph of $f$),
taking the closed convex hull
$\overline{\mathrm{co}}\, \mathrm{epi} (f)$ of the latter,
and finally taking the unique function of which this is the epigraph;
in other words, it is the function
\[
  x \mapsto \inf
  \bigl\{
  y:
  (x,y) \in \overline{\mathrm{co}}\, \mathrm{epi} (f)
  \bigr\}.
\]


\paragraph{Link with projective duality}
\label{p:leg-projdual}
Consider a strictly convex function $f: \R^n \to \R$ that is twice
differentiable
(thus, $f''>0$).
Then, for all linear functional $p \in \check \R^n$, the
supremum of all $p\cdot x - f(x)$ is attained at a unique point
$x(p) \in \R^n$, which may be characterized as the unique $x \in \R^n$
such that the tangent space to the graph of $f$ at the point
$(x,f(x))$ has slope $p$; moreover, the equation of this very tangent
space is 
\[
y= p\cdot x - \dual f (p).
\]
Therefore, the points of the graph of the Legendre--Fenchel transform
$\dual f$ naturally correspond to the tangent spaces of the graph of
$f$: this is an instance of projective duality!
(see \cite{13.th-classic}).
\begin{center}
\includegraphics[height=3.0cm, trim= 0 -1mm 0 -2mm]{legendre-dual.eps}
\end{center}

The Legendre--Fenchel transformation is also linked with classical mechanics,
hence the notation '$p$' for linear functionals.
Luckily enough, the letter 'p' can also stand for \emph{pente} and
\emph{pendenza} (French and Italian for slope).

\paragraph{}
For convex piecewise affine functions, there is an interpretation
akin to that of \ref{p:leg-projdual}.
In this context,
the Legendre--Fenchel transformation exchanges,
loosely speaking,
the roles of the corner loci and the slopes; this is perhaps best
understood by looking at the figure below, which pictures the graphs
of a piecewise affine linear function (defined on a finite interval)
and its Legendre--Fenchel
transform (defined on the whole $\R$).
It is elementary to check that things indeed happen as on the picture,
and that taking the Legendre--Fenchel transform of the function on the
right gives back the function on the left; I of course encourage the
reader to try it for him or herself.
\begin{center}
\includegraphics[height=3.0cm, trim=0 0 0 -2mm]{pieclin.eps}
\hspace*{1cm}
\raisebox{15mm}{$\leadsto$}
\newlength{\lleadsto}
\settowidth{\lleadsto}{$\leadsto$ \reflectbox{$\leadsto$}}
\hspace{-\lleadsto}
\raisebox{10mm}{\reflectbox{$\leadsto$}}
\hspace*{1cm} 
\includegraphics[height=3.0cm, trim=0 0 0 -2mm]{pieclin-tf.eps}
\end{center}

There is a similar story for functions $f$ defined at finitely many points
$x_1,\ldots,x_n$ only.
In this case, the Legendre--Fenchel transform is a convex piecewise
affine function defined on the whole dual space,
and the bitransform is a convex piecewise
affine function defined on the convex hull of $x_1,\ldots,x_n$, and
characterized by the fact that its graph is the bottom of the convex
hull of the graph of $f$.
Consider for instance the restriction to $\{x_1,x_2,x_3\}$ of the
function on the left in the above figure. Its transform is the
function on the right of the picture, and its bi-transform is the
function on the left itself. This is again elementary to check.



\paragraph{Application to tropical geometry}
\label{p:Legendre-for-tropical}
In the context of Theorem \ref{T:kapranov}, the function
$p \in \R^n \mapsto 
\max _{I \in \Supp(P)} \{ I \cdot p - v(a_I) \}$
is the Legendre--Fenchel transform of the function
\begin{equation}
%\label{eq:valfun}
  v_P: I \in \Supp(P) \mapsto v(a_I).
\end{equation}
Therefore the above discussion shows that, dual to the \amoeba{}
of $X$, which may be seen as a subdivision of $\R^n$ into convex
polytopes, there is a subdivision of the Newton polytope
$\Delta(P)$ of $P$ (\ie the convex hull of $\Supp(P)$) into convex
polytopes, given by the corner locus of the real-valued function on
$\Delta(P)$ obtained by ``extending by convexity'' the function
$v_P$,
\ie of the closed convex hull $\bar v_P$ of $v_P$.
In other words, the tiles of this subdivision of $\Delta(P)$ are the
maximal polytopes on which the function $\bar v_P$ is affine.




\section{Tropical curves}
\label{S:trop-curves}

In this section we introduce plane tropical curves, following
Mikhalkin, first as rational piecewise linear objects in $\R^2$,
which we will see coincide with the tropical hypersurfaces that
have been presented in Section \ref{S:tor-to-trop}, and then as
images of abstract tropical curves by tropical maps.
Beware not to confuse the graphs that we use here in order to support
our definitions of tropical curves with those used in Section
\ref{S:floors} to define floor diagrams; floor diagrams are purely
combinatorial objects retaining only some information of plane
tropical curves, the latter being geometric objects in nature.

\subsection{Plane tropical curves}

\begin{definition}
\label{def:plane-trop}
A \emph{plane tropical curve} is a rational, piecewise linear, real
curve $C \subset \R^2$, which is a balanced topological incarnation of
a finite graph $\Gamma$ equipped with a weight function
$w: \edg(\Gamma) \to \N^*$,
by which we mean that conditions
\eqref{cond:linpiece}--\eqref{cond:balance} below hold.
\end{definition}


\begin{inparaenum}[(i)]
\item
\label{cond:linpiece}
The curve $C$ is the union of finitely many linear pieces
(\ie segments, semi-lines, or (rarely) lines)
with rational slopes, and these linear pieces
are in bijective
correspondence with the edges of $\Gamma$.
Each such linear piece has two ends, possibly at infinity (one end at
infinity for a semi-line, two for a line),
and the ends of the linear pieces of $C$
are in bijective correspondence with the
vertices of $\Gamma$; moreover, the ends at infinity are in bijective
correspondence with the $1$-valent vertices of $\Gamma$.
Beware that points at infinity are not intended in the usual sense
of projective geometry (rather, see Remark \ref{rk:trop-P2}): 
lines have two ends at infinity, and 
disjoint parallel lines do not meet at infinity.

\smallskip
We may speak about the edges and vertices of a tropical curve
to denote their incarnations in $\R^2$ or as points at
infinity.
We call vertices at finite distance (resp., at infinity) of $C$ the
vertices of $\Gamma$ that are actually incarnated as points in $\R^2$
(resp., incarnated as points at infinity). Equivalently, the vertices
at infinity of $C$ are the $1$-valent vertices of $\Gamma$, and the
vertices at finite distance are the others.

\smallskip
\item
Any two linear pieces $C_1$ and $C_2$ of $C$ intersect properly and at
their ends, \ie
if non-empty, the intersection $C_1 \cap C_2$ is a single point,
which must be an end of both $C_1$ and $C_2$.

\item
\label{cond:corner}
Any two linear pieces $C_1$ and $C_2$ of of $C$ with the same slope
may intersect 
only if there is at least a third edge ending at $C_1 \cap C_2$.

\smallskip
For each vertex $v$ and edge $\Sigma$ ending at $v$ 
(we write $v \in \Sigma$ for this condition), we denote by
$u_{v,\Sigma}$ the primitive (see \ref{p:notation})
integral vector $(a,b) \in \Z^2$ that
has the same direction as the linear piece of $C$ corresponding to
$\Sigma$, 
and is oriented from $v$ to the other end of $C$.
We also let $u_{\Sigma,v}$ be
$-u_{v,\Sigma}$. 

\smallskip
\item 
\label{cond:balance}
\emph{(Balancing condition)\/}
For each plurivalent vertex $v$, one has
\begin{equation}
\label{eq:balance}
\sum _{\Sigma \ni v} w(\Sigma) \cdot u_{v,\Sigma} = 0.
\end{equation}
\end{inparaenum}

\smallskip
Note that conditions \eqref{cond:corner} and \eqref{cond:balance}
imply that the vertices of a plane
tropical curve have valence either $1$, or at least $3$.


\paragraph{Examples}
\label{p:ex-plane-trop}
Examples of plane tropical curves are pictured on the left in
Figures \ref{fig:ex:trop-curve1}
and \ref{fig:ex:trop-curve2}.
%the figures below.
The weight of an edge
is indicated as a circled integer, only if it is larger than one.
The grids on the pictures are drawn so that one can easily read the
rational slopes, but they do not mean that the vertices are integral
points, which indeed is not requested in the definition of plane
tropical curves. 

\begin{figure}[htb]
\centering
\noindent
\begin{minipage}[b][][b]{0.49\linewidth}
\noindent
\hfill
\includegraphics[height=4cm]{courbe1.eps}
\hfill
\raisebox{9mm}{\includegraphics[height=2cm]{courbe1N.eps}}
\hfill\phantom{p}
\captionof{figure}{}%{Example of tropical curve}
\label{fig:ex:trop-curve1}
\end{minipage}
\begin{minipage}[b][][b]{0.49\linewidth}
\noindent
\hfill
\raisebox{9mm}{\includegraphics[height=2cm]{courbe2.eps}}
\hfill
\raisebox{9mm}{\includegraphics[height=2cm]{courbe2N.eps}}
\hfill\phantom{p}
\captionof{figure}{}%{Example of tropical curve}
\label{fig:ex:trop-curve2}
\end{minipage}
\end{figure}


\begin{theorem}[Mikhalkin {\cite[Section 2.1]{mikhalkin-pants}}]
Plane tropical curves as defined in \ref{def:plane-trop} are exactly
the hypersurfaces of the tropical plane $\T^2$,
\ie the corner loci of tropical polynomials, as defined in
\ref{p:trop-hypsce}. 
\end{theorem}

The main content of this theorem is that the balancing condition 
\eqref{eq:balance} characterizes tropical hypersurfaces.
To make this statement work,
one needs to equip the corner locus of a tropical polynomial
with a weighting. This has been introduced by Mikhalkin, and
goes as follows.
Let $\Sigma$ be an edge of the corner locus of some tropical
polynomial. Then $\Sigma$ is a corner between the graphs of two affine
functions
$a+ix+jy$ and $b+kx+ly$ with rational slopes.
By definition, the \emph{weight} of $\Sigma$ is the integral distance
between the two integral points $(i,j)$ and $(k,l)$ in $\check \R^2$,
\ie the number of integral points on the segment
$\bigl[
(i,j), (k,l)
\bigr]$
minus one, which we have denoted by
$\ell_\Z \bigl[
(i,j), (k,l)
\bigr]$
in Section \ref{s:toric-surf}.

\paragraph{Newton polygon of a plane tropical curve}
\label{p:trop-Newton}
Let $C \subset \R^2$ be a tropical curve, and consider the list
$(\Sigma_1,\ldots,\Sigma_n)$ of its infinite edges, as a list ordered
up to cyclic permutation, as follows:
(a) an edge is \emph{infinite} if
it has infinite Euclidean length in $\R^2$, equivalently if it has
at least one end that is a vertex at infinity;
(b) the order on
the set of infinite edges is defined by drawing a circle of
sufficiently large
radius, so that it intersects $C$ at exactly one point on each infinite
edge and nowhere else; then the order is that of the intersection
points on the circle according to the orientation of $\R^2$.

%\sloppy
Starting at an arbitrary integral point of $\R^2$, draw
successively the vectors $w(\Sigma_1). u_{\Sigma_1,\infty}^\perp,
\ldots,\allowbreak w(\Sigma_n). u_{\Sigma_n,\infty}^\perp$, so that
when one vector is drawn, the next one starts where the previous
one ended; for all infinite edges $\Sigma$, the vector
$u_{\Sigma,\infty}$ is the unitary direction vector of $\Sigma$
oriented towards the end at infinity.
It is a consequence of the balancing condition that this circuit
of vectors is a closed path, and actually a convex integral polygon.
We call it the \emph{Newton polygon} of $C$.

\medskip
\subparagraph*{Examples}
For each example of plane tropical curve in
\ref{p:ex-plane-trop},
the corresponding Newton polygon is indicated next to it, on the
right.
The subdivision corresponds to the following construction.


\paragraph{Subdivision of the Newton polygon}
Going on with the same idea as in \ref{p:trop-Newton}, one may enhance
the Newton polygon of a plane tropical curve with a subdivision.
This subdivision is dual to the subdivision of $\R^2$ defined by the
tropical curve,
as we have seen in \ref{p:Legendre-for-tropical}
using the Legendre--Fenchel transformation.

\par Let $C\subset \R^2$ be a tropical curve, and $v$ one of its
vertices. We consider the list $(\Sigma_1,\ldots,\Sigma_n)$, ordered
up to cyclic permutation, of the edges ending at $v$.
Because of the balancing condition at $v$, drawing successively the
vectors $w(\Sigma_1)\cdot u_{v,\Sigma_1}^\perp,
\ldots, w(\Sigma_n)\cdot u_{v,\Sigma_n}^\perp$ builds an integral
convex polygon $\Delta_v$.
\par There is a canonical way of arranging all the $\Delta_v$ together
as a polygonal decomposition of the Newton polygon $\Delta$ of
$C$. Indeed, each edge $\Sigma$ of $C$ has two ends $v_1$ and $v_2$,
hence determines a glueing of $\Delta_{v_1}$ and $\Delta_{v_2}$ along
the segments of their boundaries supported along
$w(\Sigma)u_{v_1,\Sigma}$ and 
$w(\Sigma)u_{v_2,\Sigma}$, respectively (if $v$ is a vertex at
infinity, then $\Delta_v$ is the Newton polygon $\Delta$).
This is the subdivision we are interested in.

\medskip
\subparagraph*{Examples}
For each plane tropical curve in \ref{p:ex-plane-trop}, the Newton
polygon is indicated with its subdivision pictured.


\paragraph{Subdivisions and degenerations}
\label{specule-degen}
To a subdivision of a lattice polygon $\Delta$ into a tiling of
lattice polygons as above, one may associate a ``reducible toric
surface'' with 
the same degree and embedding dimension as $X_\Delta$, see below.
In fact, such a reducible toric variety (in any dimension) may be
realized as a toric degeneration of $X_\Delta$, see, \eg
\cite[Section 3]{nishinou-siebert}.
It is then natural (in hindsight!) to expect that plane tropical
curves with the same 
subdivised polygon $\Delta$ are related to this degeneration.
This has first been realized by Viro
\cite{viro}, who establishes this relation
by means of his patchworking construction.
Pursuing this idea, Shustin explains in \cite{shustin}
(see also \cite[Chapter 2]{tropicalOW}) that the two processes of
tropicalization and patchworking are somehow inverse to each other
(one can think of them as degeneration and deformation, respectively),
and as an application he gives an alternative proof of Mikhalkin's
Correspondence Theorem \ref{t:M-corresp}.
The relation of plane tropical curves with toric degenerations of the
projective plane is also illustrated in Paragraph \ref{p:trop-erwan}, 
following \cite{erwan-11}.

Now, the reducible toric variety defined by a subdivision of a lattice
polytope $\Delta$ is the following:
its irreducible components are the various
$X_{\Delta_v}$ corresponding to the various tiles $\Delta_v$ of the
subdivision of $\Delta$, and these are glued along toric varieties of
smaller dimensions,
according to the dual graph of the subdivision of $\Delta$.
Let me simply give an example
instead of making a formal definition.
Consider the subdivised polygon $\Delta$ from Figure
\ref{fig:ex:trop-curve2}. The polygon $\Delta$ is the
triangle $T_2$ of \ref{ex:P2}, which defines the $2$-Veronese surface
$X_\Delta \subset \P^5$, of degree $4$.
The trapezium in the subdivision
is a $T^1_{1,2}$
in the notation of \ref{sp:trapezium}, and thus defines a degree $3$
rational normal scroll $X_1 \subset \P^4$, built on a line $X_{1,2}$
and a conic spanning two supplementary linear spaces $\P^1$ and $\P^2$ in
$\P^4$, such that the line $X_{1,2}$ corresponds to the intersection
of the two tiles of the subdivision.
We may view the $\P^4$ spanned by $X_1$ as a linear subspace in $\P^5$.
The triangle in the subdivision defines a plane $X_2 = \P^2$. We may
view this $\P^2$ as a linear subspace of $\P^5$, intersecting the
$\P^4$ spanned by $X_1$ exactly along the $\P^1$ spanned by the line
$X_{1,2}$.
Then, the reducible toric surface corresponding to the subdivision is
the union $X_1\cup X_2 \subset \P^5$, where $X_1 \cap X_2 = X_{1,2}$.


\subsection{Abstract tropical curves and tropical maps}
\label{s:param-trop-curve}

The definitions in this section are due to Mikhalkin
\cite{mikhalkin-JAMS}.

\begin{definition}
\label{d:abs-trop-curve}
An \emph{abstract tropical curve} is the data of a finite graph $\bar
\Gamma$ without isolated vertex, together with a complete metric $g$
on $\Gamma
\overset{\text{def.}}= \bar \Gamma \setminus \Gamma ^\infty$, where $\Gamma
^\infty$ is the set of vertices of\/ $\Gamma$ having valence $1$.
\end{definition}

The condition on the completeness of the metric means that every edge
of $\Gamma$ should be isometric either to a segment, a semi-line, or a
line, depending on how many ends at infinity it has.

A tropical curve $(\bar \Gamma, g)$ is said to be \emph{irreducible}
if the space $\bar \Gamma$ is connected. The \emph{arithmetic genus}
$p_a (\bar \Gamma, g)$ of
$(\bar \Gamma, g)$ is defined by the first Betti number of $\bar
\Gamma$
(and/or its topological Euler--Poincaré characteristic)
as
\begin{equation*}
p_a (\bar \Gamma, g)
\overset{\text{def.}}{=}
1 - \chi_\top(\bar\Gamma)
= b_1(\bar \Gamma) - n +1,
\end{equation*}
where $n$ is the number of connected components of $\bar\Gamma$.


\begin{definition}
\label{d:param-trop-curve}
A \emph{tropical morphism} from an abstract tropical curve $(\bar
\Gamma, g)$ to the tropical plane is a continuous map
$f: \Gamma \to \R^2$ such that: (i) the restriction of $f$ to each
edge is affine integral; and (ii) the balancing condition holds at
every vertex at finite distance.
\end{definition}


Some more precision is in order. Let $\Sigma$ be an edge of
$\Gamma$. The restriction of $f$ to $\Sigma$ is
\emph{affine integral}
if (i) the image $f(\Sigma) \subset \R^2$ is supported on a line
directed by an integral unitary vector $u_\Sigma$, and
(ii) the differential $df_\Sigma$ is $\Z$-linear with respect to the
integral structure on the tangent spaces defined by $g$ and $u_\Sigma$
respectively; 
the absolute value of the $\Z$-linearity factor of $df_\Sigma$ is
called the \emph{stretching factor}, and denoted by $w_{\Sigma, f}$.

Let $v$ be a plurivalent vertex of $\Gamma$. The balancing
condition at $v$ is
\begin{equation*}
\sum _{\Sigma \ni v} w_{\Sigma,f} \cdot u_{v,\Sigma} =0,
\end{equation*}
where as before $u_{v,\Sigma}$ is the unitary direction vector for
$f(\Sigma)$ directed from $v$ to the other end.

\begin{example}
\label{ex:abstract}
Two abstract tropical curves are pictured on Figure
\ref{fig:abstract}, of genera $1$ and $0$, respectively. 
They both admit a tropical morphism to the plane tropical curve
pictured on Figure \ref{fig:img-of-abs}.

\begin{figure}[htbp]
\centering
\begin{minipage}[b]{\textwidth/2-1mm}
\centering
\raisebox{1.6cm}{(a)}
\includegraphics[height=2cm]{abstracta.eps}
\hspace{5mm}
\raisebox{1.6cm}{(b)}
\includegraphics[height=2cm]{abstractb.eps}
\captionof{figure}{}
\label{fig:abstract}
\end{minipage}
\hfill
\begin{minipage}[b]{\textwidth/2-1mm}
\centering
\includegraphics[height=22mm]{abstract.eps}
\hspace{5mm}
\includegraphics[height=18mm]{abstractN.eps}
\captionof{figure}{}
\label{fig:img-of-abs}
\end{minipage}
\end{figure}

% \begin{center}
% \raisebox{1.6cm}{(a)}\quad
% \includegraphics[height=2cm]{abstracta.eps}
% \hspace{2cm}
% \raisebox{1.6cm}{(b)}\quad
% \includegraphics[height=2cm]{abstractb.eps}
% \end{center}
% \begin{center}
% \includegraphics[height=2.5cm]{abstract.eps}
% \hspace{2cm}
% \includegraphics[height=1.5cm]{abstractN.eps}
% \end{center}
\end{example}


\paragraph{} 
If $C$ is an abstract tropical curve with a tropical morphism $f$ to
the plane, one defines the \emph{Newton polygon} of the map $f$,
denoted by $\Delta(C,f)$, as the Newton polygon of the plane tropical
curve image of $C$ by $f$; as such, it comes with a subdivision.
\par Actually, it is not completely straightforward how to define the
image $f(C)$ as a plane tropical curve, as it may involve the adding
of new vertices (at finite distance).
This happens for instance in Example~\ref{ex:abstract}: the
image curve must have the vertex $\#6$ since, by definition, two edges
may only intersect at a vertex, see \ref{def:plane-trop});
thus in case (b) the graph has to be modified.

\paragraph{Geometric genus and resolutions}
\label{p:gen-resol}
So far we have defined the arithmetic genus of an abstract tropical
curve; 
one may next want to define the geometric genus of a plane tropical
curve as the arithmetic genus of its normalization, as 
in algebraic geometry.
However, it is not clear how to appropriately define the
normalization.
One may instead define the \emph{geometric genus} of a plane tropical curve
$C \subset \R^2$ as the smallest possible arithmetic genus of all
abstract tropical curves $\Gamma$ such that there exists a tropical map
$f:\Gamma \to \R^2$ mapping $\Gamma$ to $C$.
In general, it is arguably best to proceed as in
the theory of stable maps and, instead of considering the geometric
genus of a plane tropical curve itself, to consider the genus of a map from
an abstract tropical curve to it, defined
as the genus of the source curve.

\paragraph{Geometric genus and singularities}
\label{p:sings-gen}
Alternatively, there is in principle
the possibility of defining the geometric
genus of a plane curve $C$ as its arithmetic genus
(defined as the number of integral points in the interior of its
Newton polygon, as in \ref{sp:p_a}),
minus some corrections determined by its singularities
(the latter concept yet to be defined).
It is however delicate to give a general definition along these lines,
and we shall therefore only consider plane curves of a particular shape.
It will follow from Proposition \ref{pr:trop-AVZ} that this limited
range of shapes is in general sufficient in view of the tropical
enumerative problem we will be interested in.

Let $C$ be a plane tropical curve, and assume that
it is reduced\footnote
{a plane tropical curve is \emph{reduced} if it cannot be written as
  the sum of two non-empty plane tropical curves $C_1$ and $C_2$ such
  that the support of $C_2$ is contained in the support of $C_1$.},
and that the tiles of the
subdivision of its Newton polygon $\Delta$ are all triangles and
parallelograms.
The latter condition means that
all vertices at finite distance of $C$ are either
trivalent or look like the crossing of two lines
(like vertex $6$ on Figure \ref{fig:img-of-abs}).
Then, define the \emph{$\delta$-invariant} of $C$ as
\[
  \delta(C) =
  \sum_{e \text{ finite segment of } C}
  \bigl( w(e)-1\bigr)
  + \sum_{\substack{v \text{ vertex of } C:\\
      \Delta_v \text{ parallelogram}}}
  \Ar(\Delta_v)
  + \sum_{\substack{v \text{ vertex of } C:\\
      \Delta_v \text{ triangle}}}
  p_a(\Delta_v)
\]
where $w$ is the weight, $\Ar$ is the Euclidean area,
and $p_a(\Delta_v)$ is the arithmetic genus of the lattice polygon
$\Delta_v$, defined as in \ref{sp:p_a} as the number of integral
points in its interior.
A \emph{finite segment} of $C$ is a maximal connected linear subset of
$C$ having its two ends at finite distance; this corresponds to a
maximal chain of parallelograms
(in the sense of footnote \ref{ft:chain-parallel} below)
in the subdivision of $\Delta$ such that none of the extremal
edges in the corresponding sequence of parallel edges lies on the
boundary of $\Delta$. 
Note that a finite segment of $C$ is in general a chain of finitely
many edges, all supported on the same line, and all having the same
weight; the weight of the finite segment is this common weight.

The above definition of $\delta(C)$ is equivalent to the
following. 
Let $v$ be a vertex of $C$, and let $\Delta_v$ be the corresponding
lattice polygon in the subdivision of $\Delta$. An edge $\sigma$ of
$\Delta_v$ is said to \emph{border} $\Delta$ if it is linked to an
edge in the boundary of $\Delta$ by a (possibly empty) chain of
parallelograms\footnote
{\forcelabel{footnote}{ft:chain-parallel}
two segments $\sigma$ and $\sigma'$ are
  \emph{linked by a chain of parallelograms}
  if they are parallel and there exist parallelograms
  $\Delta_{v_1},\ldots,\Delta_{v_n}$ in the subdivision of $\Delta$
  such that $\sigma$ and $\sigma'$
  are edges of $\Delta_{v_1}$ and $\Delta_{v_n}$ respectively and,
  for all $i=1,\ldots,n-1$, $\Delta_{v_i}$ and $\Delta_{v_{i+1}}$ are
  adjacent along an edge parallel to $\sigma$ and $\sigma'$.
}.
For example,
for the subdivision on Figure \ref{fig:img-of-abs}, in addition to the
edges directly lying on the boundary of $\Delta$, the left edge of
triangle $1$ and the bottom edge of triangle $5$ border $\Delta$.
Recall that $\lz(\sigma)$ denotes the integral length of $\sigma$, \ie the
number of integral points on $\sigma$ minus one.
Then, we let
\[
  \delta(v) =
  \begin{cases}
    p_a(\Delta_v) +
    \frac 1 2 \sum _{
         \substack{\sigma \text{ edge of } \Delta_v\\
           \text{not bordering }\Delta
         }
       }
       \bigl(\lz(\sigma)-1\bigr)
    & \text{if } \Delta_v \text{ triangle}
    \\
    \Ar(\Delta_v)
    & \text{if } \Delta_v \text{ parallelogram},
  \end{cases}
\]
and $\delta(C)$ be the sum of $\delta(v)$ over all vertices at finite
distance of $C$.

Finally,
we define the \emph{geometric genus} of $C$ as its arithmetic genus
$p_a(\Delta)$ minus its $\delta$-invariant $\delta(C)$.
This is coherent with our previous definition by Lemma \ref{l:genus} below.


\begin{examples}
With the above definitions,
the plane tropical curve in Example~\ref{ex:abstract} has arithmetic
genus $1$ and geometric genus $0$.
There are tropical maps to this plane tropical curve from the two
abstract tropical curves (a) and (b), having genus $1$ and $0$,
respectively. Note that vertex $\#6$, which gives the only non-trivial
contribution to the $\delta$-invariant of the plane curve, does not
appear in the abstract curve (b).

The plane tropical curves on Figure \ref{fig:trop-3ique-w2}
and \ref{fig:trop-3ique-nonrat}
have
arithmetic genus one and geometric genus zero. The only non-trivial
contribution to the $\delta$-invariant of the curve on
Figure \ref{fig:trop-3ique-w2}
(resp., Figure \ref{fig:trop-3ique-nonrat})
is from its weight two edge
(resp., from the vertex with associated polygon the triangle with an
integral point in its interior).

\begin{figure}[htbp]
\centering
\begin{minipage}[b]{\textwidth/2-1mm}
\centering
\includegraphics[align=c,height=30mm]{cubique-abis-shape.eps}
\hspace{10mm}
\includegraphics[align=c,height=20mm]{cubique-abis-subdiv.eps}
\captionof{figure}{}
\label{fig:trop-3ique-w2}
\end{minipage}
\hfill
\begin{minipage}[b]{\textwidth/2-1mm}
\centering
\includegraphics[align=c,height=30mm]{cubique-ater-shape.eps}
\hspace{10mm}
\includegraphics[align=c,height=20mm]{cubique-ater-subdiv.eps}
\captionof{figure}{}
\label{fig:trop-3ique-nonrat}
\end{minipage}
\end{figure}

The plane tropical curve on Figure \ref{fig:quartique-delta} has
arithmetic genus three and geometric genus zero. The vertical weight two
 finite segment contributes by one to the $\delta$-invariant,
and its crossing with another edge contributes by two.

\begin{figure}[htbp]
\centering
\includegraphics[height=40mm]{quartique-delta.eps}
\hspace{10mm}
\raisebox{5mm}
{\includegraphics[height=20mm]{quartique-delta-subdiv.eps}}
\caption{}
\label{fig:quartique-delta}
\end{figure}

\end{examples}


\begin{remark}
\label{rk:sings-trop-v-alg}
Remembering that tropical curves are in essence limits of families of
curves, 
one way to look at the above definition of the $\delta$-invariant
%in \ref{p:sings-gen}
is in terms of the description of the limit of Severi
varieties given in
\cite[Section \ttref{s:Severi-1}]{01.ciro}.
A plane tropical curve $C$ with Newton polygon $\Delta$
encodes data about
limits $C_0$ of algebraic curves $C_t$
along a degeneration of the toric surface
$X_\Delta$ into a union of the surfaces $X_{\Delta_v}$ over all vertices
$v$ of $C$, as mentioned in Paragraph \ref{specule-degen}.
For each vertex $v$, the curve $C_0 \cap X_{\Delta_v}$ may have up to
$p_a(\Delta_v)$ (resp., $\cA(\Delta_v)$)
nodes off the toric boundary of $X_{\Delta_v}$
if $\Delta_v$ is a triangle (resp., a parallelogram), and each of
these nodes may be the limit of a node on the curves $C_t$.
Moreover, for each finite segment $e$ of weight $w$ of $C$,
the curve $C_0$ may have up to a $w$-tacnode along the intersection 
$X_{\Delta_v}\cap X_{\Delta_{v'}}$, where $v$ and $v'$ are the two
ends of $e$
(if $e$ is made of several edges, this has to be taken with a grain of
salt, see \cite[Paragraph \tref{p:lim-nodes}]{07.th-diag-degen});
each such $w$-tacnode may be the limit
of $w-1$ nodes on the curves $C_t$.
In sum, the curve $C_0$ may be the limit of curves $C_t$ having
up to $\delta(C)$ nodes.
\end{remark}


\begin{lemma}
\label{l:genus}
Let $C$ be a reduced plane tropical curve with Newton polygon $\Delta$ such
that all the tiles of the
subdivision of $\Delta$ are triangles and parallelograms.
Then the two definitions of the geometric genus of a plane tropical curve
in \ref{p:gen-resol}
and \ref{p:sings-gen}
coincide.
\end{lemma}

\noindent
The following folklore proof has been communicated to me by Erwan
Brugallé. 

\begin{proof}
For the sake of simplicity, we shall assume that $C$ is reduced
and irreducible, \ie
it cannot be written as the sum of two non-empty plane tropical curves.
In order to compute the geometric genus of $C$ as in
\ref{p:gen-resol}, we note that abstract tropical plane curves of
minimal genus with a map to $C$ are obtained by separating the
``nodes'' of $C$, \ie by seeing each crossing of two line segments as the
image of two disjoint line segments.
Let $\Gamma$ be such an abstract tropical curve. It has only trivalent
vertices besides the (univalent) vertices at infinity,
in the number $t$ equal to the number of triangles in the
subdivision of $\Delta$.
The finite edges of $\Gamma$ (\ie edges joining two vertices
at finite distance) correspond to the finite segments of $C$,
and their number is the number $a$ of unordered pairs of parallel
edges $\{\sigma,\sigma'\}$ in the subdivision of $\Delta$ such that
$\sigma$ and $\sigma'$ belong to two distinct triangles
$\Delta_v$ and $\Delta_{v'}$ of the
subdivision and are 
linked by a (possibly empty) chain of parallelograms
(the most common situation is that $\sigma=\sigma'$ is the
intersection of two adjacent triangles);
note that an edge of a triangle $\Delta_v$ appears in such a pair if
and only if it does not border $\Delta$, and in that case it appears in a
unique pair. The topological Euler--Poincaré
characteristic of $\Gamma$ is
\begin{equation*}
  \chi_\top(\Gamma) = 1-g = t-a,
\end{equation*}
where $g$ is the genus of $\Gamma$,
hence $g=1-t+a$.
Note how this computation of $\chi_\top(\Gamma)$ uses the irreducibility of
$C$: 
if $C$ contained a line joining two vertices at infinity
(corresponding to two edges in the boundary of $\Delta$ linked by a
chain of parallelograms), then $\Gamma$ would have a connected
component not containing any vertex at finite distance, and the
formula for $\chi_\top(\Gamma)$ would need to be suitably adjusted.

In order to relate this value with the genus of $C$ computed as in
\ref{p:sings-gen}, we shall use Pick's formula
(see \ref{p:deg-Delta} and \ref{sp:p_a});
it says that for all
lattice polygons $D$,
\[
  p_a(D) = \Ar(D)
  -\frac 1 2 \sum\nolimits_{\sigma \text{ edge of } D} \lz(\sigma)
  +1.
\]
Thus, for all vertices $v$ of $C$,
\[
  \delta(v) =
  \begin{cases}
    \Ar(\Delta_v)
    -\frac 1 2 \sum_{\sigma \text{ edge of } \Delta_v} \lz(\sigma)
    +1
    + \frac 1 2 \sum _{
         \substack{\sigma \text{ edge of } \Delta_v\\
           \text{not bordering }\Delta
         }
       }
       \bigl(\lz(\sigma)-1\bigr)
    \quad \text{if } \Delta_v \text{ triangle}
    \\
    \Ar(\Delta_v)
    \qquad \text{if } \Delta_v \text{ parallelogram},
  \end{cases}
\]
and therefore
\begin{align*}
  \delta(C)
  &= \Ar(\Delta)
  -\frac 1 2 \sum_{\substack{
    (\sigma,\Delta_v),\\
    \sigma \text{ edge of } \Delta_v,\\
    \Delta_v \text{ triangle}}} \lz(\sigma)
  + t 
  +\frac 1 2 \sum_{\substack{
    (\sigma,\Delta_v),\\
    \sigma \text{ edge of } \Delta_v,\\
    \Delta_v \text{ triangle},\\
    \sigma \text{ not bordering }\Delta}}
  \lz(\sigma)
  -a
  \\
  &= \Ar(\Delta)
    -\frac 1 2 \sum_{\substack{
    (\sigma,\Delta_v),\\
    \sigma \text{ edge of } \Delta_v,\\
    \Delta_v \text{ triangle},\\
    \sigma \text{ bordering }\Delta}}
  \lz(\sigma)
  +t-a.
\end{align*}
Now we claim that the last sum equals the sum of the lengths
of the edges of $\Delta$.
Indeed, since $C$ is irreducible it cannot contain a line between two
vertices at infinity. Therefore, an edge in the boundary of $\Delta$
cannot be linked by a chain of parallelograms to another edge in the
boundary of $\Delta$, and thus every edge in the boundary of $\Delta$
is linked by a chain of parallelograms to an edge of a triangle of the
subdivision of $\Delta$.

Finally, by Pick's formula again,
$\delta(C) = p_a(\Delta)-1+t-a$,
hence $p_a(\Delta)-\delta(C)=1-t+a$, which coincides with the genus
$g$ computed in the first place.
\end{proof}


\section{The tropical enumerative problem and the 
correspondence theorem}
\label{S:trop-enumpb}

In this section, we first state the tropical enumerative problem and
describe its correspondence with the toric enumerative problem.
Then we give several detailed examples.

\subsection{General theory}

\paragraph{The tropical enumerative problem} 
\label{p:trop-enumpb}
Let $\Delta \subset \R^2$ be a convex integral polygon, and call
$\Sigma_1,\ldots,\Sigma_n$ its edges. We consider the data of an
integer $g$ such that $0 \leq g \leq \Card (\mathring \Delta _\Z)$,
and $\alpha = (\alpha_1,\ldots,\alpha_n),
\beta = (\beta_1,\ldots,\beta_n) \in \Nseq^n$ such that
\begin{equation*}
  \forall s=1,\ldots,n,
  \qquad
  I\alpha_s + I\beta_s = \lz (\Sigma_s),
\end{equation*}
and
\begin{equation*}
I\alpha < \Card (\partial \Delta _\Z).
\end{equation*}
In a nutshell, the problem is to find the number of
plane tropical curves of genus $g$ and Newton polygon $\Delta$ that
(i) have assigned and unassigned infinite edges as prescribed by
$\alpha$ and $\beta$, respectively,
and (ii) pass through the appropriate number of fixed general points
of $\R^2$.

To set this up precisely, fix a set
$\ux=\{x_1,\ldots,x_{g-1+|\beta|} \}$ of $g-1+|\beta|$ general points
of $\R^2$, and a set
$\Omega = (\{ p_{s,i,j} \} _{1\leq j \leq \alpha_{s,i}} )
_{1\leq s \leq n, 1 \leq i}$
of $\alpha$ general real numbers.
Let $u_1,\ldots,u_n \in \R^2$ be the unitary vectors such that $u_1
^\perp, \ldots, u_n ^\perp$ give the oriented directions of
$\Sigma_1,\ldots,\Sigma_n$, respectively
($\Sigma_1,\ldots,\Sigma_n$ are ordered, up to cyclic permutation, and
oriented according to the orientation of the $\R^2$ in which $\Delta$
dwells). 
For all $s=1,\ldots,n$ and $p \in \R$, we
let $\sL_{u_s,p}$ be the line in $\R^2$ that is directed by the vector
$u_s$ and contains the point with coordinates $p\cdot u_s ^\perp$.
\par We then define $\cE ^\Delta_g (\alpha,\beta) (\ux, \Omega)$ as the
set of tropical maps $f$ from an abstract tropical curve $C$ of
arithmetic genus $g$ to the tropical plane, 
such that the Newton polygon of $f$ equals $\Delta$, and in addition:
(i) for all $1 \leq s \leq n$ and $i \geq 1$, the plane tropical curve
$f(C)$ has $\alpha_{s,i} + \beta_{s,i}$ infinite edges $E$ of weight
$\geq i$
such that $u_{E,\infty} = u_s$, with $\alpha_{s,i}$ of them supported
on the lines $\sL _{u_s, p_{s,i,1}}, \ldots, \sL _{u_s,
  p_{s,i,\alpha_{s,i}}}$, respectively,
and (ii) $f(C)$ contains all the points $x_1,\ldots,x_{g-1+|\beta|}$.
The problem is to find the cardinality of the set 
$\cE ^\Delta_g (\alpha,\beta) (\ux, \Omega)$,
counting its elements with appropriate multiplicities;
it is expected to be
finite, \cf Proposition~\ref{pr:trop-AVZ}.



\begin{example}
\label{ex:conics-trop}
Consider the same Newton polygon $\Delta$ as in \ref{ex:P2}, (b),
with the edges labelled as in the picture below.
\begin{center}
\includegraphics[height=1.5cm]{ex-conics-trop-N.eps}
\hspace{2cm}
\includegraphics[height=2cm]{ex-conics-trop-st.eps}
\end{center}
Next to the diagram is depicted a typical plane tropical
curve with Newton polygon $\Delta$; it has arithmetic genus $0$.
\par
We consider the data $g=0$, $\alpha=( 0,0,1 )$,
$\beta = (1, [0,1], 0)$,
$\ux =\{x_1\}$, and $\Omega = \{ p_{3,1,1} \}$: this means that no condition is imposed on
the infinite edge with direction $u_1$, and we require that
(i) one edge with
direction $u_2$ have weight $\geq 2$, with unassigned support,
and (ii) one edge with direction $u_3$ be supported on the line 
$\sL_{u_3,p_{3,1,1}}$ determined by the real number $p_{3,1,1}$; we
require in addition that the curve contain the general point $x_1$.
\par
One checks that there is a unique such tropical map, as indicated on
the picture below (the fixed line $\sL_{u_3,p_{3,1,1}}$ is represented
as a dotted line).
\begin{center}
\includegraphics[height=2.5cm]{ex-conics-trop-data.eps}
\hspace{1cm}
\raisebox{1cm}{$\leadsto$}
\hspace{1cm}
\includegraphics[height=2.5cm]{ex-conics-trop-ex.eps}
\end{center}
\end{example}


\begin{remark}
\label{rk:trop-P2}
The condition on infinite edges being supported by the assigned lines
$\sL$ may be formulated in terms of the passing through assigned
points at infinity, for a suitable notion of points at infinity.
The latter are the points one needs to add to $\R^2$ in order to
obtain the tropical toric surface associated to $\Delta$, see
\cite[Section 7.3]{BIMS}.

For instance the tropical projective plane, \ie the tropical toric
surface associated to a triangle $T_d$ as in Example \ref{ex:P2},
looks like the triangle $T_d$ itself, with the interior corresponding to
$\R^2$ and the edges to the points at infinity; each edge may be
identified with $\R\cup \{\pm \infty \}$.
It
is the quotient of
$(\R\cup\{-\infty\})^3 \setminus
\bigl\{(-\infty,-\infty,-\infty)\bigr\}$
%minus the point $(-\infty,-\infty,-\infty)$
by the equivalence relation $\sim$ defined by
\[
  (x_0,x_1,x_2) \sim (x'_0,x'_1,x'_2)
  \et[$\iff$]
  \exists \lambda \in \R:\
  (x'_0,x'_1,x'_2) = (x_0+\lambda,x_1+\lambda,x_2+\lambda).
\]
If $x_0 \neq -\infty$, then $(x_0,x_1,x_2)$ is equivalent to a unique
point of the form $(0,x,y)$ with $(x,y) \in (\R\cup\{-\infty\})^2$,
namely $(0,x_1-x_0,x_2-x_0)$;
if $(x_0,x_1,x_2)\in \{-\infty\}\times \R^2$,
then $(x_0,x_1,x_2)$ is equivalent to a unique
point of the form $(-\infty, x, -x)$ with $x\in \R$,
namely $(-\infty, \frac {x_1-x_2} 2, \frac {x_2-x_1} 2)$.
\end{remark}


The following result states that for a general choice of $\Omega$ and
$\ux$, 
the set $\cE ^\Delta_g (\alpha,\beta) (\ux, \Omega)$
is indeed finite, and its
members have the simplest possible shape.
This is thus a tropical analogue of the
main theorem in \cite{03.th-acz}.
It is mainly due to Mikhalkin \cite{mikhalkin-JAMS}; the article
\cite{mikhalkin-JAMS} does not comprise the possibility of boundary
conditions (those encoded by $\alpha$ and $\beta$), even if it
contains all the necessary ingredients to handle them. Boundary
conditions in this context have first appeared in
\cite{gathmann-markwig}.

\begin{proposition}
\label{pr:trop-AVZ}
Let\/ $\Delta,g,\alpha,\beta$ be as in \ref{p:trop-enumpb}.
For a general choice of\/ $\ux, \Omega$, the set\/
$\cE ^\Delta_g (\alpha,\beta) (\ux, \Omega)$ is finite.
Moreover, for every 
$(C,f) \in \cE ^\Delta_g (\alpha,\beta) (\ux, \Omega)$,
the following hold:
\begin{mycpctenum}[(i)]
\item
\label{it:trivalent}
the graph $\Gamma=\bar \Gamma \setminus \Gamma^\infty$ underlying
$C=(\bar\Gamma, g)$ is trivalent; 
\item
\label{it:top-imm}
the map $f$ is a topological immersion;
\item
\label{it:only-nodes}
the preimage of any point $x \in \R^2$ has at most two elements; 
\item
\label{it:min-weight}
the infinite edges of $f(C)$ have minimal weight;\footnote
{\ie for all
$s=1,\ldots,n$ and $i \geq 1$, the plane tropical curve $f(C)$ has
exactly $\alpha_{s,i}+\beta_{s,i}$ infinite edges 
of weight precisely $i$ in the oriented direction $u_i$.}
\item
the set of vertices of the plane curve $f(C)$ is disjoint from the set
$\ux$; 
\item 
an edge of the plane curve $f(C)$ contains at most one point from the
set $\ux$.
\end{mycpctenum}
\end{proposition}


Condition~\eqref{it:top-imm} asserts in particular that no
neighbourhood of a trivalent vertex of $\Gamma$ is ever mapped to a
segment.
Conditions \eqref{it:trivalent} and \eqref{it:only-nodes} together
imply that the tiles of the subdivision of the Newton polygon of
$f(C)$ are all triangles and parallelograms.


One should beware that Proposition~\ref{pr:trop-AVZ} does not say that
the shapes of the plane tropical curves corresponding to tropical maps
in the 
set $\cE ^\Delta_g (\alpha,\beta) (\ux, \Omega)$ are independent of the
choice of $\ux$ and $\Omega$, and this is indeed not true in
general. For instance, their respective subdivisions of $\Delta$ 
may vary as $\ux$ moves, \cf Example~\ref{ex:cubic-etagees}
and Figure~\ref{ex:cubic-etagees-a}.


\begin{remark}
It most often happens that some members of
$\cE ^\Delta_g (\alpha,\beta) (\ux, \Omega)$
have their corresponding plane tropical curve that has finite edges of
weight larger than one
(see Example \ref{ex:cubic-etagees} for instance).
This is analogous (see Remark \ref{rk:sings-trop-v-alg})
to the fact that when considering degenerations of
(classical) nodal algebraic curves, one
more or less inevitably
ends up with some tacnodal
curves, which is one of the central themes of this
whole volume.
\end{remark}


In order to correspond to the counting of algebraic curves, the
counting of tropical curves must be made with 
appropriate multiplicities.
Besides, the mere cardinality (\ie without multiplicities) of
$\cE ^\Delta_g (\alpha,\beta) (\ux, \Omega)$ does in general depend on
the choice of $\ux$ and $\Omega$.

\paragraph{Tropical multiplicity}
\label{p:trop-mult}
Let $f$ be a tropical morphism from an abstract tropical curve $C=(\bar
\Gamma, g)$ to the tropical plane. Assume that
every vertex $v \in \Gamma$ (\ie every vertex at finite distance)
is trivalent.
\par For each such vertex $v$, we define
its multiplicity to be twice the Euclidean area of the triangle
$\Delta_v$ dual to $v$ in the subdivision of the Newton polygon of
$f$, \ie
\begin{equation}
\label{eq:mult-vertex}
\mu^\C(v)  \overset{\text{def.}}= 2 \Ar(\Delta_v)
= \bigl| \det \bigl(
w(\Sigma)\cdot u_{v,\Sigma},\, w(\Sigma')\cdot u_{v,\Sigma'}
\bigr) \bigr|,
\end{equation}
where in the last equality $\Sigma, \Sigma'$ are any two edges ending
at $v$ (out of three, since $v$ is assumed to be trivalent;
the balancing condition implies that the multipicity is independent of
the choice of those two edges).

\par The \emph{complex tropical multiplicity} of the map $(C,f)$ is
\begin{equation*}
\mu^\C (C,f) \overset{\text{def.}}= \prod _{v \in \Gamma} \mu^\C(v).
\end{equation*}
The enumeration of plane tropical curves may also be related with the
enumeration of real algebraic plane curves, albeit with a different
multiplicity: this is why we keep an index $\C$ in the notation.

\begin{example}
The plane tropical curve in Example \ref{ex:abstract}, seen as the
image of a tropical map from the genus zero curve (b), has
multiplicity one. Note that the vertex \#6 of the plane curve has two
points in its preimage, and does not correspond to a vertex of the
abstract curve.

The plane tropical curve in Figure \ref{fig:trop-3ique-w2}, seen as
the image of a tropical map from a genus zero curve, has multiplicity
four. Indeed, the two triangles marked with a star in the
decomposition of the Newton polygon correspond to vertices $v$ of the
abstract curve such that $\mu^\C(v) = 2$.
See \cite[\tref{p:lim-nodes}]{07.th-diag-degen}
for a discussion (in the context of floor diagrams)
of this multiplicity four
in relation with the multiplicity of components of limit Severi
varieties. 
\end{example}


The following result,
known as Mikhalkin's Correspondence Theorem,
states the correspondence between the algebraic and tropical
enumerative problems stated in \ref{p:enumpb} and \ref{p:trop-enumpb}
respectively.
It is mainly due to Mikhalkin \cite{mikhalkin-JAMS}; as for
Proposition \ref{pr:trop-AVZ}, the original result does not mention
boundary conditions, which have first appeared in
\cite{gathmann-markwig}. 


\begin{theorem}
\label{t:M-corresp}
Let $\Delta,g,\alpha,\beta$ be as in \ref{p:trop-enumpb}, and choose
$\ux, \Omega$ general enough.
The following equality holds:
\begin{equation*}
\sum _{(C,f) \in \cE ^\Delta_g (\alpha,\beta) (\ux, \Omega)} \mu^\C
(C,f)
= I^\alpha \cdot
N^\Delta_g (\alpha,\beta).
\end{equation*}
\end{theorem}

The starting point of the proof is the idea presented in
Section~\ref{S:tor-to-trop} that tropical
hypersurfaces are limits of toric hypersurfaces.


\subsection{Examples}

\paragraph{}
\sloppy
In the situation of Example~\ref{ex:conics-trop} above,
there is exactly one element $(C,f)$ in $\cE ^\Delta_g (\alpha,\beta) (\ux,
\Omega)$. The corresponding decomposition of $\Delta$ is the
trivial one, consisting only of the triangle $\Delta$ itself, which
has Euclidean area $\Ar (\Delta)=1$; one therefore has
$\mu^\C (C,f) = 2$.

As the Correspondence Theorem tells us, this gives
$N^\Delta_g (\alpha,\beta) = 2$, which indeed is the number of conics
tangent to the line $z=0$ at $(0:1:0)$, with prescribed general second
order osculatory behaviour at this point, tangent to the line $y=0$ at
an unprescribed point, and passing through a general point $x_1$.
\par
This is pictured below: two successive blow-ups of $\P^2$ are
drawn, with exceptional divisors $E$ and $E'$; base points are
represented by black dots or arrows when they are infinitely near, and
the unassigned tangency condition is represented by an arrow with a dash.
\begin{center}
\includegraphics[width=\textwidth-1cm]{ex-conics-trop-P2.eps}
\end{center}

\paragraph{}
\label{sp:E4-trop0}
Let us return to the enumerative problem \ref{sp:E4}: we let $\Delta$
be the Newton polygon indicated below, and fix
$\alpha=(1,1,1,0)$, $\beta=(0,0,0,1)$. The set $\Omega$ consists of
three real values, fixing three lines $\sL_1, \sL_2, \sL_3$ as
indicated on the picture below.
\begin{center}
\includegraphics[height=1.5cm]{ex-E4.0-N.eps}
\quad \raisebox{.8cm}{;}\qquad
\includegraphics[height=2.5cm]{ex-E4.0-data.eps}
\end{center}
The tropical curves defined by this data move in a $1$-dimensional
family, in the way pictured below (two curves are pictured, one in
green and one in blue): the deformations of the curves amount to
change the size of the central rectangle by sliding one of its corners
along a line $\sL_i$, which lets all the rest follow.
As the curves move in this family, one notices that the semi-line
corresponding to the edge $\Sigma_4$ of the Newton polygon is always
supported on the same line, which we shall call $\tilde{\sL}_4$:
this is the tropical incarnation of the
toric Cayley--Bacharach property stated in Lemma~\ref{l:torCB}.
\begin{center}
\includegraphics[height=2.5cm]{ex-E4.0-pencil.eps}
\hspace{15mm}
\includegraphics[height=2.5cm]{ex-E4.0-CB.eps}
\captionof{figure}{A pencil of tropical curves and the
  Cayley--Bacharach property}
\label{fig:tropical-CB}
\end{center}
We want to count curves of genus $g=0$ in this system.
There is a finite number of such curves, thus the set $\ux$ of base
points is empty. There is a
unique rational curve, depicted below together with the corresponding
triangulation of the Newton polygon
(note that a different choice for the lines $\sL_1, \sL_2, \sL_3$ may
lead to another, similar, triangulation).
\begin{center}
\includegraphics[align=c,height=2.5cm]{ex-E4.0-ratcurve.eps}
\hspace{20mm}
\includegraphics[align=c,height=1cm]{ex-E4.0-Nrat.eps}
\end{center}
Both triangles in this triangulation yield the same multiplicity,
\begin{equation*}
\mu(\Delta_v) = \left| \det
\begin{pmatrix}
1 & 1 \\
1 & -1
\end{pmatrix}
\right|
= 2.
\end{equation*}
One thus finds
$N^\Delta _0\bigl( (1,1,1,0),(0,0,0,1) \bigr) =4$,
in tune with the number previously found in \ref{sp:E4}.

\paragraph{}
\label{sp:3A2-trop}
We now consider the enumerative problem \ref{sp:3A2}: we let $\Delta$
be the Newton polygon indicated below, and set $g=0$,
$\alpha=(1,1,0)$, $\beta=(0,0,1)$. The set $\Omega$ consists of two
real values, fixing two lines $\sL_1, \sL_2$ as indicated on the
picture below, and the set $\ux$ of general base points is empty.
\begin{center}
\includegraphics[height=1.5cm]{ex-3A2-N.eps}
\quad \raisebox{.8cm}{;}\qquad
\includegraphics[height=2cm]{ex-3A2-data.eps}
\hspace{1cm}
\raisebox{.8cm}{$\leadsto$}
\hspace{1cm}
\includegraphics[height=2cm]{ex-3A2-curve.eps}
\end{center}
This enumerative problem is very similar to \ref{sp:E4} and may be
solved exactly as in \ref{sp:E4-trop0} above.
There is only one tropical map in $\cE^\Delta _0\bigl(
(1,1,0),(0,0,1) \bigr)$; the corresponding subdivision of $\Delta$ is
the trivial one, with only one triangle $\Delta_v$ giving the
multiplicity
\begin{equation*}
\mu(\Delta_v) = \left| \det
\begin{pmatrix}
2 & 1 \\
-1 & -2
\end{pmatrix}
\right|
= 3.
\end{equation*}
One thus finds
$N^\Delta _0\bigl( (1,1,0),(0,0,1) \bigr) =3$,
in tune with the number previously found in \ref{sp:3A2}.

\paragraph{}
\label{sp:E4-trop}
Let us consider one last enumerative problem, which is linked with
\ref{sp:E4}.
The problem is to 
 enumerate genus $0$ curves of type
$(2,2)$ on $\P^1 \times \P^1$ tangent to all four points cut out on an
anticanonical quadrilateral by a general curve of type $(1,1)$.  As
this imposes only seven independent linear conditions, this amounts to
requiring the tangency at three fixed points and one mobile point.
\par Correspondingly, we consider the Newton polygon $\Delta$
indicated below, and set $g=0$,
$\alpha=(2,2,2,0)$ and $\beta=(0,0,0,2)$.
 The set $\Omega$ determines three lines $\sL_1,\sL_2,\sL_3$, and
the set $\ux$ is empty.
\begin{center}
\includegraphics[height=1.5cm]{ex-E4-N.eps}
\quad \raisebox{.8cm}{;}\qquad
\includegraphics[height=2cm]{ex-E4-data.eps}
\hspace{1cm}
\raisebox{.8cm}{$\leadsto$}
\hspace{1cm}
\includegraphics[height=2cm]{ex-E4-curve.eps}
\end{center}
There is only one tropical map $(C,f)$ in $\cE^\Delta _0 (\alpha, \beta)$;
note that its shape depends on the relative vertical position of the
two parallel lines $\sL_1$ and $\sL_3$. In any event, there are five
edges of weight $2$, and the subdivision of $\Delta$ consists of two
triangles, each with Euclidean area $2$.
The Correspondence Theorem thus gives
\begin{equation*}
N^\Delta_0 (\alpha,\beta) = \frac 1 {I^\alpha} \times \mu^\C(C,f)
= \frac {4 \times 4} {2^3} = 2.
\end{equation*}

The relation with \ref{sp:E4} comes from 
seeing the quartic Del Pezzo surface with four ordinary double points
of \ref{sp:E4} as a double
cover of $\P^1 \times \P^1$ branched over an anticanonical
quadrilateral.
The number $2$ found above fits with the number $4$ given in
\ref{sp:E4} and \ref{sp:E4-trop0}, the factor $2$
between $4$ and $2$ being accounted for by the double cover.


\bigskip
For one more example, slightly more involved than the above ones, you
can consult Example \ref{sp:tropWij}, in which the enumerative problem
of \ref{sp:W_ij} is considered.



\section{Floor diagrams and enumeration}
\label{S:floors}


This section is dedicated to the translation of the tropical
enumerative problem \ref{p:trop-enumpb}
in purely combinatorial terms, under certain technical assumptions.
We first define floors and elevators of a plane tropical curve, which
will enable its encoding as a floor diagram.
Next we give an abstract definition of floor diagrams, and discuss
the relevant technical conditions. When this is done we state Brugallé
and Mikhalkin's Correspondence Theorem. Many examples are discussed
throughout. 
% The following definition indicates what we will consider a
% ``component'' of a plane tropical curve, with respect to a preferred
% direction $\sd$.
We use the notation of Section~\ref{s:param-trop-curve}.


The floor diagrams that I define here are a mixture
of those defined in \cite{BM-11} and \cite{arroyoetal-11}, with a
presentation according to my personal taste.
As Brugallé taught me, floor diagrams are more a philosophy than a
specific object.
Besides, the floor diagrams considered in
\cite{fomin-mikhalkin} are themselves slightly different from those in
\cite{BM-11}, see \cite[Remark 1.2]{fomin-mikhalkin}.
Note that the floor
diagrams introduced in \cite{07.th-diag-degen} are a
particular instance of those presented here, corresponding to the
Newton polygons of complete linear systems of plane curves
(\ie the triangles $T_d$ of Example \ref{ex:P2}).


\begin{definition}
\label{d:floors-n-elevators}
Let\/ $\sd = (a,b) \in \Z^2$ be a primitive vector, and let
$(C,f)$ be a parametrized plane tropical curve,
\ie $C = (\bar \Gamma, g)$ 
is an abstract tropical curve with a tropical map $f$ to the
plane.
An\/ \emph{elevator} of\/ $(C,f)$ is an edge $\Sigma$ of\/ $C$ with
oriented direction vector in the plane $u_\Sigma = \pm \sd$ (see Definition
\ref{d:param-trop-curve}).
A\/ \emph{floor} of\/ $(C,f)$ is a connected component of\/
$\Gamma \setminus \operatorname{Elev}$,
where\/ $\Gamma= \bar \Gamma \setminus \Gamma^\infty$
as in Definition \ref{d:abs-trop-curve}, and\/
$\operatorname{Elev}$ is the union of all elevators of\/ $(C,f)$.
\end{definition}

\begin{example}
Below, I explicit the respective decompositions of a genus $1$ and a
genus $0$ plane tropical cubics into floors and elevators, assuming
$\sd$ is the vertical direction.
% (in favourable circumstances, see Remark~\ref{rk:messed-floors}
% below).
On the left, I picture the plane
tropical curve;
in the middle, I separate the floors and elevators
(the former are chains of line segments with no vertical components,
the latter are vertical segments or semi-lines);
on the right, I provide a schematic picture of the incidence between
floors and diagrams, on which the floors are
represented by ellipses and the elevators by vertical segments.

On Figure~\ref{fig:floors-rat3ic}, note that we see the curve as a
parametrized rational curve, so that the two segments intersecting at
the black square are separate in the source curve, as in Example
\ref{ex:abstract}, case (b). The floors and elevators are defined at
the level of the source curve.

\begin{center}
\includegraphics[align=c, scale=.8]{floors-sm3ic-curve.eps}
\hspace{1cm}
\includegraphics[align=c, scale=.8]{floors-sm3ic-comps.eps}
\hspace{1cm}
\includegraphics[align=c, scale=.8]{floors-sm3ic-diag.eps}
\captionof{figure}{Floor decomposition of a genus $1$ tropical cubic}
\end{center}
\begin{center}
\includegraphics[align=c, scale=.8]{floors-rat3ic-curve.eps}
\hspace{1cm}
\includegraphics[align=c, scale=.8]{floors-rat3ic-comps.eps}
\hspace{1cm}
\includegraphics[align=c, scale=.8]{floors-rat3ic-diag.eps}
\captionof{figure}{Floor decomposition of a genus $0$ tropical cubic}
\label{fig:floors-rat3ic}
\end{center}
\end{example}


\begin{remark}
\label{rk:messed-floors}
In general it is not true that floors are chains of line
segments, or that an elevator intersects a given floor only once, see
the examples in Figure \ref{fig:messed-floors}.
This will however be the case when we impose the passing through base
points $\ux$ sufficiently stretched out along direction $\sd$.
\begin{figure}[htbp]
\centering
\includegraphics[align=c]{messed-cubic-i.eps}
\hspace{2cm}
\includegraphics[align=c]{messed-cubic-ii.eps}
\caption{Tropical curves with messed up floor
  decomposition (see
  Remark \ref{rk:messed-floors})}
\label{fig:messed-floors}
\end{figure}

It is also possible that the planar incarnations of two floors
intersect, even under our general favourable framework when the points
$\ux$ are sufficiently stretched out along direction $\sd$.
See \ref{sp:unordered} for an example.
\end{remark}


The feature that will enable the translation of a tropical enumerative
problem into an enumeration of floor diagrams is the following:
if the the base
points $\ux$ are sufficiently streched in the direction $\sd$, then for
all curve $(C,f) \in \cE_g^{\Delta}(\alpha,\beta)(\ux, \Omega)$,
each elevator (resp.\ floor) of $(C,f)$ will pass through exactly one
point $x_i$ of $\ux$.
In particular, we will see that
the cardinality of $\ux$ equals the number of
elevators and floors in $(C,f)$.



\bigskip
There are two technical conditions for the translation into an
enumeration of floor diagrams to work correctly.  The first one is
that the Newton polygon $\Delta$ should be ``transverse to the
direction $\trsp \sd$'', and the second one is that non-trivial
boundary conditions (\ie conditions of types $\alpha$ and $\beta$) may
only be imposed corresponding to specific components of the boundary
of $\Delta$, orthogonal to the direction $\sd$.


\begin{definition}
Set\/ $\sd = (a,b) \in \Z^2$ with\/ $\gcd(a,b)=1$.
% and choose $u,v\in \Z$ so that
% $au+bv=1$.
Let\/ $\Delta$ be a
Newton polygon.
The \emph{left and right boundaries} of\/ $\Delta$ with respect to\/ $\sd$
are, respectively,
\[
  \partial_l\Delta = \left\{
    p \in \Delta:\
    \forall t >0, \ p+t. \orth \sd \not\in \Delta
  \right\}
  \quad \text{and}
  \quad
  \partial_r\Delta = \left\{
    p \in \Delta:\
    \forall t >0, \ p-t. \orth \sd \not\in \Delta
  \right\}.
\]
The Newton polygon\/ $\Delta$ is\/ \emph{$\orth \sd$-transverse} if
for all vector\/ $u \in \Z^2$, parallel to an edge of
$\partial_l\Delta$ or\/ $\partial_r\Delta$ and with relatively prime
coordinates, one has\/ $\det(u, \orth \sd) =\pm 1$.
\end{definition}

\bigskip
The original definition
\cite[2.2]{BM-11} corresponds to $\sd = (0,1)$, and is called
$h$-transversality there, `$h$' standing for `horizontal'.

The geometric meaning of $\orth \sd$-transversality is that for all
tropical curves $\Gamma$ with Newton diagram $\Delta$, any
(weight one) line
in $\R^2$ directed by $\sd$ should intersect each infinite branch $e$
of $\Gamma$ with
multiplicity equal to the weight $w(e)$
(except if the branch has the same direction $\sd$).
This implies that the total number of intersection of such a line with
$\Gamma$ is the number of floors of $\Gamma$.
The definition of intersection multiplicity to make this work is the
following: two lines directed by primitive vectors $u_1,u_2 \in \Z^2$
and with weights $w_1$ and $w_2$
intersect with multiplicity 
$w_1\cdot w_2\cdot\det(u_1,u_2)$.


\begin{examples}
\label{ex:h-tr}
The triangle $T_d$, corresponding to the complete linear system $|dH|$
on $\P^2$ (see \ref{ex:P2}),
is $\orth \sd$-transverse for $\sd = (0,1)$.

The trapezium 
$\Tz^r_{a,b}$,
corresponding to the complete linear system
$|aH+bF|$ on the Hirzebruch surface $\F_r$
(see \ref{sp:trapezium}),
is $\orth \sd$-transverse for $\sd = (0,1)$,
but if $r>1$ it is not for $\sd = (1,0)$.

The two polygons given in \ref{sp:W_ij} and \ref{sp:E4}
are $\orth \sd$-transverse for $\sd = (0,1)$,
but neither for $\sd = (1,1)$, nor for $\sd =(1,-1)$.

The triangle in \ref{sp:3A2} is not $\orth \sd$-transverse either for
$\sd=(0,1)$, or $(1,0)$, or $(1,1)$, or $(1,-1)$.
\end{examples}


\paragraph{}
\label{p:boundary-dir-d}
The second condition to be fulfilled by a tropical enumerative problem
in order to be translatable into a floor diagram problem is that one
should impose non-trivial boundary conditions only along those edges
of $\Delta$ that are orthogonal to $\sd$, or equivalently along the
one or two edges from $\partial \Delta$ off
$\partial_l \Delta \cup \partial_r \Delta$.

In other words, in the notation of \ref{p:trop-enumpb}, for all $s
=1, \ldots, n$, if $\Sigma_s$ lies on the left or right boundary of
$\Delta$ with respect to $\sd$, then $\alpha_s = 0$ and
$\beta _s = [\lz (\Sigma_s) ]$.

\bigskip
\noindent
We need the following before we can define floor diagrams.

\paragraph{}
\label{p:polygon:directions}
Let $\Delta$ be a $\orth \sd$-transverse Newton polygon, for some
primitive vector $\sd \in \Z^2$.
Let $\Sigma$ be an edge of $\Delta$ lying on its left or right
boundary, 
and view it as a vector going down with respect to the direction
$\sd$:
this vector writes $\lz(\Sigma).u$, with $u$ a primitive integer
vector 
such that $\det(\orth \sd, u)=+1$. The list of directions
associated to $\Sigma$ is the unordered list
$[\orth u,\ldots,\orth u]$ consisting of the primitive vector $\orth
u$ repeated $\lz(\Sigma)$ times.
The \emph{list of left (resp.\ right) directions} of $\Delta$ is the
unordered list 
$D_l(\Delta)$ (resp.\ $D_r(\Delta)$) obtained by concatenating the
lists of directions 
of all edges $\Sigma$ lying on the left (resp.\ right) boundary of
$\Delta$.

Note that, for tropical curves $(C,f)$ with Newton polygon
$\Delta$,
the list of left directions of $\Delta$ correspond to the
direction vectors $u_{\infty,\Sigma}$ pointing from infinity inwards
of infinite branches of coming from the left with respect to the
direction $\sd$, 
whereas the right directions correspond to vectors $u_{\Sigma,\infty}$
pointing outwards to infinity for infinite branches going to the
right. In other words, the direction is always from left to right with
respect to the direction $\sd$.

Lastly, let $d_+(\Delta)$ (resp.\ $d_-(\Delta)$) be the integral
length of the top (resp.\ bottom) edge of $\Delta$, parallel to the
direction $\orth \sd$. If there is no such edge, we set the
corresponding value $d_\pm (\Delta)$ to $0$.

The $\orth \sd$-transversality condition ensures that
$D_l(\Delta)$ and $D_r(\Delta)$ have the same number of
elements\footnote
{by a suitable change of coordinates in $\SL_2(\Z)$ we may reduce to
  the case $\sd=(0,1)$, and then the transversality condition is that
  any primitive vector $u \in\Z^2$ parallel to an edge on the left or
  right boundary of $\Delta$ is of the form $(\alpha,\pm 1)$, $\alpha
  \in \Z$.},
which we shall call the $\sd$-height of the polygon $\Delta$, and
denote by $d_\sd(\Delta)$.
Thus
\begin{align*}
  d_\sd(\Delta)
  &= \operatorname{length}(D_l(\Delta))
    =   \Card(\partial_l(\Delta) \cap \Z^2) -1
  \\
  &= \operatorname{length}(D_r(\Delta)) 
  = \Card(\partial_r(\Delta) \cap \Z^2)-1.
\end{align*}
Moreover the following holds,
\begin{equation}
\label{eq:polygon:directions}
  2d_\sd(\Delta) + d_+(\Delta) + d_-(\Delta)
  = \Card(\partial\Delta _{\Z}).
\end{equation}



\begin{examples}
\label{ex:h-tr2}
The following are the examples from \ref{ex:h-tr} continued.
We take $\sd = (0,1)$ in all cases.
\setlength{\parindent}{0cm}

For the triangle $T_d$, one has
$d_\sd = d_-=d$, $d_+=0$, and
\[
  D_l = \bigl[
  (1,0),\ldots,(1,0)
  \bigr]
  \quad \text{and}
  \quad
  D_r = \bigl[
  (1,1),\ldots,(1,1)
  \bigr].
\]

For the trapezium 
$\Tz^r_{a,b}$,
one has
$d_\sd = a$,
$d_- = b+ar$,
$d_+=b$,
and
\[
  D_l = \bigl[
  (1,0),\ldots,(1,0)
  \bigr]
  \quad \text{and}
  \quad
  D_r = \bigl[
  (1,r),\ldots,(1,r)
  \bigr].
\]

For the polygon in \ref{sp:E4}, one has
$d_\sd = 2$, $d_-=d_+=0$, and
\[
  D_l = D_r = \bigl[
  (1,-1),(1,1)
  \bigr].
\]

For the polygon in \ref{sp:W_ij}, one has
$d_\sd = 3$, $d_-=d_+=0$, and
\[
  D_l = D_r = \bigl[
  (1,-1),(1,1),(1,1)
  \bigr].
\]
\end{examples}


\noindent
Let us now give an abstract definition of floor diagrams.


\paragraph{Weighted oriented graphs}
%\label{p:graphs}
Consider a connected, acyclic, oriented graph $\diag$, with finitely
many vertices and edges. We let $\vt (\diag)$ and $\edg (\diag)$ be the
sets of vertices and edges of $\diag$ respectively (or simply $\vt$
and $\edg$ if no confusion is likely), and see $\edg$ as a subset of
$\vt \times \vt$.
We call $\diag_{\rm top}$ the topological incarnation of $\diag$ as a
$1$-dimensional CW-complex.

\par We assume that there is a distinguished subset of $1$-valent
vertices of $\diag$, which we call the \emph{vertices at
  infinity}.
We let
$\vt ^{-\infty}$ (resp.\ $\vt ^{+\infty}$) be the set of vertices
at infinity whose unique adjacent edge is outgoing (resp.\ ingoing).
We let $\vt^{\rm fin}$ be the complement in $\vt$ of
$\vt ^{-\infty} \coprod \vt ^{+\infty}$, and call those vertices in
$\vt^{\rm fin}$ \emph{floors}.

We assume that there is no edge joining two vertices at infinity. Thus
we have a partition
$\edg = \edg^{-\infty} \coprod \edg^{\rm fin} \coprod \edg^{+\infty}$,
where $\edg^{\pm\infty}$ is the set of those edges adjacent to a
vertex in $\vt^{\pm \infty}$. Thus
$\edg^{\rm fin}$ is the set of those edges joining two floors.
The edges in $\edg^{-\infty} \coprod
\edg^{+\infty}$ are called \emph{infinite}, and the others
\emph{finite}.
In the terminology of Definition \ref{d:floors-n-elevators}, one calls
the edges of $\diag$ (either finite or infinite)
\emph{elevators}.

% In our setup for graphs an edge always connects two vertices, and the
% definition of vertices at infinity is thus arbitrary. This may be
% rendered more natural by considering metric graphs instead; another
% possibility is to allow the possibility of non-compact edges adjacent
% to only one vertex. I do not wish to enter into this territory.

\par We let $\orient$ be the abstract set $\vt ^{\rm fin} \coprod
\edg$, consisting of floors and all edges (finite or infinite) of
$\diag$. Since $\diag$ is acylic, the set $\orient$ inherits a partial
ordering from the orientation.

\par We will in addition assume that $\diag$ is weighted, which means
that it 
comes equipped with a
\emph{weight function} $w: \edg \to \N^*$. 
One then defines the
\emph{divergence} $\div (v)$ of a vertex $v$ (either
a vertex at infinity or a floor) as
\begin{equation*}
\textstyle
\div (v) = \sum _{(s,v) \in \edg} w(s,v) - \sum _{(v,t) \in \edg} w(v,t)
\end{equation*}
(``sum of weights of incoming edges minus sum of weights of outgoing
edges'').


\begin{definition}
Let $\Delta$ be a $\orth\sd$-transverse lattice polygon, and $g$ be a
non-negative integer.
A (plane)\/ \emph{floor diagram} $(\diag,\theta)$ of genus $g$ and
Newton polygon 
$\Delta$ with respect to direction $\sd$
is the data of an acyclic connected weighted oriented graph
$\diag$ and a map $\theta: \vt(\diag)^{\rm fin} \to \Z$, such that the
following conditions hold:
\begin{mycpctenum}[(i)]
\item the first Betti number $b_1(\diag_{\rm top})$ equals $g$;
\item\label{fldiag:inf-edges} one has
$\sum _{v \in \vt ^{-\infty} (\diag)} \div(v) = -d_-(\Delta)$
and
$\sum _{v \in \vt ^{+\infty} (\diag)} \div(v) = d_+(\Delta)$;
\item\label{fldiag:left} the unordered list 
$\bigl[ \theta(v), v\in \vt(\diag)^{\rm fin} \bigr]$
equals $D_l(\Delta)$;
\item\label{fldiag:balance} the unordered list 
$\bigl[ \theta(v)+\div(v).\sd, v\in \vt(\diag)^{\rm fin} \bigr]$
equals $D_r(\Delta)$.
\end{mycpctenum}
\end{definition}


To understand condition
\eqref{fldiag:balance}, note that it follows from the
balancing condition for plane tropical curves that if a floor
of some tropical curve has
direction at infinity from the left $u$, and is intersected from below
by $k$ edges (counted with weights) with direction $\sd$ and from
above by $l$ edges (counted with weights) with 
direction $\sd$, then its direction at infinity to the right is
$u+(k-l).\sd$.
For conditions \eqref{fldiag:left} and \eqref{fldiag:balance} to be
compatible, one needs that $D_l(\Delta)$ and $D_r(\Delta)$ have the
same length, which is granted by the $\orth \sd$-transversality
condition, see \ref{p:polygon:directions};
then $d_\sd (\Delta)$ is the number of floors of a floor diagram with
Newton polygon $\Delta$.

In condition \eqref{fldiag:inf-edges},
$\pm \sum _{v \in \vt ^{\pm\infty} (\diag)} \div(v)$ is the number of
edges in $\edg^{\pm \infty}$, counted with weights;
we may also refer to it as the number of
vertices in $\vt^{\pm \infty}$ counted with weights
(even though, strictly speaking, vertices at infinity don't have
weights). 

The number of vertices of a diagram $\diag$ as above is thus, counting
the vertices at infinity with weights,
\begin{equation}
\label{diag:rel1}
  \Card_w(\vt(\diag))
  = d_\sd(\Delta) + d_+(\Delta) + d_-(\Delta)
  = \Card(\partial\Delta _{\Z}) - d_\sd(\Delta),
\end{equation}
where the last equality is given by Relation
\eqref{eq:polygon:directions}
(the subscript '$w$' indicates that the vertices should be
counted with weigths).
On the other hand, the Euler formula for $\diag_{\rm top}$,
\begin{equation}
\label{eq:polygon:euler}
  \Card(\edg(\diag)) = g-1+ \Card(\vt(\diag)),
\end{equation}
implies, since there is exactly one infinite edge for each vertex at
infinity, 
\begin{equation}
\label{diag:rel2}
  \Card_w(\edg(\diag)) = g-1+ \Card_w(\vt(\diag)),
\end{equation}
where infinite edges are counted with weights (be careful
that, on the contrary, finite edges are not counted with
weigths).
Relations \eqref{diag:rel1} and \eqref{diag:rel2} yield
\begin{equation}
\label{euler}
  \Card_w (\orient) = d_\sd(\Delta) + \Card_w(\edg(\diag))
  = \Card(\partial\Delta _{\Z}) +g -1,
\end{equation}
where infinite edges are counted with weights.


\bigskip
\par We adopt the following graphical convention: floors will be
represented by ellipses, and vertices at infinity will be omitted;
edges will be represented by vertical line segments, the orientation
is from the bottom to the top. %down to up. 
The weight of an edge is indicated
only if it is greater than $1$, as a circled integer.
We indicate $\theta(v)$ inside the ellipse $v$, except if $\theta$
takes the same value on all floors in which case we don't indicate
it.


\begin{examples}
\label{ex:h-tr3}
Let us continue with the examples from \ref{ex:h-tr} and
\ref{ex:h-tr2}. 
For each of these I picture below the unique floor diagram
corresponding to curves with the maximal genus, with respect to 
the direction $\sd =(0,1)$.

\begin{center}
\begin{minipage}{\textwidth/2-5mm}
  \centering
  \vphantom{\includegraphics[scale=.7]{h-tr-hirzebruch.eps}}
  \includegraphics[scale=.7]{h-tr-cubique.eps}
  \captionof{figure}{Floor diagram of Newton polygon $T_3$ and genus
    $1$} 
\end{minipage}
\hspace{7mm}
\begin{minipage}{\textwidth/2-5mm}
  \centering
  \includegraphics[scale=.7]{h-tr-hirzebruch.eps}
  \captionof{figure}{Floor diagram of Newton polygon $\Tz^2_{3,2}$
    (see Figure~\ref{fig:tz}) and genus $8$} 
\end{minipage}
\\[2mm]
\begin{minipage}{\textwidth/2-5mm}
  \centering
  \vphantom{\includegraphics[scale=.7]{h-tr-Wij}}
  \includegraphics[scale=.7]{h-tr-DP4.eps}
  \captionof{figure}{Floor diagram of genus $1$ for the Newton polygon of
    \ref{sp:E4}}
\end{minipage}
\hspace{7mm}
\begin{minipage}{\textwidth/2-5mm}
  \centering
  \includegraphics[scale=.7]{h-tr-Wij}
  \captionof{figure}{Floor diagram of genus $2$ for the Newton polygon of
    \ref{sp:W_ij}}
\end{minipage}
\end{center}
\end{examples}



\bigskip
In order to appropriately count floor diagrams, we need to enhance
them with markings, which encode the distribution of the base points
$\ux$ and of the assigned supports for the boundary conditions
(encoded in the set $\Omega$).
To understand the following definition, keep in mind that the idea is
that if the points $\ux$ are sufficiently stretched in the direction
$\sd$, then for all curves $(C,f) \in \cE_g^\Delta(\alpha,\beta)$, the
points $\ux$ distribute one on each floor or elevator, except on those
elevators that are already taken by a type $\alpha$ boundary condition.
Moreover, we shall label the points $\ux$ according to their order
along the direction $\sd$, which is where 
the monotonicity condition \eqref{marking:increasing} comes
from.

Due to our requirement \ref{p:boundary-dir-d}, the boundary conditions
reduce to only $\alpha^\pm,\beta^\pm \in \Nseq$, tangency conditions
along the top and bottom edges of $\Delta$ respectively, parallel to
direction 
$\orth \sd$ (with '$+$' for the top and '$-$' for the bottom), at
fixed and mobile points respectively.

\begin{definition}
\label{d:mark-diag}
Let $\Delta$ be a $\orth\sd$-transverse lattice polygon, and consider
$g \in \N$, and $\alpha^+,\alpha^-,\beta^+,\beta^- \in \Nseq$, subject to
the conditions
\[
  0\leq g \leq \Card (\mathring{\Delta}_\Z)
  \quad \text{and}
  \quad
  I\alpha^\pm + I\beta^\pm = d_\pm(\Delta).
\]
Set $s = g-1+2d_\sd(\Delta)+|\beta^+|+|\beta^-|$.
A \emph{marking of type $(\alpha^+,\alpha^-,\beta^+,\beta^-)$}
of a floor diagram $(\diag,\theta)$ of genus $g$ and
Newton polygon $\Delta$ is a map
$m: \bigl\{ {-|\alpha^-|+1},\ldots,1,\ldots {s+ |\alpha^+|}
\bigr\}\to \orient$ such that the following conditions hold:
\begin{mycpctenum}[(i)]
\item the map $m$ is injective;
\item\label{marking:increasing}
 if $m(i)>m(j)$ for the order of $\orient$, then $i>j$;
\item for all $k \in \N^*$, if
  $-|\alpha^-|+1 +\sum_{l=1} ^{k-1} \alpha^-_l \leq i \leq
  -|\alpha^-| +\sum_{l=1} ^{k} \alpha^-_l $
  (resp.\
  $s+1 +\sum_{l=1} ^{k-1}  \alpha^+_l \leq i \leq
  s +\sum_{l=1} ^{k} \alpha^+_l $),
  then $m(i) \in \edg^{-\infty}$ (resp.\ $m(i) \in \edg^{+\infty}$),
  and the edge $m(i)$ has weight $k$;
\item for all $k \in \N^*$,
  there are exactly $\beta^\pm_k$ elements of $\edg ^{\pm \infty}$ of
  weight $k$ 
  in $m\bigl( \{1,\ldots,s\} \bigr)$.
\end{mycpctenum}
\end{definition}

A floor diagram $\diag$ enhanced with a marking $m$ of type
$(\alpha^+,\alpha^-,\beta^+,\beta^-)$ is called a
\emph{marked floor diagram} $(\diag,m)$ of type
$(\alpha^+,\alpha^-,\beta^+,\beta^-)$. 

Two marked floor diagrams of the same type are \emph{equivalent}
if there exists a homeomorphism of oriented graphs
$\phi: \diag  \cong \diag'$ such that
$w=w'\circ \phi$, $\theta=\theta'\circ \phi$,
and $m= \phi \circ m'$.

\medskip
Now, the fundamental result is the following.
The enumerative application is given in Corollary
\ref{c:enum-diag} below.

\begin{theorem}[Brugallé--Mikhalkin {\cite[Prop.~5.9]{BM-11}}]
\label{t:stretch=>floor}
Maintain the situation of Definition~\ref{d:mark-diag} above, and
consider the corresponding enumerative problem as in
\ref{p:trop-enumpb}.
If the points $\ux$ are sufficiently strectched along direction $\sd$,
then there is a bijection between
$\cE ^\Delta_g (\alpha,\beta) (\ux, \Omega)$
and the set of equivalence classes of marked floor diagrams of type
$(\alpha^+,\alpha^-,\beta^+,\beta^-)$.
\end{theorem}


I shall not prove this result and refer instead to \cite[\S 5]{BM-11},
but I will try to convey some ideas why it is true.
First of all, it follows from Definition~\ref{d:floors-n-elevators}
how to associate a floor diagram to a tropical curve, with the same
genus and Newton polygon. Moreover, each tangency condition of order
$k$ along the boundary imposed to the tropical curve translates into
a condition that the floor diagram has an infinite edge of weight
$k$.

These features of the curve being fixed, we need to let it move so as
to meet the points $\ux$ and $\Omega$. One has to convince 
oneself that the degrees of freedom in order to do so are to let
floors move along the direction $\sd$ (which correspondingly
stretches the elevators), and let elevators move along the
direction $\orth \sd$.
By the way, note that indeed the number of floors and elevators
(which is also the cardinality of $\orient$) equals
the number of points in $\ux$ and $\Omega$, \ie
$s+|\alpha^+|+|\alpha^-|$ in the above notation, by the version
of formula \eqref{euler} where we no longer count infinite edges with
weights: the number of vertices of $\diag$ is
\[
  \Card(\vt(\diag)) = d_\sd(\Delta)+|\alpha^+|+|\beta^+|
  +|\alpha^-|+|\beta^-|
\]
(compare with \eqref{diag:rel1}),
hence by the Euler formula \eqref{eq:polygon:euler}
\begin{multline*}
  \Card(\orient)
  = \Card(\edg(\diag)) + \Card(\vt(\diag)) -
  \bigl( |\alpha^+|+|\beta^+|
  +|\alpha^-|+|\beta^-| \bigr)
  \\
  = g-1+2d_\sd(\Delta)+|\alpha^+|+|\beta^+|
  +|\alpha^-|+|\beta^-|
  = s+|\alpha^+|+|\alpha^-|,
\end{multline*}
as we said.

How the points $\ux$ and $\Omega$ are taken up by the curve is
encoded in the marking of the corresponding diagram. The points
$\Omega$ must be taken up by pairwise distinct infinite elevators, wich
correspond to infinite edges of the floor diagram.
Next, when the points $\ux$ are sufficiently distant one from another
in direction $\sd$,
it happens that they are taken up one by one by the floors and
remaining elevators.
The condition that the marking $m$ be increasing, \ie
\eqref{marking:increasing} in Definition~\ref{d:mark-diag},
is satisfied when one orders the points $\ux$ following direction
$\sd$; note that the increasing condition is meaningful only in the
range $\{1,\ldots,s\}$ (which corresponds to points $\ux$), as it is
otherwise implied by the requirement that $m(i)$ is in
$\edg^{-\infty}$ if $i<1$ and in $\edg^{+\infty}$ if $i>s$.


Lastly one has to convince oneself that, given the incidence relations
prescribed by a marked floor diagram, there is a unique corresponding
tropical curve.
The idea is this: consider a floor in the diagram; in the plane it
corresponds to a chain of line segments, intersecting various elevators
coming from below or from above (with respect to direction $\sd$) in a
way prescribed by the diagram; each of these elevators has to pass
through one base point prescribed by the marking, so that the line
supporting each elevator in the plane is known. The slope of the
leftmost (with respect to $\sd$) line segment in the chain is
prescribed by the function $\theta$ attached to the diagram, and this
in turn determines the slopes of the other segments via the balancing
condition, see also the proof of Corollary \ref{c:enum-diag}
below. At this point, we know the slopes of all segments in the floor,
and we know that the changes of slopes occur along the lines
supporting the elevators; therefore the incarnation of the floor in
the plane is determined up to translation along the direction $\sd$.
Therefore, there is a unique translate passing through the base point
prescribed by the marking.
It is arguably best to experiment this construction by one's self,
playing around with examples; I provide some material to do so in the
following example.


\begin{example}
\label{ex:cubic-etagees}
We display all marked floor diagrams of rational plane cubics with
trivial boundary conditions in Figures
\ref{ex:cubic-etagees-a}, \ref{ex:cubic-etagees-b},
and \ref{ex:cubic-etagees-c} below.

For the first diagram (Figure \ref{ex:cubic-etagees-a}),
we picture the corresponding
tropical curve for two different distributions of the base points
(always stretched out in the vertical direction).
For both of them, I try to explain how to construct the curves in
practice by showing the constructions lines that I have used to find
the curves, following the
procedure explained in the previous paragraph.

The five next marked diagrams (Figure \ref{ex:cubic-etagees-b})
correspond to 
five different markings of the same diagram. I give the corresponding
plane tropical curves for a given distribution of the base points
(the same distribution for all five curves).
I use black circles to picture the base points, and black squares to
picture the ``nodes'' of the plane tropical curve (one on each curve
in this case).

The three remaining marked diagrams are pictured on
Figure \ref{ex:cubic-etagees-c},
and I leave it as
an exercise to construct the corresponding tropical curves for a given
sufficiently stretched distribution of base points.

\begin{center}
\raisebox{1.5cm}{
\includegraphics[height=2cm]{cubique-a-diag.eps}}
\hspace{2cm}
\includegraphics[height=5cm]{cubique-a-constr.eps}
\hspace{1cm}
\includegraphics[height=5cm]{cubique-a-11.eps}
% \hspace{1cm}
% \includegraphics[height=5cm]{cubique-a-tout.eps}
\hspace{2cm}
\includegraphics[height=5cm]{cubique-abis-constr.eps}
\hspace{1cm}
\includegraphics[height=5cm]{cubique-abis.eps}
\captionof{figure}{Tropical cubics with the same marked floor diagram
  for two different distributions of the base points
(for each, on the left: construction lines)}
\label{ex:cubic-etagees-a}
\end{center}

\begin{center}
\raisebox{1.5cm}{
  \includegraphics[height=2cm]{cubique-b1-diag.eps}}
\hspace{.3cm}
\includegraphics[height=5cm]{cubique-b1.eps}
\hspace{1cm}
\raisebox{1.5cm}{
\includegraphics[height=2cm]{cubique-b2-diag.eps}}
\hspace{.3cm}
\includegraphics[height=5cm]{cubique-b2.eps}
\hspace{1cm}
\raisebox{1.5cm}{
\includegraphics[height=2cm]{cubique-b3-diag.eps}}
\hspace{.3cm}
\includegraphics[height=5cm]{cubique-b3.eps}
\\
\raisebox{1.5cm}{
\includegraphics[height=2cm]{cubique-b4-diag.eps}}
\hspace{.3cm}
\includegraphics[height=5cm]{cubique-b4.eps}
\hspace{1cm}
\raisebox{1.5cm}{
\includegraphics[height=2cm]{cubique-b5-diag.eps}}
\hspace{.3cm}
\includegraphics[height=5cm]{cubique-b5.eps}
\captionof{figure}{Tropical cubics with the same floor diagram,
  all possible markings}
\label{ex:cubic-etagees-b}
\end{center}

\begin{center}
\includegraphics[height=1.5cm]{cubique-c6-diag.eps}
\hspace{1cm}
\includegraphics[height=1.5cm]{cubique-c7-diag.eps}
\hspace{1cm}
\includegraphics[height=1.5cm]{cubique-c8-diag.eps}
\captionof{figure}{Remaining marked floor diagrams for rational plane
  cubics}
\label{ex:cubic-etagees-c}
\end{center}
\end{example}


\paragraph{Warnings} Here are a few caveats about the correspondence
between tropical curves and floor diagrams, which I feel are helpful
to properly understand what is going on.

\smallskip
\subparagraph{}
\label{sp:unordered}
There is no reason why the left infinite directions of floors
(those encoded by $\theta$) would be
ordered following the order in which they appear on the Newton
polygon: this is the reason why the lists $D_l(\Delta)$ and
$D_r(\Delta)$ are unordered.

An example is given in the figure below
(you should try and draw the tropical curve for yourself).
We take $\sd=(0,1)$; the Newton polygon pictured on the left is indeed
$\orth \sd$-transverse.
Note that the floor diagram
has genus $3$, while the arithmetic genus of the Newton polygon is $5$.
The singularities of a curve with the indicated floor diagram are to
be found as intersection points between the planar incarnation of two
distinct floors. 
\begin{center}
\includegraphics[align=c, scale=.8]{unordered-Newton.eps}
\hspace{2cm}
\includegraphics[align=c, scale=.8]{unordered-diag.eps}
\end{center}


\smallskip
\subparagraph{}
In general the datum of the floor diagram does not impose a particular
subdivision of the Newton polygon.
This can be observed on the examples of Figure~\ref{ex:cubic-etagees-a}
above.


\medskip\noindent
Finally, let us give the application of
Theorem~\ref{t:stretch=>floor} to the enumerative problem
\ref{p:enumpb}.

\begin{corollary}
\label{c:enum-diag}
Let $\Delta$ be a $\orth\sd$-transverse lattice polygon, and consider
$g \in \N$, and $\alpha^+,\alpha^-,\beta^+,\beta^- \in \Nseq$, subject to
the conditions
\[
  0\leq g \leq \Card (\mathring{\Delta}_\Z)
  \quad \text{and}
  \quad
  I\alpha^\pm + I\beta^\pm = d_\pm(\Delta).
\]
The number $N_g^\Delta(\alpha^+,\alpha^-,\beta^+,\beta^-)$ equals the
number of equivalence classes of
marked floor diagrams of genus $g$,
Newton polygon $\Delta$,
and type $(\alpha^+,\alpha^-,\beta^+,\beta^-)$, 
where each marked diagram $(\diag, m)$ is to be counted with the
multiplicity 
\begin{equation*}
\mu^\C (\diag,m) = I^\beta \prod _{e \in \edg^{\rm fin}} w(e) ^2.
\end{equation*}
\end{corollary}

\begin{proof}
By Mikhalkin's correspondence theorem \ref{t:M-corresp},
the number $N_g^\Delta(\alpha^+,\alpha^-,\beta^+,\beta^-)$ equals
$I^{-\alpha}$ times the
number of parametrized plane tropical curves
$(C,f) \in \cE ^\Delta_g (\alpha^+,\alpha^-,\beta^+,\beta^-)
(\ux, \Omega)$, for a general choice of points $\ux$ and $\Omega$,
each tropical curve being counted with the multipicity
$\mu^\C(C,f)$ defined in \ref{p:trop-mult}.
In turn, this number counts marked floor diagrams if we take the
points $\ux$ as in Theorem \ref{t:stretch=>floor}.
It thus only remains to show that the multiplicities of the tropical
curves in $\cE ^\Delta_g (\alpha^+,\alpha^-,\beta^+,\beta^-)
(\ux, \Omega)$ relate to that of the corresponding marked floor
diagrams in the appropriate way.

Let us consider a curve $(C,f)$ as above. In the corresponding subdivision
of the Newton polygon $\Delta$, each sub-polygon is a triangle
corresponding to a vertex at which a floor intersects an elevator and
changes slope. Let us thus consider a floor of $(C,f)$, and name
$u_0,\ldots,u_n$ the direction vectors of the various line segments
composing this floor, oriented and numbered from left to right with
respect to direction $\sd$ as indicated on the figure below.
\begin{center}
\begin{minipage}{\textwidth}
\centering
\includegraphics{floor-slopes.eps}
\captionof{figure}{Slopes of line segments along a floor}
\end{minipage}
\end{center}
Label the vertices on this floor from $1$ to $n$, and for each let
$w_i$ be the weight of the corresponding elevator, and $\epsilon_i=+1$
(resp.\ $-1$) if it arrives from the bottom (resp.\ from the top).
The balancing condition says that, for all $i=0,\ldots,n$,
\begin{equation}
\label{balance:floor}
  u_i = u_{i-1} + \epsilon_i w_i \sd.
\end{equation}
By $\orth\sd$-transversality, one has
$\det(u_0, \sd) =\pm 1$.
Then it follows from the induction relation \eqref{balance:floor} that
$\det(u_i, \sd) =\pm 1$ for all $i=0,\ldots,n$,
hence the vertex $\#i$ contributes to the multiplicity $\mu^\C(C,f)$ by
$w_i$, \cf \eqref{eq:mult-vertex}.

Thus, the multiplicity $\mu^\C(C,f)$ may be computed as a product of
contributions from the elevators, the contribution of an elevator of
weight $w$ being $w$ (resp.\ $w^2$) if it is attached to one (resp.\
two) floor. Therefore
\[
  \mu^\C(C,f) =
  \prod _{e \in \edg^{\pm \infty}} w(e)
  \cdot
  \prod _{e \in \edg^{\rm fin}} w(e) ^2,
\]
where the products on the right-hand-side are indexed on the edges of
the floor diagram associated to $(C,f)$.
This coincides with the multiplicity $\mu^\C(\diag,m)$ after we
multiply by the factor $I^{-\alpha}$ indicated by
Mikhalkin's correspondence theorem.
\end{proof}


\bigskip
Applications of Corollary \ref{c:enum-diag}
to the enumeration of plane cubics with various tangency conditions
along a fixed line have already been given in
\cite[\tref{ex:cubics-diag}]{07.th-diag-degen}.
Let us now give a few other examples,
in continuation of Section \ref{s:degenK3}.

\begin{examples}
We continue with some of the examples from \ref{ex:h-tr},
\ref{ex:h-tr2}, and \ref{ex:h-tr3}.

\smallskip
\subparagraph{Class of the quartic surface of \ref{sp:E4}}
\label{sp:E4-floor}
This amounts to counting marked floor diagrams of type $\Delta$ and
genus $0$ (with trivial boundary conditions), where $\Delta$ is the
square displayed in \ref{sp:E4}, with respect to the direction
$\sd =(0,1)$. There is only one such diagram up to equivalence, which
is the following.
\begin{center}
\includegraphics[scale=.7]{h-tr-DP4-g0.eps}
\captionof{figure}{Floor diagram of genus $0$ for the Newton polygon of
  \ref{sp:E4}}
\end{center}
Thus the number of irreducible rational curves in a pencil of
hyperplane sections 
of the surface $(xy-t^2=zw-t^2=0) \subset \P^4$ is $4$, by Corollary
\ref{c:enum-diag}.

\bigskip
\subparagraph{Invariants of the octic surface of \ref{sp:W_ij}}
\label{sp:tropWij0}
We want to count irreducible genus $1$ (resp.\ genus $0$) curves in a
pencil (resp.\ a web) of hyperplane sections of the octic surface in
$\P^7$ corresponding to the rectangle $\Delta$ displayed in
\ref{sp:W_ij}. 
The corresponding marked floor diagrams,
with respect to direction $\sd =(0,1)$,
are the following.
\begin{center}
\begin{minipage}[b]{7cm}
  \centering
\includegraphics[scale=.7]{h-tr-Wij-g1a.eps}
\hspace{.4cm}
\includegraphics[scale=.7]{h-tr-Wij-g1b.eps}
\hspace{.4cm}
\includegraphics[scale=.7]{h-tr-Wij-g1c.eps}
\captionof{figure}{Genus $1$ floor diagrams}
\label{fig:tropWij0:diag1}
\end{minipage}
\hspace{.4cm}
\begin{minipage}[b]{6cm}
  \centering
  \includegraphics[scale=.7]{h-tr-Wij-g0.eps}
  \captionof{figure}{Genus $0$ floor diagram}
\label{fig:tropWij0:diag0}
\end{minipage}
\end{center}
In the genus $1$ case, the rightmost diagram has four possible
markings, as $i$ may take any value in $\intint 1 4$, which then
determines the rest of the marking (\ie the marking of the one floor and
two elevators with nothing indicated on the figure). 
We thus find
$N_1^\Delta = 12$, and $N_0^\Delta = 16$.

Note that the number in genus $1$ does not coincide with the one given
in \ref{sp:W_ij}, which is not a contradiction because this is not the
same 
enumerative problem: in the computation above, no base points have been
imposed along the toric anticanonical cycle, whereas in \ref{sp:W_ij}
all the points along the toric anticanonical cycle are fixed.
The latter computation cannot be performed purely in terms of floor
diagrams, because we want too many boundary conditions with respect to
what is possible, according to the condition given
in \ref{p:boundary-dir-d}. We solve the tropical problem corresponding
to the enumerative problem of \ref{sp:W_ij} in the next example.
\end{examples}


\begin{example}
\label{sp:tropWij}
So, let us consider the enumerative problem of \ref{sp:W_ij}:
we let $\Delta$ be the Newton polygon indicated below, and fix
$\alpha=(2,1,2,0)$, $\beta=(0,0,0,1)$. Thus the set $\Omega$
of boundary conditions consists of
five real values, fixing five lines $\sL_1,\sL_1', \sL_2, \sL_3,
\sL_3'$ as indicated on the picture below.
\begin{center}
\includegraphics[height=1.5cm,align=c]{tropWij-N.eps}
\qquad ; \qquad\qquad
\includegraphics[height=4cm, align=c]{tropWij-data.eps}
\end{center}
The tropical curves defined by this data move in a $2$-dimensional
family, in the way pictured below (three curves are pictured, in
green, blue, and purple, respectively):
the deformations of the curves amount to
change the sizes of the two rectangles by letting their corners slide
along the lines $\sL_i$ and $\sL_i'$.
As the curves move in this family, one notices that the semi-line
corresponding to the edge $\Sigma_4$ of the Newton polygon is always
supported on the same line, which we shall call $\tilde{\sL}_4$:
this is yet another tropical incarnation of the
toric Cayley--Bacharach property stated in Lemma~\ref{l:torCB}.
\begin{center}
\includegraphics[height=4cm]{tropWij-web.eps}
\hspace{15mm}
\includegraphics[height=4cm]{tropWij-CB.eps}
\captionof{figure}{A pencil of tropical curves and the
  Cayley--Bacharach property}
\label{fig:Wij:tropical-CB}
\end{center}
We want to count curves of genus $g=1$ and $g=0$ in this system.
Let us focus on the case of genus $g=1$.
We need to fix a set $\ux$ of base points consisting of one point
only, which is represented by a black dot on 
Figure~\ref{fig:tropWij:g1} below. With the configuration depicted on
this figure, we find the four physical curves represented below:
the first two count with multiplicity $1$ each, and the last two with
multiplicity $4$ each. This confirms the number $N^\Delta_1 = 10$
given in \ref{sp:W_ij} and found in \cite{quartiche}.
\begin{center}
\null \hfill
\includegraphics[align=c,height=4cm]{tropWij-g1a.eps}
\hfill
\includegraphics[align=c,height=4cm]{tropWij-g1b.eps}
\hfill
\includegraphics[align=c,height=4cm]{tropWij-g1c.eps}
\hfill
\includegraphics[align=c,height=4cm]{tropWij-g1d.eps}
\hfill \null
\captionof{figure}{Genus $1$ curves in the pencil defined by one base
  point}
\label{fig:tropWij:g1}
\end{center}
Note that these four curves all have a perfectly fine floor
decomposition, with corresponding (unmarked) floor diagram one of the
diagrams in Figure~\ref{fig:tropWij0:diag1} above. It is however not true
that the base points and boundary conditions are taken up exactly one
by one by the floors and elevators.

To complete the picture, note that there is a unique genus $g=0$ curve
in this tropical linear system, which you can see by filling out the
spaces between the dots in the picture on the right of
Figure~\ref{fig:Wij:tropical-CB}. It counts with multiplicity $16$,
and has the (unmarked) floor diagram given in
Figure~\ref{fig:tropWij0:diag0}.
\end{example}


\section{Tropical representation of algebraic curves}
\label{S:trop-design}

In this section we elaborate on the idea that tropical curves are
great for the graphic representation of algebraic curves in toric
surfaces, and illustrate this with meaningful examples.  A natural
attempt to represent complex algebraic plane curves is to draw the set
of their real points, in $\R^2$ say, but as anyone who has tried
knows, this does not reflect the reality of things very well. For
instance, the set of real points may be disconnected, it may contain
isolated points, and it does not respect the Bezout Theorem. These
problems do not occur with tropical curves.

\begin{theorem}[Bezout Theorem, see
  {\cite[Section 4]{richter-gebert-etal}}]
Let $C,D \subset \R^2$ be two plane tropical curves with Newton
polygon $\Delta$. If $C$ and $D$ intersect at finitely many points,
then the number of their intersection points, counted with
multiplicities, 
is $c_1(\O_{X_\Delta}(1))^2 = 2 \Ar (\Delta)$,
in the notation of \ref{sp:p_a}.
\end{theorem}

\noindent
The intersection multiplicity of two line segments with primitive
direction vectors $u$ and $v$ and multiplicities $m$ and $n$ is
defined as $m\cdot n\cdot \bigl| \det(u,v) \bigr|$.
Note that the theorem says not only that all intersection points are
visible in the tropical shadow, but also that none of them has
wandered at infinity to some component of the anticanonical cycle. 

The next property is merely an observation, as it follows directly
from the definition of the Newton polygon of a plane tropical curve.
At a more conceptual level, plane tropical curves are by
design projected shadows of curves in the torus $(\C^*)^2$; it is
therefore expected that they behave well with respect to the
completion of $(\C^*)^2$ in a toric surface by the addition of a toric
boundary. 

\begin{remark}
Let $C \subset \R^2$ be a plane tropical curve with Newton polygon
$\Delta$.
The number, counted with multiplicities,
of infinite branches of $C$ in the direction corresponding to
a segment $\delta$ of the boundary of $\Delta$ equals the intersection
number $c_1(\O_{X_\Delta}(1)) \cdot C_\delta$, where $C_\delta$
is the component of the anticanonical cycle $\antiK_\Delta$
corresponding to $\delta$.
\end{remark}


Now, the principles of ``my'' tropically inspired way of graphically
representing algebraic curves on (surfaces birational to) toric
surfaces are the following.

\paragraph{Graphic representation}
Let $C$ be a curve in a toric surface $X_\Delta$.
We represent the surface $X_\Delta$ by drawing its anticanonical cycle
$\antiK_\Delta$ as a polygon (which looks much like the Newton polygon
$\Delta$); then the surface $X_\Delta$ is the inside of this polygon.
To represent the curve $C$, we draw a (finite length portion of a)
tropical curve $C_\trop$ with the same 
Newton polygon as $C$, inside the polygon representing $X_\Delta$: the
infinite branches of $C_\trop$ are represented by finite segments
hitting the appropriate segment of $\antiK_\Delta$, and the finite
segments of $C_\trop$ do not hit $\antiK_\Delta$.
The concept of tropical toric varieties,
see \cite[Section 7.3]{BIMS}, gives a
mathematical meaning to this graphic process.

Note that the Newton polygon of $C$ may differ from $\Delta$: for
instance, we may want to represent a fibre of the ruling of a
Hirzebruch surface $\F_e$, or a curve $C$ in $\F_e$ such that the
complete linear system $|C|$ represents $\F_e$ as a cone over a
rational normal curve.
In this case the curve $C$ is not ample in $X_\Delta$,
and some segments of
$\antiK_\Delta$ will not be hit by any infinite branch of $C_\trop$.
We give first examples in Figure \ref{fig:graphic-exem1}.

\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth-10mm]{graphic-exem1.eps}
\caption{Curves linearly equivalent to
  $H$ in $\P^2$, $H$ in $\F_1$, $F$ in $\F_1$, and $H+F$ in $\F_1$}
\label{fig:graphic-exem1}
\begin{minipage}{\textwidth}
\centering
(in the notation introduced in \ref{p:notation})
\end{minipage}
\end{figure}

One more nice feature of this way of picturing curves is that it lets
graphically see the genus, as it is the first Betti number of the
real object that we are actually seeing. Thus, in Figure
\ref{fig:graphic-exem2}, we see that the curve on the left (resp., on
the right) has genus one (resp., two).

\begin{figure}[htbp]
\centering
\includegraphics{graphic-exem2.eps}
\caption{Hyperplane sections of the cubic of \ref{sp:3A2} and the
  quartic of \ref{sp:W_ij}}
\label{fig:graphic-exem2}
\end{figure}


Note that what we are considering is really representations of algebraic
curves inspired by tropical geometry, and not actual tropical curves.
In particular, we may forget about the integral structure underlying
$\R^2$ (\ie, $\Z^2$), the balancing condition, the subdivision of the
Newton polygon of the curve, and so on. This allows for an
essentialization of our drawings: we may for instance
simply represent a Hirzebruch
surface by a rectangle instead of a trapezium (or by whatever
quadrilateral we fancy), and simplify the representations of curves as
indicated on Figure \ref{fig:graphic-essence}.

\begin{figure}[htbp]
\centering
\includegraphics{graphic-essence.eps}
\caption{Curves linearly equivalent to
  $3H$ in $\P^2$, and $H+F$ in $\F_1$}
\label{fig:graphic-essence}
\end{figure}

In the same vein it frequently happens, as we have seen in
\cite{01.ciro}, 
 that one needs to represent
curves that actually lie on some blow-up of a toric surface at points
lying on the toric boundary. In that case we adapt our representation
in a rather flexible way without much trouble.

Our interest resides especially in representing curves lying on
reducible surfaces, the irreducible components of which are toric
surfaces (or blow-ups thereof). In that case we may simply tile our
polygons so as to reflect the dual graph of the various irreducible
components, somehow as in \ref{specule-degen}.
A nice example is given in \cite[Figure
\ttref{fig:granchio}]{01.ciro}. In that example, the dual graph
of our reducible surface is a tiling of the sphere $\SS^2$, and we have
tweaked some of the sides of our polygons to obtain a better looking
drawing; incidentally, we have also tweaked some line segments of the
representation of our curve.
Note that the surface $T^1$ is actually outside of its
polygon, as we have performed a kind of stereographic projection from
a point inside this surface $T^1$, in order to represent the sphere
$\SS^2$ on the plane.
You may observe that the representation of the curve is topologically
the same as 
the union of the edges of a tetrahedron, which is none other than the
dual of the tetrahedron (in the sense of Section
\ref{s:degenK3})
we had started with.



\paragraph{Application to Brugallé degenerations
  {\normalfont (see \cite{07.th-diag-degen})}}
\label{p:trop-erwan}
I will simply give an example which, I believe,
displays all I want to show.
Let us follow a degeneration of a plane cubic along the
degeneration of $\P^2$ to a chain of Hirzebruch $\F_1$ surfaces
$S_0,\ldots,S_9$, with a (useless) projective plane $S_{10}$ at one
end of the chain. The plane cubic degenerates
(in our example) to a curve which
restricts to curves linearly equivalent to $H$ on $S_9$, $H+F$ on
$S_7$, $H+2F$ on $S_4$, and
multiples of $F$ on all other $\F_1$ surfaces (and $0$
on the plane), in the notation introduced in \ref{p:notation}.
We may see our plane cubic as a hyperplane section of
the Veronese surface $v_3(\P^2) \subset \P^9$, and its degeneration as
a hyperplane section of a ``reducible toric surface'' as in
\ref{specule-degen}, made of a projective plane, attached to a
rational normal scroll of type $(1,2)$ along a line, and the latter
attached to a scroll of type $(2,3)$ along a conic.

In Figure \ref{fig:erwanA}, we have drawn ``proper tropical curves''
inside the various polygons (those on which the curve has class $F$
are skipped). Now the wonder is that when we put all the pieces
together, what we obtain is a plane tropical cubic!
In Figure \ref{fig:erwanB}, we have drawn ``essentialized tropical
curves''; if you look at their patching together with the
right kind of eyes, you should see only floors and elevators.

\begin{subnum-fig}
\begin{figure}[htbp]
\centering
\includegraphics[scale=.8]{degen-erwan-sm3ic-trop.eps}
\caption{Smooth plane cubic in a degeneration of $v_3(\P^2)$
  to a union of scrolls (tropical version)}
\label{fig:erwanA}
\end{figure}

\begin{figure}[htbp]
\includegraphics[width=\textwidth]{degen-erwan-sm3ic-th.eps}
\caption{Smooth plane cubic in a degeneration of $v_3(\P^2)$
  to a union of scrolls (arts déco version)}
\label{fig:erwanB}
\end{figure}
\end{subnum-fig}


\begin{references}
  

\begin{thebibliography}[Chapters in this Volume\footnote
  {see \url{https://www.math.univ-toulouse.fr/~tdedieu/\#enumTV}}]{VIII}

\bibitem[I]{01.ciro}
  C.~Ciliberto and Th.~Dedieu,
  \emph{Limits of nodal curves: generalities and examples}.

\bibitem[III]{03.th-acz}
  \Th.~Dedieu,
  \emph{Geometry of logarithmic Severi varieties at a general
  point}.

\bibitem[VI]{04.concettina}
Th.~Dedieu and C.~Galati,
\emph{Degenerations and deformations of generalized Severi varieties}.

\bibitem[IX]{07.th-diag-degen}
\Th.~Dedieu, \emph{Enumeration of curves by floor diagrams, via degenerations of
  the projective plane}.

\bibitem[XI]{10.th-panoramico}
Th.~Dedieu,
\emph{Enumerative geometry of $K3$ surfaces}.

\bibitem[XII]{13.th-classic}
Th.~Dedieu,
\emph{Some classical formul{\ae} for curves and surfaces}.

\bibitem[XIII]{14.th-vainsencher}
Th.~Dedieu,
\emph{Node polynomials for curves on surfaces}.

\bibitem[XIV]{12.fra-goettsche}
F.~Bastianelli and Th.~Dedieu,
\emph{The G\"ottsche conjecture
  and the G\"ottsche--Yau--Zaslow formula}.

\end{thebibliography}


\begin{thebibliography}[External References]{99}

\bibitem{arnold}
V.~I. {Arnold}, \emph{Mathematical methods of classical mechanics}, second
  \smfedname, Graduate Texts in Mathematics, vol.~60, Springer-Verlag, New
  York, 1989, Translated from the Russian by K. Vogtmann and A. Weinstein.

\bibitem{arroyoetal-11}
A.~Arroyo, E.~Brugall\'{e} {\normalfont \smfandname} L.~L\'{o}pez~de Medrano,
  \emph{Recursive formulas for {W}elschinger invariants of the projective
  plane}, Int. Math. Res. Not. IMRN (2011), no.~5, 1107--1134.

\bibitem{block-gathmann-markwig}
F.~Block, A.~Gathmann {\normalfont \smfandname} H.~Markwig, \emph{Psi-floor
  diagrams and a {C}aporaso-{H}arris type recursion}, Israel J. Math.
  \textbf{191} (2012), no.~1, 405--449.

\bibitem{erwan-11}
  E.~Brugallé,
  \emph{Floor diagrams relative to a conic, and GW–W
    invariants of Del Pezzo surfaces},
  Adv.\ Math.\ \textbf{279} (2015), 438--500.

\bibitem{BIMS}
E.~Brugall\'e, I.~Itenberg, G.~Mikhalkin {\normalfont \smfandname} K.~Shaw,
\emph{Brief introduction to tropical geometry},
in \emph{Proceedings of the {G}\"okova {G}eometry-{T}opology
{C}onference 2014},
G\"okova Geometry/Topology Conference (GGT), G\"okova, 2015, 1--75.

\bibitem{BM-higherdim}
E.~Brugall\'{e} {\normalfont \smfandname} G.~Mikhalkin, \emph{Floor
  decompositions of tropical curves in any dimension},
  \url{http://erwan.brugalle.perso.math.cnrs.fr/miscellaneous.html}.

\bibitem{AMMonthly}
E.~Brugall\'e {\normalfont \smfandname} K.~Shaw, \emph{A bit of tropical
  geometry}, Amer. Math. Monthly \textbf{121} (2014), no.~7, 563--589.

\bibitem{BM-11}
\bysame , \emph{Floor decompositions of tropical curves: the planar case}, in
  \emph{Proceedings of {G}\"{o}kova {G}eometry-{T}opology {C}onference 2008},
  G\"{o}kova Geometry/Topology Conference (GGT), G\"{o}kova, 2009, 64--90.

\bibitem{cavalieri-etal}
R.~Cavalieri, P.~Johnson, H.~Markwig {\normalfont \smfandname} D.~Ranganathan,
  \emph{Counting curves on {H}irzebruch surfaces: tropical geometry and the
  {F}ock space}, Math. Proc. Cambridge Philos. Soc. \textbf{171} (2021), no.~1,
  165--205.

\bibitem{quartiche}
C.~Ciliberto {\normalfont \smfandname} \Th.~Dedieu, \emph{Limits of pluri-tangent
  planes to quartic surfaces}, in \emph{Algebraic and complex geometry},
  Springer Proc. Math. Stat., vol.~71, Springer, Cham, 2014, 123--199.

\bibitem{CLS}
D.~A. Cox, J.~B. Little {\normalfont \smfandname} H.~K. Schenck, \emph{Toric
  varieties}, Graduate Studies in Mathematics, vol.~124, American Mathematical
  Society, Providence, RI, 2011.

\bibitem{kapranov-etal}
M.~Einsiedler, M.~Kapranov {\normalfont \smfandname} D.~Lind,
  \emph{Non-{A}rchimedean amoebas and tropical varieties}, J. Reine Angew.
  Math. \textbf{601} (2006), 139--157.

\bibitem{fomin-mikhalkin}
S.~Fomin {\normalfont \smfandname} G.~Mikhalkin, \emph{Labeled floor diagrams
  for plane curves}, J. Eur. Math. Soc. (JEMS) \textbf{12} (2010), no.~6,
  1453--1496.

\bibitem{gathmann-markwig}
A.~Gathmann {\normalfont \smfandname} H.~Markwig, \emph{The {C}aporaso-{H}arris
  formula and plane relative {G}romov-{W}itten invariants in tropical
  geometry}, Math. Ann. \textbf{338} (2007), no.~4, 845--868.

\bibitem{gkz}
I.~M. Gelfand, M.~M. Kapranov {\normalfont \smfandname} A.~V. Zelevinsky,
  \emph{Discriminants, resultants and multidimensional determinants}, Modern
  Birkh\"auser Classics, Birkh\"auser Boston, Inc., Boston, MA, 2008, Reprint
  of the 1994 edition.

\bibitem{X-UPS}
  P.~Harinck, A.~Plagne {\normalfont \smfandname} C.~Sabbah eds,
  \emph{Géométrie tropicale (X-UPS 2008)},
  Éditions de l'École Polytechnique, Palaiseau, 2008.
  With contributions by
  E.~Brugallé, I.~Itenberg, B.~Teissier.

\bibitem{hull}
J.-B. Hiriart-Urruty {\normalfont \smfandname} C.~Lemar\'echal,
  \emph{Fundamentals of convex analysis}, Grundlehren Text Editions,
  Springer-Verlag, Berlin, 2001.

\bibitem{tropicalOW}
I.~Itenberg, G.~Mikhalkin {\normalfont \smfandname} E.~Shustin, \emph{Tropical
  algebraic geometry}, second \smfedname, Oberwolfach Seminars, vol.~35,
  Birkh\"auser Verlag, Basel, 2009.

\bibitem{Kontsevich}
M.~Kontsevich,
\emph{What is tropical mathematics?},
talk at the Fields Institute, Toronto, 2013,
\url{https://video-archive.fields.utoronto.ca/list/event/170}.

\bibitem{kontsevich-soibelman}
M.~Kontsevich {\normalfont \smfandname} Y.~Soibelman, \emph{Homological mirror
  symmetry and torus fibrations}, in \emph{Symplectic geometry and mirror
  symmetry ({S}eoul, 2000)}, World Sci. Publ., River Edge, NJ, 2001, 203--263.

\bibitem{mikhalkin-faces}
G.~Mikhalkin, \emph{Amoebas of algebraic varieties and tropical geometry}, in
  \emph{Different faces of geometry}, Int. Math. Ser. (N. Y.), vol.~3,
  Kluwer/Plenum, New York, 2004, 257--300.

\bibitem{mikhalkin-pants}
\bysame , \emph{Decomposition into pairs-of-pants for complex algebraic
  hypersurfaces}, Topology \textbf{43} (2004), no.~5, 1035--1065.

\bibitem{mikhalkin-JAMS}
\bysame , \emph{Enumerative tropical algebraic geometry in {$\mathbb{R}^2$}},
  J. Amer. Math. Soc. \textbf{18} (2005), no.~2, 313--377.

\bibitem{nishinou-siebert}
T.~Nishinou {\normalfont \smfandname} B.~Siebert, \emph{Toric degenerations of
  toric varieties and tropical curves}, Duke Math. J. \textbf{135} (2006),
  no.~1, 1--51.

\bibitem{richter-gebert-etal}
J.~Richter-Gebert, B.~Sturmfels {\normalfont \smfandname} T.~Theobald,
  \emph{First steps in tropical geometry}, in \emph{Idempotent mathematics and
  mathematical physics}, Contemp. Math., vol.~377, Amer. Math. Soc.,
  Providence, RI, 2005, 289--317.

\bibitem{shustin}
E.~Shustin, \emph{A tropical approach to enumerative geometry}, Algebra i
  Analiz \textbf{17} (2005), no.~2, 170--214, a.k.a. Patchworking singular
  algebraic curves, non-Archimedean amoebas and enumerative geometry.

\bibitem{viro}
O.~Viro, \emph{Dequantization of real algebraic geometry on logarithmic paper},
  in \emph{European {C}ongress of {M}athematics, {V}ol. {I} ({B}arcelona,
  2000)}, Progr. Math., vol.~201, Birkh\"auser, Basel, 2001, 135--146.

\end{thebibliography}


% \bibliographystyle{mysmf-alpha}
% \bibliography{etages}


\end{references}


\stopcontents[toric-trop]





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End: 
 	

